Towards Tackling MaxSAT by Combining Nested Monte Carlo with Local Search

Recent work proposed the UCTMAXSAT algorithm to address Maximum Satisfiability Problems (MaxSAT) and shown improved performance over pure Stochastic Local Search algorithms (SLS). UCTMAXSAT is based on Monte Carlo Tree Search but it uses SLS instead of purely random playouts. In this work, we introduce two algorithmic variations over UCTMAXSAT. We carry an empirical analysis on MaxSAT benchmarks from recent competitions and establish that both ideas lead to performance improvements. First, a nesting of the tree search inspired by the Nested Monte Carlo Search algorithm is effective on most instance types in the benchmark. Second, we observe that using a static flip limit in SLS, the ideal budget depends heavily on the instance size and we propose to set it dynamically. We show that it is a robust way to achieve comparable performance on a variety of instances without requiring additional tuning.

==> tables/fullexperiments_160v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{3}{*}{1300}
&1&1116.1&1114.9&1118.3&1121.4&1121.7&1121.1&1133\\
&2&1147.0&1148.3&1150.0&1155.1&1154.9&1153.4&1161\\
&3&1122.5&1123.7&1123.4&1130.2&1130.9&1130.8&1143\\
\midrule
\multirow{3}{*}{1400}
&1&1215.1&1215.8&1217.8&1222.8&1221.7&1220.7&1234\\
&2&1218.3&1219.1&1218.3&1223.9&1225.7&1224.2&1236\\
&3&1213.0&1213.6&1216.3&1222.6&1221.2&1219.1&1233\\
\midrule
\multirow{3}{*}{1500}
&1&1294.3&1296.8&1295.7&1304.2&1303.2&1300.1&1317\\
&2&1278.1&1277.7&1278.6&1284.6&1283.4&1283.8&1300\\
&3&1297.0&1298.1&1299.2&1306.0&1306.0&1302.8&1316\\
\midrule
\multirow{3}{*}{1600}
&1&1354.4&1354.0&1355.3&1362.1&1363.4&1361.1&1378\\
&2&1354.1&1354.5&1355.1&1360.3&1362.5&1362.0&1378\\
&3&1362.0&1361.0&1364.3&1370.8&1370.5&1368.1&1387\\
\midrule
\multirow{3}{*}{1700}
&1&1449.6&1449.4&1450.7&1458.2&1460.0&1456.9&1474\\
&2&1446.0&1445.9&1448.9&1454.9&1455.7&1452.8&1470\\
&3&1424.4&1426.2&1427.0&1434.6&1434.6&1432.7&1451\\
\midrule
\multirow{3}{*}{1800}
&1&1517.6&1519.8&1520.6&1529.5&1528.3&1528.3&1548\\
&2&1517.5&1517.9&1521.1&1526.5&1526.9&1525.4&1544\\
&3&1519.5&1520.8&1521.7&1527.6&1528.2&1527.3&1545\\
\midrule
\multirow{3}{*}{1900}
&1&1612.9&1613.0&1615.7&1624.0&1622.3&1618.4&1639\\
&2&1610.2&1610.6&1611.6&1620.0&1615.7&1618.9&1638\\
&3&1608.5&1607.4&1611.2&1616.5&1618.7&1614.6&1636\\
\midrule
\multirow{3}{*}{2000}
&1&1677.3&1676.8&1680.3&1687.1&1687.1&1683.4&1707\\
&2&1697.0&1696.7&1699.9&1710.8&1708.0&1707.7&1728\\
&3&1684.4&1686.4&1691.1&1698.6&1698.4&1700.8&1718\\
\midrule
\multirow{3}{*}{2100}
&1&1776.3&1777.5&1780.5&1783.9&1783.2&1784.2&1806\\
&2&1772.4&1772.3&1774.1&1780.3&1781.1&1781.7&1801\\
&3&1764.6&1765.7&1768.6&1775.3&1774.0&1771.6&1795\\
\midrule
\multirow{3}{*}{2200}
&1&1858.6&1858.7&1862.3&1864.8&1869.1&1867.3&1890\\
&2&1830.9&1831.7&1834.1&1844.7&1841.6&1838.9&1867\\
&3&1840.7&1842.3&1845.7&1851.4&1852.1&1850.7&1874\\
\midrule
\multirow{3}{*}{2300}
&1&1913.4&1914.3&1918.3&1923.6&1919.5&1925.9&1947\\
&2&1915.8&1915.1&1917.3&1927.1&1921.8&1923.2&1951\\
&3&1923.1&1923.1&1922.9&1930.2&1930.5&1929.1&1957\\
\midrule
\multirow{3}{*}{2400}
&1&1992.7&1991.2&1997.6&1999.5&2000.6&2000.7&2030\\
&2&1999.7&2002.7&2002.2&2008.2&2008.7&2009.9&2035\\
&3&1981.5&1980.2&1981.6&1993.0&1990.3&1987.1&2020\\
\midrule
\multirow{3}{*}{2500}
&1&2080.3&2079.5&2083.0&2089.7&2092.8&2087.9&2117\\
&2&2081.6&2082.2&2086.9&2087.5&2087.4&2090.8&2120\\
&3&2081.3&2079.5&2085.2&2088.7&2090.3&2088.4&2118\\
\midrule
\multirow{3}{*}{1300}
&1&2166.4&2168.7&2171.0&2177.1&2178.0&2176.5&2208\\
&2&2161.0&2163.3&2167.5&2174.3&2174.7&2172.2&2203\\
&3&2147.9&2148.1&2149.8&2153.9&2162.7&2151.5&2187\\
statistic&\\


\midrule
\multicolumn{2}{l}{Aggregate}&1643.5&1643.9&1646.2&1652.5&1652.6&1651.2&1672.38\\
\bottomrule
\end{tabular}

==> tables/fullexperiments_180v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{4}{*}{1200}
&1&1049.4&1049.7&1051.9&1054.3&1054.9&1055.5&1066\\
&2&1053.3&1054.3&1055.3&1061.9&1060.4&1059.3&1070\\
&3&1055.6&1056.5&1057.7&1060.3&1059.7&1059.8&1069\\
&4&1055.4&1055.6&1059.0&1062.7&1061.4&1062.2&1072\\
&1&1126.4&1127.1&1128.8&1134.5&1133.7&1128.9&1147\\
&2&1145.7&1145.8&1146.6&1153.8&1154.2&1151.9&1162\\
&3&1133.1&1131.1&1134.0&1138.5&1139.0&1137.5&1150\\
&4&1133.3&1133.7&1134.8&1139.7&1139.5&1137.8&1151\\
&1&1214.9&1214.6&1216.3&1221.1&1222.6&1222.1&1235\\
&2&1215.8&1215.5&1218.4&1222.2&1222.5&1222.7&1235\\
&3&1227.7&1228.6&1230.7&1234.8&1234.2&1231.5&1244\\
&4&1218.0&1216.9&1221.8&1226.5&1229.4&1226.6&1240\\
&1&1293.2&1293.3&1296.4&1301.2&1299.7&1303.1&1316\\
&2&1297.0&1297.2&1299.0&1304.7&1304.5&1304.3&1320\\
&3&1295.8&1297.1&1299.7&1303.7&1305.2&1305.0&1321\\
&4&1296.3&1296.4&1298.5&1303.5&1302.4&1302.9&1319\\
&1&1376.4&1376.2&1379.9&1383.5&1382.5&1380.5&1400\\
&2&1369.8&1368.7&1370.8&1374.3&1373.3&1375.8&1396\\
&3&1359.8&1357.9&1359.7&1365.7&1365.1&1364.3&1384\\
&4&1377.3&1376.4&1378.3&1384.8&1383.2&1384.0&1400\\
&1&1449.6&1450.2&1452.3&1455.9&1455.5&1458.2&1475\\
&2&1444.6&1443.1&1447.3&1450.8&1448.7&1450.3&1471\\
&3&1467.2&1466.6&1469.9&1472.6&1475.5&1475.0&1491\\
&4&1469.0&1469.2&1472.5&1473.9&1474.6&1476.8&1494\\
&1&1528.9&1530.1&1533.8&1535.4&1537.3&1535.8&1559\\
&2&1530.4&1530.1&1531.1&1538.2&1535.7&1536.8&1558\\
&3&1541.8&1542.4&1545.0&1549.9&1548.0&1547.5&1568\\
&4&1529.0&1530.2&1533.2&1537.6&1538.4&1536.3&1559\\
&1&1626.4&1625.1&1629.3&1633.9&1635.1&1633.6&1655\\
&2&1625.8&1627.0&1628.4&1634.9&1635.2&1629.9&1654\\
&3&1615.4&1617.5&1617.6&1626.6&1622.1&1625.5&1648\\
&4&1609.1&1609.6&1612.7&1618.6&1618.5&1622.5&1643\\
&1&1683.6&1683.7&1684.6&1689.9&1693.6&1693.7&1718\\
&2&1683.4&1683.8&1685.4&1691.7&1692.7&1692.9&1715\\
&3&1699.5&1702.3&1702.3&1706.1&1706.9&1707.0&1729\\
&4&1686.9&1686.3&1689.6&1692.7&1694.9&1695.3&1720\\
&1&1773.0&1775.7&1775.1&1781.9&1780.7&1780.1&1806\\
&2&1763.0&1763.3&1765.5&1768.9&1773.6&1770.7&1799\\
&3&1773.5&1775.0&1776.8&1781.1&1783.3&1782.1&1807\\
&4&1755.3&1758.0&1759.8&1764.3&1770.5&1770.6&1797\\
&1&1835.0&1838.3&1838.5&1842.1&1840.2&1843.0&1870\\
&2&1842.8&1843.7&1846.8&1843.2&1851.4&1851.3&1882\\
&3&1856.4&1858.8&1862.3&1868.3&1868.9&1865.4&1894\\
&4&1847.2&1847.5&1849.7&1856.1&1856.5&1853.2&1883\\

\midrule
\multicolumn{2}{l}{Aggregate}&1453.0&1453.4&1455.6&1460.1&1460.6&1460.2&1479.36\\
\bottomrule
\end{tabular}

==> tables/fullexperiments_80v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{10}{*}{600}
&1&586.0&585.9&586.0&586.0&586.0&585.8&586\\
&2&584.0&584.0&584.0&584.0&584.0&584.0&584\\
&3&589.0&589.0&589.0&589.0&589.0&589.0&589\\
&4&587.0&587.0&587.0&587.0&587.0&587.0&587\\
&5&588.0&588.0&588.0&588.0&588.0&588.0&588\\
&6&586.0&586.0&586.0&586.0&586.0&586.0&586\\
&7&588.0&588.0&588.0&588.0&588.0&588.0&588\\
&8&585.0&585.0&585.0&585.0&585.0&585.0&585\\
&9&588.0&588.0&588.0&588.0&588.0&588.0&588\\
&10&585.0&585.0&585.0&585.0&585.0&585.0&585\\
\midrule
\multirow{10}{*}{700}
&1&681.0&681.0&681.0&681.0&681.0&681.0&681\\
&2&680.0&679.9&680.0&680.0&680.0&680.0&680\\
&3&682.0&682.0&682.0&682.0&682.0&682.0&682\\
&4&685.0&685.0&685.0&685.0&685.0&685.0&685\\
&5&679.0&679.0&679.0&679.0&679.0&678.9&679\\
&6&682.0&682.0&682.0&682.0&682.0&682.0&682\\
&7&679.0&678.9&679.0&679.0&679.0&679.0&679\\
&8&681.0&681.0&681.0&681.0&681.0&681.0&681\\
&9&682.0&682.0&682.0&682.0&682.0&682.0&682\\
&10&681.0&681.0&681.0&681.0&681.0&681.0&681\\
\midrule
\multirow{10}{*}{800}
&1&772.0&772.0&772.0&772.0&772.0&772.0&772\\
&2&767.4&767.4&768.0&767.8&767.9&767.6&768\\
&3&773.0&773.0&773.0&773.0&773.0&773.0&773\\
&4&774.0&774.0&774.0&774.0&774.0&774.0&774\\
&5&772.8&772.9&773.0&773.0&773.0&772.7&773\\
&6&772.0&772.0&772.0&772.0&772.0&772.0&772\\
&7&773.0&773.0&773.0&773.0&773.0&773.0&773\\
&8&775.0&775.0&775.0&775.0&775.0&775.0&775\\
&9&774.0&774.0&774.0&774.0&774.0&774.0&774\\
&10&772.0&772.2&772.3&772.8&773.0&772.6&773\\
\midrule
\multirow{10}{*}{900}
&1&864.8&864.7&865.0&865.0&865.0&864.7&865\\
&2&863.0&863.0&863.0&863.0&863.0&863.0&863\\
&3&865.0&865.1&865.6&865.8&865.9&865.5&866\\
&4&864.1&864.5&864.9&865.0&865.0&864.7&865\\
&5&867.9&867.8&867.8&868.0&868.0&867.9&868\\
&6&868.2&868.4&869.0&869.0&869.0&869.0&869\\
&7&866.0&866.0&866.0&866.0&866.0&866.0&866\\
&8&867.0&867.0&867.0&867.0&867.0&867.0&867\\
&9&864.0&863.9&864.0&864.0&864.0&863.8&864\\
&10&863.6&864.3&864.5&864.1&864.3&864.1&865\\
\midrule
\multirow{10}{*}{1000}
&1&956.0&956.0&956.0&956.0&956.0&955.8&956\\
&2&956.2&956.2&957.0&957.0&957.0&956.2&957\\
&3&961.0&961.0&960.8&961.0&961.0&960.4&961\\
&4&953.9&954.4&954.7&954.5&954.8&954.6&955\\
&5&958.8&958.4&959.0&959.0&959.0&959.0&959\\
&6&960.0&960.0&960.0&960.0&960.0&960.0&960\\
&7&960.0&960.0&960.0&960.0&960.0&960.0&960\\
&8&958.0&958.1&958.4&958.9&959.0&958.8&959\\
&9&960.4&961.7&962.0&962.0&962.0&962.0&962\\
&10&960.6&960.6&961.0&961.0&961.0&961.0&961\\

\midrule
\multicolumn{2}{l}{Aggregate}&772.8&772.9&773.0&773.0&773.0&772.9&773.06\\
\bottomrule
\end{tabular}


==> tables/max2sat140variable.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
&\multicolumn{2}{c}{MCTS}&\multicolumn{2}{c}{MCTS\_H1}&\multicolumn{3}{c}{NMC}&\multicolumn{3}{c}{NMC\_H1}&\multicolumn{3}{c}{NRPA}&\multicolumn{3}{c}{GNRPA}\\
\hline
&m=200&m=1000&m=200&m=1000&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2\\
\hline
s2v140c1200-1&&&&&\makecell[c]{(901.5, 14.4)\\(0.0, 0.0)}&\makecell[c]{(954.8, 8.5)\\(6.4, 0.4)}&\makecell[c]{(991.0, 8.0)\\(616.5, 263.4)}&\makecell[c]{(1012.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1046.0, 0.0)\\(9.3, 2.2)}&\makecell[c]{(1049.0, 0.0)\\(603.8, 230.2)}&\makecell[c]{(896.3, 14.8)\\(0.0, 0.0)}&\makecell[c]{(968.2, 10.2)\\(0.8, 0.5)}&\makecell[c]{(1047.2, 3.9)\\(313.4, 21.7)}&\makecell[c]{(969.2, 12.2)\\(0.0, 0.0)}&\makecell[c]{(1003.4, 7.8)\\(3.4, 1.1)}&\makecell[c]{(1047.7, 3.6)\\(361.8, 24.5)}\\\hline
s2v140c1200-2&&&&&\makecell[c]{(900.8, 15.7)\\(0.0, 0.0)}&\makecell[c]{(952.9, 10.1)\\(6.9, 0.5)}&\makecell[c]{(987.2, 7.6)\\(616.1, 250.0)}&\makecell[c]{(996.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1034.0, 0.0)\\(6.2, 0.4)}&\makecell[c]{(1039.0, 0.0)\\(612.2, 256.1)}&\makecell[c]{(899.8, 14.2)\\(0.0, 0.0)}&\makecell[c]{(964.1, 10.5)\\(1.3, 0.5)}&\makecell[c]{(1037.0, 3.2)\\(322.6, 27.7)}&\makecell[c]{(963.9, 10.0)\\(0.0, 0.0)}&\makecell[c]{(994.7, 6.4)\\(3.5, 1.1)}&\makecell[c]{(1037.5, 3.3)\\(366.6, 27.0)}\\\hline
s2v140c1200-3&&&&&\makecell[c]{(899.4, 12.8)\\(0.0, 0.0)}&\makecell[c]{(950.1, 10.0)\\(6.2, 0.2)}&\makecell[c]{(983.9, 6.3)\\(618.6, 255.5)}&\makecell[c]{(992.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1028.0, 0.0)\\(6.0, 0.4)}&\makecell[c]{(1035.0, 0.0)\\(607.4, 229.2)}&\makecell[c]{(900.0, 12.3)\\(0.0, 0.0)}&\makecell[c]{(962.2, 8.4)\\(1.2, 0.4)}&\makecell[c]{(1034.7, 4.8)\\(311.4, 19.8)}&\makecell[c]{(954.2, 10.5)\\(0.0, 0.0)}&\makecell[c]{(987.0, 8.1)\\(3.3, 1.1)}&\makecell[c]{(1037.2, 4.1)\\(377.4, 46.9)}\\\hline
s2v140c1200-4&&&&&\makecell[c]{(902.1, 14.1)\\(0.0, 0.0)}&\makecell[c]{(953.8, 8.9)\\(6.5, 0.3)}&\makecell[c]{(990.5, 6.2)\\(615.0, 241.5)}&\makecell[c]{(997.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1033.0, 0.0)\\(5.9, 0.2)}&\makecell[c]{(1040.0, 0.0)\\(603.4, 213.8)}&\makecell[c]{(900.3, 15.4)\\(0.0, 0.0)}&\makecell[c]{(965.4, 10.0)\\(1.2, 0.4)}&\makecell[c]{(1042.4, 4.0)\\(328.7, 26.4)}&\makecell[c]{(962.4, 10.4)\\(0.0, 0.0)}&\makecell[c]{(994.5, 6.9)\\(3.0, 0.8)}&\makecell[c]{(1042.8, 3.2)\\(362.3, 25.1)}\\\hline
s2v140c1200-5&&&&&\makecell[c]{(900.5, 16.6)\\(0.0, 0.0)}&\makecell[c]{(960.0, 9.1)\\(6.2, 0.1)}&\makecell[c]{(995.5, 7.5)\\(611.1, 235.9)}&\makecell[c]{(1011.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1045.0, 0.0)\\(5.8, 0.0)}&\makecell[c]{(1054.0, 0.0)\\(602.0, 214.4)}&\makecell[c]{(899.9, 17.5)\\(0.0, 0.0)}&\makecell[c]{(973.2, 10.1)\\(1.1, 0.6)}&\makecell[c]{(1049.9, 3.2)\\(300.9, 14.6)}&\makecell[c]{(977.5, 11.1)\\(0.0, 0.0)}&\makecell[c]{(1008.9, 7.0)\\(3.3, 1.1)}&\makecell[c]{(1051.4, 2.3)\\(374.7, 35.3)}\\\hline
s2v140c1200-6&&&&&\makecell[c]{(899.4, 13.5)\\(0.0, 0.0)}&\makecell[c]{(954.1, 9.7)\\(6.4, 0.4)}&\makecell[c]{(988.3, 6.7)\\(616.1, 268.4)}&\makecell[c]{(996.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1037.0, 0.0)\\(6.2, 0.4)}&\makecell[c]{(1042.0, 0.0)\\(605.0, 215.4)}&\makecell[c]{(899.7, 15.1)\\(0.0, 0.0)}&\makecell[c]{(966.4, 9.9)\\(1.3, 0.5)}&\makecell[c]{(1042.6, 4.3)\\(314.1, 42.0)}&\makecell[c]{(966.2, 10.2)\\(0.0, 0.0)}&\makecell[c]{(996.0, 7.0)\\(2.9, 0.8)}&\makecell[c]{(1043.5, 3.8)\\(377.7, 37.1)}\\\hline
s2v140c1200-7&&&&&\makecell[c]{(900.4, 16.0)\\(0.0, 0.0)}&\makecell[c]{(956.4, 9.8)\\(6.2, 0.1)}&\makecell[c]{(991.2, 7.1)\\(619.5, 281.0)}&\makecell[c]{(1002.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1037.0, 0.0)\\(6.7, 0.5)}&\makecell[c]{(1046.0, 0.0)\\(605.2, 225.1)}&\makecell[c]{(899.3, 17.7)\\(0.0, 0.0)}&\makecell[c]{(968.2, 10.7)\\(1.0, 0.5)}&\makecell[c]{(1043.1, 2.9)\\(328.3, 37.1)}&\makecell[c]{(968.4, 9.8)\\(0.0, 0.0)}&\makecell[c]{(999.6, 6.4)\\(3.3, 1.1)}&\makecell[c]{(1043.6, 3.1)\\(375.0, 62.7)}\\\hline
s2v140c1200-8&&&&&\makecell[c]{(900.1, 14.0)\\(0.0, 0.0)}&\makecell[c]{(952.9, 9.5)\\(6.2, 0.2)}&\makecell[c]{(986.5, 7.3)\\(619.6, 274.1)}&\makecell[c]{(992.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1034.0, 0.0)\\(6.7, 0.5)}&\makecell[c]{(1041.0, 0.0)\\(604.2, 236.4)}&\makecell[c]{(900.7, 15.2)\\(0.0, 0.0)}&\makecell[c]{(965.4, 9.1)\\(1.4, 0.6)}&\makecell[c]{(1039.5, 2.9)\\(314.5, 26.6)}&\makecell[c]{(959.9, 10.0)\\(0.0, 0.0)}&\makecell[c]{(992.4, 7.5)\\(3.0, 0.8)}&\makecell[c]{(1040.2, 3.1)\\(367.8, 28.7)}\\\hline
s2v140c1200-9&&&&&\makecell[c]{(901.3, 13.4)\\(0.0, 0.0)}&\makecell[c]{(952.8, 11.0)\\(6.5, 0.4)}&\makecell[c]{(984.2, 7.1)\\(613.5, 243.6)}&\makecell[c]{(999.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1039.0, 0.0)\\(6.4, 0.5)}&\makecell[c]{(1046.0, 0.0)\\(603.7, 216.8)}&\makecell[c]{(898.6, 15.2)\\(0.0, 0.0)}&\makecell[c]{(965.0, 9.2)\\(1.3, 0.4)}&\makecell[c]{(1043.2, 3.1)\\(337.5, 19.9)}&\makecell[c]{(958.0, 10.9)\\(0.0, 0.0)}&\makecell[c]{(991.9, 7.5)\\(3.4, 1.1)}&\makecell[c]{(1043.9, 2.8)\\(393.5, 71.6)}\\\hline
s2v140c1200-10&&&&&\makecell[c]{(898.6, 16.6)\\(0.0, 0.0)}&\makecell[c]{(954.7, 9.4)\\(6.4, 0.2)}&\makecell[c]{(992.1, 7.3)\\(612.8, 233.5)}&\makecell[c]{(1009.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1048.0, 0.0)\\(5.9, 0.1)}&\makecell[c]{(1052.0, 0.0)\\(610.4, 250.8)}&\makecell[c]{(900.4, 14.2)\\(0.0, 0.0)}&\makecell[c]{(969.0, 9.9)\\(1.0, 0.5)}&\makecell[c]{(1053.7, 3.7)\\(310.6, 19.4)}&\makecell[c]{(967.5, 11.2)\\(0.0, 0.0)}&\makecell[c]{(1002.1, 6.9)\\(3.4, 1.1)}&\makecell[c]{(1054.4, 3.1)\\(364.0, 29.8)}\\\hline
s2v140c1300-1&&&&&\makecell[c]{(973.7, 15.8)\\(0.0, 0.0)}&\makecell[c]{(1033.3, 10.9)\\(6.6, 0.1)}&\makecell[c]{(1070.9, 7.0)\\(633.1, 313.5)}&\makecell[c]{(1093.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1124.0, 0.0)\\(6.8, 0.2)}&\makecell[c]{(1132.0, 0.0)\\(622.9, 252.1)}&\makecell[c]{(971.5, 15.4)\\(0.0, 0.0)}&\makecell[c]{(1046.1, 11.5)\\(1.3, 0.6)}&\makecell[c]{(1129.7, 3.3)\\(333.2, 26.5)}&\makecell[c]{(1047.0, 12.7)\\(0.0, 0.0)}&\makecell[c]{(1081.5, 8.5)\\(3.6, 1.1)}&\makecell[c]{(1130.7, 3.0)\\(384.1, 41.3)}\\\hline
s2v140c1300-2&&&&&\makecell[c]{(974.7, 15.7)\\(0.0, 0.0)}&\makecell[c]{(1032.3, 10.8)\\(6.9, 0.2)}&\makecell[c]{(1066.4, 7.8)\\(642.8, 439.9)}&\makecell[c]{(1085.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1111.0, 0.0)\\(6.8, 0.5)}&\makecell[c]{(1122.0, 0.0)\\(624.1, 300.6)}&\makecell[c]{(974.1, 16.9)\\(0.0, 0.0)}&\makecell[c]{(1044.3, 9.1)\\(1.0, 0.5)}&\makecell[c]{(1121.4, 3.5)\\(335.4, 24.6)}&\makecell[c]{(1041.3, 13.2)\\(0.0, 0.0)}&\makecell[c]{(1073.5, 6.9)\\(3.6, 1.1)}&\makecell[c]{(1122.3, 3.3)\\(400.7, 59.5)}\\\hline
s2v140c1300-3&&&&&\makecell[c]{(974.1, 14.8)\\(0.0, 0.0)}&\makecell[c]{(1030.7, 9.7)\\(7.2, 0.7)}&\makecell[c]{(1067.2, 8.0)\\(627.5, 287.1)}&\makecell[c]{(1072.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1117.0, 0.0)\\(6.6, 0.0)}&\makecell[c]{(1124.0, 0.0)\\(626.5, 276.7)}&\makecell[c]{(975.1, 14.8)\\(0.0, 0.0)}&\makecell[c]{(1041.6, 9.3)\\(1.6, 0.8)}&\makecell[c]{(1124.8, 3.5)\\(330.0, 25.8)}&\makecell[c]{(1034.5, 11.9)\\(0.0, 0.0)}&\makecell[c]{(1073.7, 9.0)\\(3.1, 0.9)}&\makecell[c]{(1125.5, 2.5)\\(388.1, 48.5)}\\\hline
s2v140c1300-4&&&&&\makecell[c]{(972.9, 13.9)\\(0.0, 0.0)}&\makecell[c]{(1030.2, 9.7)\\(6.9, 0.3)}&\makecell[c]{(1069.0, 8.0)\\(630.4, 272.3)}&\makecell[c]{(1092.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1126.0, 0.0)\\(6.4, 0.1)}&\makecell[c]{(1133.0, 0.0)\\(625.7, 287.8)}&\makecell[c]{(974.6, 17.0)\\(0.0, 0.0)}&\makecell[c]{(1044.5, 10.7)\\(1.6, 0.7)}&\makecell[c]{(1127.8, 4.0)\\(348.3, 77.5)}&\makecell[c]{(1039.4, 11.5)\\(0.0, 0.0)}&\makecell[c]{(1074.9, 9.2)\\(3.2, 0.9)}&\makecell[c]{(1128.8, 4.1)\\(385.3, 38.6)}\\\hline
s2v140c1300-5&&&&&\makecell[c]{(975.6, 15.0)\\(0.0, 0.0)}&\makecell[c]{(1030.0, 10.4)\\(6.8, 0.1)}&\makecell[c]{(1068.1, 8.0)\\(628.3, 282.8)}&\makecell[c]{(1075.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1116.0, 0.0)\\(7.9, 0.1)}&\makecell[c]{(1122.0, 0.0)\\(627.3, 299.9)}&\makecell[c]{(974.2, 15.9)\\(0.0, 0.0)}&\makecell[c]{(1043.5, 10.0)\\(1.3, 0.5)}&\makecell[c]{(1122.9, 2.9)\\(342.9, 30.1)}&\makecell[c]{(1041.3, 12.8)\\(0.0, 0.0)}&\makecell[c]{(1075.7, 9.1)\\(3.1, 0.9)}&\makecell[c]{(1123.8, 2.5)\\(397.9, 102.6)}\\\hline
s2v140c1300-6&&&&&\makecell[c]{(975.8, 12.1)\\(0.0, 0.0)}&\makecell[c]{(1031.1, 11.8)\\(6.9, 0.4)}&\makecell[c]{(1064.0, 7.6)\\(627.8, 275.6)}&\makecell[c]{(1077.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1115.0, 0.0)\\(6.5, 0.3)}&\makecell[c]{(1125.0, 0.0)\\(624.8, 292.6)}&\makecell[c]{(974.7, 15.8)\\(0.0, 0.0)}&\makecell[c]{(1044.4, 9.9)\\(2.2, 1.0)}&\makecell[c]{(1124.6, 3.7)\\(347.9, 26.0)}&\makecell[c]{(1035.6, 11.4)\\(0.0, 0.0)}&\makecell[c]{(1072.5, 8.3)\\(3.2, 0.9)}&\makecell[c]{(1125.8, 2.9)\\(379.5, 35.0)}\\\hline
s2v140c1300-7&&&&&\makecell[c]{(975.4, 15.2)\\(0.0, 0.0)}&\makecell[c]{(1029.3, 10.2)\\(6.8, 0.1)}&\makecell[c]{(1071.5, 8.5)\\(627.2, 265.4)}&\makecell[c]{(1083.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1126.0, 0.0)\\(6.6, 0.0)}&\makecell[c]{(1137.0, 0.0)\\(623.6, 278.1)}&\makecell[c]{(973.5, 16.2)\\(0.0, 0.0)}&\makecell[c]{(1047.7, 10.5)\\(1.2, 0.5)}&\makecell[c]{(1133.5, 3.3)\\(332.8, 24.4)}&\makecell[c]{(1043.0, 11.7)\\(0.0, 0.0)}&\makecell[c]{(1079.4, 8.5)\\(3.6, 1.1)}&\makecell[c]{(1134.3, 3.3)\\(387.3, 42.0)}\\\hline
s2v140c1300-8&&&&&\makecell[c]{(976.3, 15.1)\\(0.0, 0.0)}&\makecell[c]{(1032.3, 10.1)\\(7.5, 0.5)}&\makecell[c]{(1071.3, 7.5)\\(632.6, 304.8)}&\makecell[c]{(1087.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1132.0, 0.0)\\(6.5, 0.2)}&\makecell[c]{(1135.0, 0.0)\\(625.0, 263.5)}&\makecell[c]{(979.0, 16.9)\\(0.0, 0.0)}&\makecell[c]{(1047.8, 10.7)\\(1.2, 0.5)}&\makecell[c]{(1137.3, 3.6)\\(336.0, 28.1)}&\makecell[c]{(1044.3, 11.8)\\(0.0, 0.0)}&\makecell[c]{(1080.3, 8.6)\\(3.1, 0.9)}&\makecell[c]{(1137.3, 3.9)\\(381.1, 53.9)}\\\hline
s2v140c1300-9&&&&&\makecell[c]{(972.3, 15.9)\\(0.0, 0.0)}&\makecell[c]{(1032.9, 12.2)\\(6.9, 0.3)}&\makecell[c]{(1071.2, 8.4)\\(629.6, 289.6)}&\makecell[c]{(1090.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1130.0, 0.0)\\(7.6, 0.1)}&\makecell[c]{(1131.0, 0.0)\\(620.6, 258.2)}&\makecell[c]{(975.6, 17.7)\\(0.0, 0.0)}&\makecell[c]{(1046.7, 11.1)\\(1.4, 0.7)}&\makecell[c]{(1130.1, 3.6)\\(332.5, 19.9)}&\makecell[c]{(1042.3, 10.5)\\(0.0, 0.0)}&\makecell[c]{(1079.8, 8.3)\\(3.6, 1.1)}&\makecell[c]{(1131.9, 2.2)\\(392.3, 69.4)}\\\hline
s2v140c1300-10&&&&&\makecell[c]{(977.3, 15.3)\\(0.0, 0.0)}&\makecell[c]{(1029.9, 9.5)\\(8.8, 3.2)}&\makecell[c]{(1066.2, 6.7)\\(630.9, 303.3)}&\makecell[c]{(1100.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1124.0, 0.0)\\(7.3, 0.6)}&\makecell[c]{(1126.0, 0.0)\\(630.4, 297.8)}&\makecell[c]{(976.6, 16.2)\\(0.0, 0.0)}&\makecell[c]{(1044.1, 9.6)\\(1.4, 0.7)}&\makecell[c]{(1120.2, 3.6)\\(325.0, 18.7)}&\makecell[c]{(1041.9, 11.6)\\(0.0, 0.0)}&\makecell[c]{(1074.5, 7.6)\\(3.3, 0.9)}&\makecell[c]{(1121.2, 3.2)\\(396.2, 83.8)}\\\hline
s2v140c1400-1&&&&&\makecell[c]{(1053.4, 16.0)\\(0.0, 0.0)}&\makecell[c]{(1109.1, 10.8)\\(8.1, 0.7)}&\makecell[c]{(1147.9, 7.7)\\(641.6, 326.7)}&\makecell[c]{(1167.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1202.0, 0.0)\\(8.1, 0.5)}&\makecell[c]{(1212.0, 0.0)\\(643.6, 426.9)}&\makecell[c]{(1047.9, 15.4)\\(0.0, 0.0)}&\makecell[c]{(1123.2, 11.2)\\(1.2, 0.5)}&\makecell[c]{(1209.2, 4.3)\\(346.2, 22.5)}&\makecell[c]{(1118.2, 14.3)\\(0.0, 0.0)}&\makecell[c]{(1156.5, 9.4)\\(3.8, 1.2)}&\makecell[c]{(1210.5, 3.3)\\(411.6, 68.0)}\\\hline
s2v140c1400-2&&&&&\makecell[c]{(1050.0, 16.8)\\(0.0, 0.0)}&\makecell[c]{(1110.3, 10.8)\\(7.3, 0.2)}&\makecell[c]{(1148.7, 8.3)\\(641.4, 321.1)}&\makecell[c]{(1178.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1205.0, 0.0)\\(12.1, 0.8)}&\makecell[c]{(1209.0, 0.0)\\(632.1, 333.0)}&\makecell[c]{(1049.2, 16.5)\\(0.0, 0.0)}&\makecell[c]{(1124.8, 11.2)\\(1.1, 0.5)}&\makecell[c]{(1212.6, 5.1)\\(349.0, 23.1)}&\makecell[c]{(1124.5, 14.2)\\(0.0, 0.0)}&\makecell[c]{(1160.5, 8.7)\\(3.4, 0.9)}&\makecell[c]{(1212.6, 5.3)\\(405.9, 63.6)}\\\hline
s2v140c1400-3&&&&&\makecell[c]{(1049.7, 15.9)\\(0.0, 0.0)}&\makecell[c]{(1102.7, 8.4)\\(7.3, 0.1)}&\makecell[c]{(1139.7, 7.1)\\(647.9, 369.0)}&\makecell[c]{(1150.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1189.0, 0.0)\\(8.5, 0.1)}&\makecell[c]{(1206.0, 0.0)\\(637.3, 308.9)}&\makecell[c]{(1050.2, 17.0)\\(0.0, 0.0)}&\makecell[c]{(1117.7, 9.8)\\(1.2, 0.6)}&\makecell[c]{(1198.1, 5.1)\\(363.7, 58.2)}&\makecell[c]{(1104.7, 11.4)\\(0.0, 0.0)}&\makecell[c]{(1143.3, 7.3)\\(5.4, 2.5)}&\makecell[c]{(1199.9, 4.1)\\(394.1, 50.0)}\\\hline
s2v140c1400-4&&&&&\makecell[c]{(1048.5, 17.5)\\(0.0, 0.0)}&\makecell[c]{(1107.2, 10.4)\\(8.1, 0.7)}&\makecell[c]{(1146.5, 8.4)\\(650.6, 450.4)}&\makecell[c]{(1166.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1197.0, 0.0)\\(7.2, 0.1)}&\makecell[c]{(1211.0, 0.0)\\(635.3, 292.8)}&\makecell[c]{(1048.0, 16.1)\\(0.0, 0.0)}&\makecell[c]{(1122.2, 10.6)\\(1.7, 0.8)}&\makecell[c]{(1208.7, 4.9)\\(358.4, 28.6)}&\makecell[c]{(1116.0, 11.1)\\(0.0, 0.0)}&\makecell[c]{(1150.7, 8.7)\\(3.5, 1.1)}&\makecell[c]{(1210.4, 4.5)\\(394.6, 45.3)}\\\hline
s2v140c1400-5&&&&&\makecell[c]{(1051.5, 16.5)\\(0.0, 0.0)}&\makecell[c]{(1105.8, 10.6)\\(8.0, 0.6)}&\makecell[c]{(1145.1, 7.3)\\(642.4, 321.6)}&\makecell[c]{(1162.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1195.0, 0.0)\\(7.7, 0.5)}&\makecell[c]{(1208.0, 0.0)\\(634.2, 290.0)}&\makecell[c]{(1048.5, 15.6)\\(0.0, 0.0)}&\makecell[c]{(1118.0, 11.8)\\(1.5, 0.7)}&\makecell[c]{(1205.0, 4.1)\\(353.7, 27.6)}&\makecell[c]{(1109.9, 13.2)\\(0.0, 0.0)}&\makecell[c]{(1148.4, 7.0)\\(3.3, 0.9)}&\makecell[c]{(1205.1, 4.6)\\(406.0, 63.4)}\\\hline
s2v140c1400-6&&&&&\makecell[c]{(1050.5, 18.3)\\(0.0, 0.0)}&\makecell[c]{(1107.9, 11.1)\\(8.5, 0.2)}&\makecell[c]{(1146.0, 7.4)\\(639.4, 315.2)}&\makecell[c]{(1156.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1200.0, 0.0)\\(8.5, 0.1)}&\makecell[c]{(1204.0, 0.0)\\(637.2, 338.7)}&\makecell[c]{(1050.2, 17.9)\\(0.0, 0.0)}&\makecell[c]{(1121.4, 10.0)\\(1.5, 0.8)}&\makecell[c]{(1205.6, 3.1)\\(352.6, 26.9)}&\makecell[c]{(1116.9, 12.7)\\(0.0, 0.0)}&\makecell[c]{(1153.2, 7.5)\\(3.4, 0.8)}&\makecell[c]{(1206.0, 2.8)\\(387.6, 33.9)}\\\hline
s2v140c1400-7&&&&&\makecell[c]{(1052.4, 17.1)\\(0.0, 0.0)}&\makecell[c]{(1105.9, 10.1)\\(8.3, 0.6)}&\makecell[c]{(1143.5, 8.9)\\(643.1, 336.4)}&\makecell[c]{(1155.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1194.0, 0.0)\\(7.3, 0.5)}&\makecell[c]{(1208.0, 0.0)\\(633.7, 289.8)}&\makecell[c]{(1052.0, 15.1)\\(0.0, 0.0)}&\makecell[c]{(1122.5, 10.9)\\(1.8, 1.0)}&\makecell[c]{(1202.4, 4.1)\\(344.6, 17.6)}&\makecell[c]{(1112.8, 12.2)\\(0.0, 0.0)}&\makecell[c]{(1150.2, 8.7)\\(3.4, 0.9)}&\makecell[c]{(1203.9, 4.0)\\(411.1, 76.5)}\\\hline
s2v140c1400-8&&&&&\makecell[c]{(1050.6, 15.1)\\(0.0, 0.0)}&\makecell[c]{(1109.7, 11.5)\\(8.6, 0.1)}&\makecell[c]{(1147.7, 8.4)\\(644.9, 363.2)}&\makecell[c]{(1184.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1210.0, 0.0)\\(7.2, 0.5)}&\makecell[c]{(1212.0, 0.0)\\(639.8, 335.1)}&\makecell[c]{(1048.4, 15.8)\\(0.0, 0.0)}&\makecell[c]{(1123.6, 11.2)\\(1.7, 0.8)}&\makecell[c]{(1211.1, 4.4)\\(342.3, 19.8)}&\makecell[c]{(1123.4, 13.5)\\(0.0, 0.0)}&\makecell[c]{(1158.4, 8.8)\\(3.7, 1.1)}&\makecell[c]{(1211.5, 3.3)\\(395.8, 48.3)}\\\hline
s2v140c1400-9&&&&&\makecell[c]{(1049.5, 17.6)\\(0.0, 0.0)}&\makecell[c]{(1106.8, 10.0)\\(8.8, 0.1)}&\makecell[c]{(1145.5, 8.0)\\(644.6, 360.7)}&\makecell[c]{(1156.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1201.0, 0.0)\\(11.5, 2.8)}&\makecell[c]{(1211.0, 0.0)\\(630.1, 287.7)}&\makecell[c]{(1049.6, 16.2)\\(0.0, 0.0)}&\makecell[c]{(1123.2, 10.5)\\(1.4, 0.7)}&\makecell[c]{(1207.3, 3.8)\\(352.0, 32.7)}&\makecell[c]{(1116.7, 12.0)\\(0.0, 0.0)}&\makecell[c]{(1152.7, 9.1)\\(3.3, 0.9)}&\makecell[c]{(1207.9, 3.5)\\(396.5, 47.7)}\\\hline
s2v140c1400-10&&&&&\makecell[c]{(1050.3, 14.6)\\(0.0, 0.0)}&\makecell[c]{(1104.2, 11.2)\\(7.4, 0.4)}&\makecell[c]{(1144.5, 7.9)\\(640.3, 313.3)}&\makecell[c]{(1159.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1196.0, 0.0)\\(8.3, 0.1)}&\makecell[c]{(1203.0, 0.0)\\(635.2, 306.7)}&\makecell[c]{(1052.4, 17.3)\\(0.0, 0.0)}&\makecell[c]{(1120.5, 9.9)\\(1.3, 0.6)}&\makecell[c]{(1199.1, 4.3)\\(385.2, 104.9)}&\makecell[c]{(1105.5, 12.8)\\(0.0, 0.0)}&\makecell[c]{(1146.6, 9.1)\\(3.3, 0.9)}&\makecell[c]{(1201.0, 4.1)\\(404.1, 59.2)}\\\hline
s2v140c1500-1&&&&&\makecell[c]{(1126.2, 15.2)\\(0.0, 0.0)}&\makecell[c]{(1184.4, 10.5)\\(9.4, 0.1)}&\makecell[c]{(1224.8, 8.3)\\(661.4, 515.2)}&\makecell[c]{(1244.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1283.0, 0.0)\\(7.6, 0.1)}&\makecell[c]{(1286.0, 0.0)\\(649.6, 351.6)}&\makecell[c]{(1124.9, 17.7)\\(0.0, 0.0)}&\makecell[c]{(1201.3, 11.1)\\(1.8, 0.9)}&\makecell[c]{(1289.0, 3.1)\\(372.2, 41.3)}&\makecell[c]{(1191.3, 12.9)\\(0.0, 0.0)}&\makecell[c]{(1232.5, 7.5)\\(3.5, 0.9)}&\makecell[c]{(1289.7, 2.8)\\(406.8, 59.0)}\\\hline
s2v140c1500-2&&&&&\makecell[c]{(1125.6, 17.1)\\(0.0, 0.0)}&\makecell[c]{(1188.1, 10.7)\\(7.8, 0.1)}&\makecell[c]{(1232.4, 8.5)\\(649.7, 344.8)}&\makecell[c]{(1267.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1290.0, 0.0)\\(8.1, 0.6)}&\makecell[c]{(1298.0, 0.0)\\(647.3, 357.4)}&\makecell[c]{(1125.7, 18.0)\\(0.0, 0.0)}&\makecell[c]{(1203.7, 12.5)\\(1.3, 0.7)}&\makecell[c]{(1293.4, 3.5)\\(372.7, 42.5)}&\makecell[c]{(1202.9, 13.1)\\(0.0, 0.0)}&\makecell[c]{(1243.3, 8.8)\\(3.5, 0.8)}&\makecell[c]{(1294.7, 2.7)\\(407.2, 61.8)}\\\hline
s2v140c1500-3&&&&&\makecell[c]{(1128.7, 15.2)\\(0.0, 0.0)}&\makecell[c]{(1181.5, 9.4)\\(8.4, 0.7)}&\makecell[c]{(1221.8, 8.7)\\(651.3, 371.1)}&\makecell[c]{(1212.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1271.0, 0.0)\\(8.9, 0.1)}&\makecell[c]{(1279.0, 0.0)\\(649.6, 367.1)}&\makecell[c]{(1128.8, 15.9)\\(0.0, 0.0)}&\makecell[c]{(1194.9, 11.0)\\(1.4, 0.8)}&\makecell[c]{(1279.8, 3.3)\\(382.4, 41.9)}&\makecell[c]{(1182.5, 12.6)\\(0.0, 0.0)}&\makecell[c]{(1223.3, 7.8)\\(3.6, 0.9)}&\makecell[c]{(1280.5, 3.3)\\(409.7, 60.8)}\\\hline
s2v140c1500-4&&&&&\makecell[c]{(1126.8, 16.4)\\(0.0, 0.0)}&\makecell[c]{(1188.7, 13.2)\\(7.9, 0.3)}&\makecell[c]{(1230.2, 9.1)\\(658.0, 484.8)}&\makecell[c]{(1261.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1285.0, 0.0)\\(7.5, 0.2)}&\makecell[c]{(1293.0, 0.0)\\(657.6, 343.4)}&\makecell[c]{(1125.4, 17.2)\\(0.0, 0.0)}&\makecell[c]{(1205.0, 12.6)\\(1.9, 0.9)}&\makecell[c]{(1294.6, 4.8)\\(388.8, 78.5)}&\makecell[c]{(1202.0, 15.0)\\(0.0, 0.0)}&\makecell[c]{(1239.0, 9.1)\\(3.5, 0.9)}&\makecell[c]{(1295.3, 4.7)\\(411.5, 69.9)}\\\hline
s2v140c1500-5&&&&&\makecell[c]{(1123.4, 16.8)\\(0.0, 0.0)}&\makecell[c]{(1185.3, 11.8)\\(8.0, 0.4)}&\makecell[c]{(1224.7, 8.2)\\(651.6, 348.2)}&\makecell[c]{(1243.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1280.0, 0.0)\\(7.6, 0.3)}&\makecell[c]{(1291.0, 0.0)\\(644.1, 327.1)}&\makecell[c]{(1126.0, 15.7)\\(0.0, 0.0)}&\makecell[c]{(1198.8, 10.3)\\(1.1, 0.6)}&\makecell[c]{(1286.4, 3.5)\\(359.6, 20.8)}&\makecell[c]{(1189.3, 12.9)\\(0.0, 0.0)}&\makecell[c]{(1232.9, 9.3)\\(3.4, 0.9)}&\makecell[c]{(1287.5, 2.6)\\(400.5, 46.9)}\\\hline
s2v140c1500-6&&&&&\makecell[c]{(1123.2, 15.9)\\(0.0, 0.0)}&\makecell[c]{(1188.9, 11.3)\\(7.7, 0.1)}&\makecell[c]{(1226.2, 9.5)\\(652.8, 354.0)}&\makecell[c]{(1256.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1287.0, 0.0)\\(7.4, 0.2)}&\makecell[c]{(1297.0, 0.0)\\(648.1, 331.8)}&\makecell[c]{(1124.6, 17.2)\\(0.0, 0.0)}&\makecell[c]{(1200.2, 12.7)\\(1.8, 1.0)}&\makecell[c]{(1294.1, 3.9)\\(355.1, 18.7)}&\makecell[c]{(1198.4, 12.8)\\(0.0, 0.0)}&\makecell[c]{(1238.5, 9.8)\\(3.7, 1.0)}&\makecell[c]{(1294.8, 3.3)\\(416.2, 89.0)}\\\hline
s2v140c1500-7&&&&&\makecell[c]{(1123.5, 16.9)\\(0.0, 0.0)}&\makecell[c]{(1186.6, 11.7)\\(7.7, 0.1)}&\makecell[c]{(1225.4, 8.7)\\(653.5, 367.1)}&\makecell[c]{(1239.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1282.0, 0.0)\\(8.6, 0.6)}&\makecell[c]{(1291.0, 0.0)\\(646.4, 337.1)}&\makecell[c]{(1125.3, 18.4)\\(0.0, 0.0)}&\makecell[c]{(1200.8, 12.0)\\(1.8, 1.0)}&\makecell[c]{(1289.7, 3.8)\\(378.9, 39.6)}&\makecell[c]{(1199.9, 13.3)\\(0.0, 0.0)}&\makecell[c]{(1236.8, 7.7)\\(5.8, 2.4)}&\makecell[c]{(1290.6, 3.5)\\(412.6, 82.0)}\\\hline
s2v140c1500-8&&&&&\makecell[c]{(1126.7, 17.2)\\(0.0, 0.0)}&\makecell[c]{(1188.0, 12.6)\\(9.0, 0.4)}&\makecell[c]{(1227.9, 8.3)\\(649.6, 347.2)}&\makecell[c]{(1244.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1283.0, 0.0)\\(9.0, 0.1)}&\makecell[c]{(1290.0, 0.0)\\(651.3, 379.4)}&\makecell[c]{(1125.5, 17.7)\\(0.0, 0.0)}&\makecell[c]{(1203.0, 11.4)\\(1.4, 0.8)}&\makecell[c]{(1292.1, 4.6)\\(364.0, 28.6)}&\makecell[c]{(1198.7, 14.5)\\(0.0, 0.0)}&\makecell[c]{(1236.5, 8.6)\\(3.6, 0.9)}&\makecell[c]{(1291.5, 4.8)\\(417.9, 76.4)}\\\hline
s2v140c1500-9&&&&&\makecell[c]{(1127.2, 15.0)\\(0.0, 0.0)}&\makecell[c]{(1185.5, 8.5)\\(11.0, 2.4)}&\makecell[c]{(1226.9, 8.7)\\(649.7, 354.1)}&\makecell[c]{(1265.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1293.0, 0.0)\\(8.3, 0.7)}&\makecell[c]{(1298.0, 0.0)\\(651.0, 378.8)}&\makecell[c]{(1129.2, 17.3)\\(0.0, 0.0)}&\makecell[c]{(1200.4, 10.9)\\(1.3, 0.7)}&\makecell[c]{(1294.7, 3.0)\\(358.5, 19.4)}&\makecell[c]{(1195.5, 13.9)\\(0.0, 0.0)}&\makecell[c]{(1236.0, 8.2)\\(5.6, 2.5)}&\makecell[c]{(1295.9, 3.1)\\(402.1, 48.8)}\\\hline
s2v140c1500-10&&&&&\makecell[c]{(1124.3, 20.1)\\(0.0, 0.0)}&\makecell[c]{(1190.7, 13.0)\\(8.0, 0.4)}&\makecell[c]{(1230.3, 8.9)\\(652.4, 356.0)}&\makecell[c]{(1259.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1285.0, 0.0)\\(7.5, 0.1)}&\makecell[c]{(1294.0, 0.0)\\(649.6, 373.5)}&\makecell[c]{(1123.7, 19.1)\\(0.0, 0.0)}&\makecell[c]{(1202.6, 12.1)\\(2.0, 1.1)}&\makecell[c]{(1290.7, 3.4)\\(379.1, 67.7)}&\makecell[c]{(1199.4, 13.4)\\(0.0, 0.0)}&\makecell[c]{(1237.5, 9.4)\\(3.8, 0.8)}&\makecell[c]{(1291.6, 2.4)\\(413.1, 64.8)}\\\hline
s2v140c1600-1&&&&&\makecell[c]{(1201.4, 16.3)\\(0.0, 0.0)}&\makecell[c]{(1261.1, 11.0)\\(9.3, 0.7)}&\makecell[c]{(1302.5, 7.9)\\(661.1, 396.9)}&\makecell[c]{(1323.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1358.0, 0.0)\\(8.1, 0.1)}&\makecell[c]{(1376.0, 0.0)\\(657.4, 374.6)}&\makecell[c]{(1199.1, 14.8)\\(0.0, 0.0)}&\makecell[c]{(1276.8, 11.8)\\(1.7, 1.0)}&\makecell[c]{(1372.1, 3.7)\\(373.6, 23.3)}&\makecell[c]{(1267.7, 13.8)\\(0.0, 0.0)}&\makecell[c]{(1309.8, 11.1)\\(4.1, 1.1)}&\makecell[c]{(1372.7, 3.3)\\(409.7, 53.5)}\\\hline
s2v140c1600-2&&&&&\makecell[c]{(1200.3, 17.5)\\(0.0, 0.0)}&\makecell[c]{(1262.0, 10.8)\\(8.3, 0.2)}&\makecell[c]{(1305.2, 9.1)\\(659.1, 372.7)}&\makecell[c]{(1345.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1372.0, 0.0)\\(8.0, 0.3)}&\makecell[c]{(1376.0, 0.0)\\(653.6, 358.6)}&\makecell[c]{(1202.9, 15.8)\\(0.0, 0.0)}&\makecell[c]{(1278.2, 12.5)\\(2.1, 1.0)}&\makecell[c]{(1370.9, 4.5)\\(383.6, 36.5)}&\makecell[c]{(1268.4, 13.9)\\(0.0, 0.0)}&\makecell[c]{(1311.7, 9.4)\\(3.7, 0.9)}&\makecell[c]{(1372.1, 3.7)\\(413.4, 62.7)}\\\hline
s2v140c1600-3&&&&&\makecell[c]{(1198.3, 18.5)\\(0.0, 0.0)}&\makecell[c]{(1262.3, 11.9)\\(9.3, 0.8)}&\makecell[c]{(1301.4, 7.2)\\(661.5, 377.4)}&\makecell[c]{(1306.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1347.0, 0.0)\\(8.6, 0.7)}&\makecell[c]{(1366.0, 0.0)\\(659.1, 378.9)}&\makecell[c]{(1199.2, 16.9)\\(0.0, 0.0)}&\makecell[c]{(1275.6, 11.3)\\(2.0, 1.1)}&\makecell[c]{(1363.5, 3.9)\\(372.6, 25.1)}&\makecell[c]{(1265.0, 13.7)\\(0.0, 0.0)}&\makecell[c]{(1305.9, 8.8)\\(3.8, 0.9)}&\makecell[c]{(1364.2, 3.9)\\(421.7, 79.0)}\\\hline
s2v140c1600-4&&&&&\makecell[c]{(1203.4, 17.2)\\(0.0, 0.0)}&\makecell[c]{(1266.0, 11.7)\\(9.5, 0.4)}&\makecell[c]{(1306.3, 8.9)\\(659.2, 373.9)}&\makecell[c]{(1327.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1363.0, 0.0)\\(10.4, 3.2)}&\makecell[c]{(1368.0, 0.0)\\(651.5, 371.8)}&\makecell[c]{(1201.0, 18.7)\\(0.0, 0.0)}&\makecell[c]{(1279.1, 10.9)\\(2.2, 1.2)}&\makecell[c]{(1368.9, 4.6)\\(372.3, 29.4)}&\makecell[c]{(1273.6, 12.8)\\(0.0, 0.0)}&\makecell[c]{(1313.5, 8.2)\\(3.7, 0.8)}&\makecell[c]{(1369.4, 3.4)\\(411.7, 52.9)}\\\hline
s2v140c1600-5&&&&&\makecell[c]{(1198.9, 15.9)\\(0.0, 0.0)}&\makecell[c]{(1261.4, 11.1)\\(8.3, 0.2)}&\makecell[c]{(1300.1, 8.5)\\(661.1, 393.1)}&\makecell[c]{(1307.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1357.0, 0.0)\\(8.8, 0.7)}&\makecell[c]{(1363.0, 0.0)\\(653.4, 355.3)}&\makecell[c]{(1198.9, 14.0)\\(0.0, 0.0)}&\makecell[c]{(1277.7, 11.6)\\(1.7, 1.1)}&\makecell[c]{(1362.4, 4.3)\\(389.1, 43.6)}&\makecell[c]{(1259.9, 14.0)\\(0.0, 0.0)}&\makecell[c]{(1303.8, 8.5)\\(3.7, 1.0)}&\makecell[c]{(1363.5, 3.7)\\(414.2, 62.7)}\\\hline
s2v140c1600-6&&&&&\makecell[c]{(1200.4, 17.7)\\(0.0, 0.0)}&\makecell[c]{(1265.5, 11.6)\\(9.4, 0.5)}&\makecell[c]{(1304.6, 8.5)\\(671.3, 514.5)}&\makecell[c]{(1319.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1360.0, 0.0)\\(8.0, 0.5)}&\makecell[c]{(1366.0, 0.0)\\(660.5, 403.0)}&\makecell[c]{(1197.9, 19.7)\\(0.0, 0.0)}&\makecell[c]{(1280.3, 10.7)\\(1.7, 1.0)}&\makecell[c]{(1370.8, 4.7)\\(374.5, 32.1)}&\makecell[c]{(1266.7, 12.7)\\(0.0, 0.0)}&\makecell[c]{(1309.5, 8.9)\\(4.1, 1.3)}&\makecell[c]{(1372.6, 4.0)\\(417.1, 74.3)}\\\hline
s2v140c1600-7&&&&&\makecell[c]{(1198.4, 19.1)\\(0.0, 0.0)}&\makecell[c]{(1262.1, 12.6)\\(8.3, 0.1)}&\makecell[c]{(1304.7, 8.5)\\(669.3, 392.6)}&\makecell[c]{(1346.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1375.0, 0.0)\\(8.3, 0.6)}&\makecell[c]{(1381.0, 0.0)\\(653.2, 359.3)}&\makecell[c]{(1197.9, 17.5)\\(0.0, 0.0)}&\makecell[c]{(1278.2, 12.0)\\(2.2, 1.2)}&\makecell[c]{(1377.0, 2.8)\\(376.6, 31.0)}&\makecell[c]{(1271.2, 14.9)\\(0.0, 0.0)}&\makecell[c]{(1314.6, 9.7)\\(4.2, 1.3)}&\makecell[c]{(1377.2, 2.4)\\(422.5, 82.9)}\\\hline
s2v140c1600-8&&&&&\makecell[c]{(1202.7, 17.4)\\(0.0, 0.0)}&\makecell[c]{(1263.4, 10.8)\\(9.1, 0.7)}&\makecell[c]{(1301.0, 7.5)\\(658.6, 366.7)}&\makecell[c]{(1325.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1359.0, 0.0)\\(8.9, 0.6)}&\makecell[c]{(1368.0, 0.0)\\(661.1, 376.6)}&\makecell[c]{(1203.7, 16.8)\\(0.0, 0.0)}&\makecell[c]{(1274.7, 10.3)\\(1.8, 1.1)}&\makecell[c]{(1364.0, 3.8)\\(376.4, 28.6)}&\makecell[c]{(1262.7, 13.2)\\(0.0, 0.0)}&\makecell[c]{(1305.4, 9.5)\\(4.1, 1.2)}&\makecell[c]{(1364.9, 3.2)\\(419.7, 70.9)}\\\hline
s2v140c1600-9&&&&&\makecell[c]{(1200.3, 14.6)\\(0.0, 0.0)}&\makecell[c]{(1260.8, 10.8)\\(8.3, 0.1)}&\makecell[c]{(1299.2, 7.7)\\(663.6, 423.2)}&\makecell[c]{(1305.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1348.0, 0.0)\\(9.3, 0.5)}&\makecell[c]{(1357.0, 0.0)\\(656.5, 375.5)}&\makecell[c]{(1203.3, 15.2)\\(0.0, 0.0)}&\makecell[c]{(1272.5, 11.9)\\(2.2, 1.2)}&\makecell[c]{(1363.3, 4.3)\\(380.8, 46.8)}&\makecell[c]{(1255.0, 12.7)\\(0.0, 0.0)}&\makecell[c]{(1298.9, 9.0)\\(3.7, 0.9)}&\makecell[c]{(1364.5, 4.3)\\(417.3, 67.9)}\\\hline
s2v140c1600-10&&&&&\makecell[c]{(1201.7, 18.9)\\(0.0, 0.0)}&\makecell[c]{(1261.9, 11.5)\\(14.7, 0.9)}&\makecell[c]{(1304.1, 8.3)\\(662.4, 444.0)}&\makecell[c]{(1311.0, 0.0)\\(0.0, 0.0)}&\makecell[c]{(1362.0, 0.0)\\(9.0, 0.7)}&\makecell[c]{(1367.0, 0.0)\\(656.4, 375.6)}&\makecell[c]{(1200.9, 16.0)\\(0.0, 0.0)}&\makecell[c]{(1278.5, 10.9)\\(2.0, 1.0)}&\makecell[c]{(1366.7, 4.0)\\(382.0, 33.1)}&\makecell[c]{(1267.4, 12.9)\\(0.0, 0.0)}&\makecell[c]{(1310.2, 8.7)\\(3.8, 1.0)}&\makecell[c]{(1368.3, 3.2)\\(413.2, 62.9)}\\\hline




\hline
\end{tabular}


==> tables/max2sat180variable_sls.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
&WalkSat&$MCTS\_{WalkSat}$&\multicolumn{3}{c}{$NMC\_{WalkSat}$}&$NMC\_{Novelty}$&Best Solver\\
\hline
&flip=$10^{6}$&m=200&level 1, flip=$10^{3.5}$&level 1, flip=30*numflexibleliteral&level 2&level 1&-\\
\hline
statistic&\makecell[c]{(1454.7, 2.0),(191.0, 23.5)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&\makecell[c]{(1458.0, 4.3),(128.6, 16.8)}&\makecell[c]{(1461.1, 4.0),(397.9, 40.4)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&1479.4\\\hline
s2v180c1200-1&\makecell[c]{(1050.1, 1.6),(156.9, 12.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1052.1, 4.1),(96.4, 6.7)}&\makecell[c]{(1054.6, 3.3),(312.4, 20.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1066\\\hline
s2v180c1200-2&\makecell[c]{(1055.5, 2.1),(155.1, 12.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1058.7, 4.6),(101.8, 6.1)}&\makecell[c]{(1057.8, 1.1),(319.8, 12.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1070\\\hline
s2v180c1200-3&\makecell[c]{(1056.0, 1.2),(156.8, 11.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1059.4, 3.8),(100.5, 7.0)}&\makecell[c]{(1060.5, 1.8),(321.5, 18.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1069\\\hline
s2v180c1200-4&\makecell[c]{(1055.7, 0.9),(154.7, 10.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1060.2, 2.9),(95.0, 8.0)}&\makecell[c]{(1061.2, 2.3),(308.3, 15.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1072\\\hline
s2v180c1300-1&\makecell[c]{(1128.0, 1.6),(165.4, 10.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1129.0, 4.0),(113.1, 9.7)}&\makecell[c]{(1134.9, 3.2),(339.6, 14.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1147\\\hline
s2v180c1300-2&\makecell[c]{(1147.2, 0.9),(170.3, 14.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1147.6, 2.5),(110.3, 11.9)}&\makecell[c]{(1151.3, 2.5),(330.1, 16.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1162\\\hline
s2v180c1300-3&\makecell[c]{(1132.8, 1.4),(172.9, 19.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1136.5, 3.9),(107.4, 8.7)}&\makecell[c]{(1138.9, 2.9),(344.5, 16.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1150\\\hline
s2v180c1300-4&\makecell[c]{(1133.7, 1.3),(165.1, 12.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1136.9, 3.7),(108.4, 6.5)}&\makecell[c]{(1138.1, 2.5),(339.9, 24.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1151\\\hline
s2v180c1400-1&\makecell[c]{(1216.5, 1.0),(175.3, 11.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1220.8, 3.8),(115.5, 10.4)}&\makecell[c]{(1220.7, 3.7),(351.6, 18.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1235\\\hline
s2v180c1400-2&\makecell[c]{(1216.4, 2.0),(179.7, 18.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1219.8, 3.6),(113.1, 10.6)}&\makecell[c]{(1222.8, 3.4),(355.3, 11.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1235\\\hline
s2v180c1400-3&\makecell[c]{(1228.6, 1.9),(174.8, 14.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1231.4, 2.0),(111.0, 8.8)}&\makecell[c]{(1234.9, 2.3),(359.0, 19.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1244\\\hline
s2v180c1400-4&\makecell[c]{(1219.6, 1.3),(170.7, 9.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1222.4, 4.3),(110.6, 8.6)}&\makecell[c]{(1226.1, 2.6),(359.5, 23.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1240\\\hline
s2v180c1500-1&\makecell[c]{(1295.3, 2.0),(185.0, 25.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1298.7, 3.1),(124.4, 10.4)}&\makecell[c]{(1300.2, 3.2),(376.8, 19.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1316\\\hline
s2v180c1500-2&\makecell[c]{(1298.2, 1.3),(172.7, 8.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1302.1, 4.3),(123.6, 14.5)}&\makecell[c]{(1305.7, 2.9),(369.5, 21.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1320\\\hline
s2v180c1500-3&\makecell[c]{(1298.2, 1.9),(179.2, 16.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1303.9, 4.6),(118.3, 9.8)}&\makecell[c]{(1303.8, 2.1),(376.1, 26.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1321\\\hline
s2v180c1500-4&\makecell[c]{(1297.6, 2.8),(181.4, 15.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1300.2, 3.0),(120.1, 8.9)}&\makecell[c]{(1303.8, 2.0),(372.9, 25.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1319\\\hline
s2v180c1600-1&\makecell[c]{(1377.2, 2.2),(185.6, 21.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1378.5, 3.8),(127.2, 15.5)}&\makecell[c]{(1383.6, 2.8),(379.5, 20.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1400\\\hline
s2v180c1600-2&\makecell[c]{(1371.2, 2.5),(186.6, 21.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1373.9, 3.4),(127.7, 18.0)}&\makecell[c]{(1379.5, 4.0),(389.9, 33.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1396\\\hline
s2v180c1600-3&\makecell[c]{(1359.7, 1.6),(181.1, 17.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1363.9, 5.4),(128.9, 16.4)}&\makecell[c]{(1366.4, 3.2),(390.8, 30.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1384\\\hline
s2v180c1600-4&\makecell[c]{(1378.2, 1.2),(182.4, 16.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1382.9, 2.9),(126.4, 11.6)}&\makecell[c]{(1385.5, 4.1),(386.5, 26.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1400\\\hline
s2v180c1700-1&\makecell[c]{(1451.2, 2.2),(189.7, 21.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1455.9, 3.6),(129.0, 12.7)}&\makecell[c]{(1458.1, 4.2),(409.3, 39.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1475\\\hline
s2v180c1700-2&\makecell[c]{(1445.5, 2.3),(206.2, 15.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1446.3, 6.9),(135.0, 10.4)}&\makecell[c]{(1448.0, 4.8),(399.4, 33.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1471\\\hline
s2v180c1700-3&\makecell[c]{(1469.4, 2.7),(185.7, 19.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1473.0, 3.7),(132.8, 20.0)}&\makecell[c]{(1474.8, 4.6),(394.0, 32.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1491\\\hline
s2v180c1700-4&\makecell[c]{(1471.4, 1.4),(186.3, 21.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1474.8, 4.9),(133.2, 20.3)}&\makecell[c]{(1475.6, 5.4),(396.4, 30.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1494\\\hline
s2v180c1800-1&\makecell[c]{(1531.9, 2.8),(199.9, 30.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1532.4, 5.0),(137.2, 23.2)}&\makecell[c]{(1538.6, 6.1),(422.6, 48.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1559\\\hline
s2v180c1800-2&\makecell[c]{(1531.6, 1.4),(194.1, 27.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1534.4, 3.0),(130.4, 15.1)}&\makecell[c]{(1537.4, 6.2),(418.0, 53.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1558\\\hline
s2v180c1800-3&\makecell[c]{(1542.5, 1.4),(195.5, 26.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1545.3, 3.8),(134.3, 19.7)}&\makecell[c]{(1552.1, 4.7),(413.1, 47.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1568\\\hline
s2v180c1800-4&\makecell[c]{(1532.7, 3.3),(197.0, 26.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1535.9, 4.7),(134.1, 19.4)}&\makecell[c]{(1538.0, 6.6),(416.9, 50.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1559\\\hline
s2v180c1900-1&\makecell[c]{(1627.0, 3.7),(206.1, 36.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1630.0, 5.5),(139.6, 25.1)}&\makecell[c]{(1634.0, 4.4),(427.1, 53.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1655\\\hline
s2v180c1900-2&\makecell[c]{(1627.2, 1.8),(202.0, 33.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1630.0, 3.4),(135.5, 18.6)}&\makecell[c]{(1632.2, 3.4),(426.8, 52.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1654\\\hline
s2v180c1900-3&\makecell[c]{(1616.6, 1.4),(205.3, 27.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1619.8, 4.6),(143.4, 26.9)}&\makecell[c]{(1624.7, 6.0),(427.9, 60.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1648\\\hline
s2v180c1900-4&\makecell[c]{(1611.5, 1.4),(201.1, 30.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1614.6, 5.6),(137.1, 20.5)}&\makecell[c]{(1619.9, 5.2),(428.6, 57.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1643\\\hline
s2v180c2000-1&\makecell[c]{(1686.5, 2.3),(208.7, 34.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1688.8, 6.8),(144.8, 26.6)}&\makecell[c]{(1692.8, 4.9),(431.4, 52.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1718\\\hline
s2v180c2000-2&\makecell[c]{(1684.2, 1.8),(205.8, 30.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1690.0, 3.8),(145.6, 25.2)}&\makecell[c]{(1695.8, 4.0),(435.5, 59.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1715\\\hline
s2v180c2000-3&\makecell[c]{(1702.4, 2.2),(204.1, 30.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1703.5, 4.4),(142.3, 24.6)}&\makecell[c]{(1707.6, 3.6),(446.1, 69.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1729\\\hline
s2v180c2000-4&\makecell[c]{(1688.5, 1.8),(207.5, 37.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1692.1, 4.6),(143.4, 24.0)}&\makecell[c]{(1695.0, 3.7),(443.4, 62.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1720\\\hline
s2v180c2100-1&\makecell[c]{(1776.0, 2.4),(216.5, 40.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1776.7, 5.5),(146.9, 27.4)}&\makecell[c]{(1783.1, 3.7),(448.2, 59.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1806\\\hline
s2v180c2100-2&\makecell[c]{(1764.9, 3.0),(236.2, 15.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1770.5, 5.6),(145.6, 22.5)}&\makecell[c]{(1774.0, 5.1),(459.4, 67.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1799\\\hline
s2v180c2100-3&\makecell[c]{(1777.1, 2.6),(214.2, 36.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1782.4, 5.6),(145.4, 23.5)}&\makecell[c]{(1781.9, 3.3),(463.3, 74.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1807\\\hline
s2v180c2100-4&\makecell[c]{(1759.7, 2.1),(215.8, 37.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1766.1, 4.7),(144.7, 22.6)}&\makecell[c]{(1767.8, 4.2),(455.5, 70.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1797\\\hline
s2v180c2200-1&\makecell[c]{(1838.6, 2.2),(218.7, 38.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1840.4, 5.4),(150.2, 26.5)}&\makecell[c]{(1842.8, 4.2),(464.4, 71.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1870\\\hline
s2v180c2200-2&\makecell[c]{(1846.5, 3.3),(219.6, 38.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1850.4, 3.9),(147.3, 23.7)}&\makecell[c]{(1859.4, 6.0),(467.4, 75.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1882\\\hline
s2v180c2200-3&\makecell[c]{(1860.9, 3.7),(216.0, 36.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1866.0, 5.9),(149.2, 22.5)}&\makecell[c]{(1867.6, 9.3),(461.2, 69.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1894\\\hline
s2v180c2200-4&\makecell[c]{(1848.8, 1.8),(218.4, 40.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1854.4, 6.1),(152.4, 29.4)}&\makecell[c]{(1858.4, 5.9),(466.5, 71.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1883\\\hline

\end{tabular}


==> tables/max2sat200variable_sls.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
&WalkSat&$MCTS\_{WalkSat}$&\multicolumn{3}{c}{$NMC\_{WalkSat}$}&$NMC\_{Novelty}$&Best Solver\\
\hline
&flip=$10^{6}$&m=200&level 1, flip=$10^{3.5}$&level 1, flip=30*numflexibleliteral&level 2&level 1&-\\
\hline
statistic&\makecell[c]{(1307.0, 1.7),(182.9, 20.5)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&\makecell[c]{(1310.3, 4.0),(129.6, 16.5)}&\makecell[c]{(1313.3, 3.7),(435.2, 53.5)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&1329.0\\\hline
s2v200c1200-1&\makecell[c]{(1066.3, 1.4),(160.7, 9.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1069.4, 3.2),(117.7, 11.6)}&\makecell[c]{(1070.8, 2.8),(383.0, 24.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1082\\\hline
s2v200c1200-2&\makecell[c]{(1055.8, 2.4),(167.0, 11.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1060.9, 4.2),(112.2, 7.3)}&\makecell[c]{(1060.9, 3.5),(383.1, 27.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1073\\\hline
s2v200c1200-3&\makecell[c]{(1059.7, 1.2),(161.5, 6.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1063.2, 2.6),(121.4, 10.3)}&\makecell[c]{(1064.3, 3.5),(380.5, 38.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1075\\\hline
s2v200c1200-4&\makecell[c]{(1070.9, 1.5),(165.5, 8.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1074.6, 1.1),(109.5, 6.5)}&\makecell[c]{(1075.6, 3.0),(364.7, 19.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1085\\\hline
s2v200c1200-5&\makecell[c]{(1068.0, 1.5),(169.8, 22.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1070.0, 3.2),(109.4, 7.2)}&\makecell[c]{(1074.4, 3.0),(371.9, 17.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1083\\\hline
s2v200c1200-6&\makecell[c]{(1055.3, 1.2),(158.8, 11.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1057.8, 2.3),(111.0, 10.9)}&\makecell[c]{(1060.1, 3.4),(377.5, 25.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1073\\\hline
s2v200c1200-7&\makecell[c]{(1074.0, 1.2),(169.3, 19.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1075.2, 4.3),(106.7, 8.9)}&\makecell[c]{(1079.6, 2.4),(362.4, 20.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1088\\\hline
s2v200c1300-1&\makecell[c]{(1137.5, 1.5),(169.2, 9.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1139.9, 3.3),(120.0, 13.4)}&\makecell[c]{(1141.9, 2.6),(404.8, 38.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1156\\\hline
s2v200c1300-2&\makecell[c]{(1137.8, 1.8),(169.0, 14.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1139.6, 3.2),(120.4, 11.4)}&\makecell[c]{(1145.0, 2.2),(387.4, 20.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1157\\\hline
s2v200c1300-3&\makecell[c]{(1163.4, 1.6),(169.6, 17.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1166.6, 4.2),(114.2, 11.2)}&\makecell[c]{(1167.6, 2.2),(399.8, 38.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1179\\\hline
s2v200c1300-4&\makecell[c]{(1142.3, 1.2),(167.6, 12.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1146.4, 4.7),(119.1, 8.4)}&\makecell[c]{(1148.1, 2.9),(411.0, 49.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1161\\\hline
s2v200c1300-5&\makecell[c]{(1138.9, 1.7),(174.3, 13.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1143.0, 2.8),(117.7, 14.3)}&\makecell[c]{(1145.3, 4.2),(404.3, 38.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1158\\\hline
s2v200c1300-6&\makecell[c]{(1147.6, 1.9),(176.6, 13.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1148.5, 3.0),(118.4, 9.2)}&\makecell[c]{(1154.5, 3.1),(395.1, 33.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1166\\\hline
s2v200c1300-7&\makecell[c]{(1157.3, 1.4),(172.0, 13.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1158.6, 3.2),(117.8, 11.5)}&\makecell[c]{(1161.2, 2.0),(389.5, 28.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1172\\\hline
s2v200c1400-1&\makecell[c]{(1223.3, 1.9),(177.8, 16.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1227.9, 4.4),(125.0, 10.9)}&\makecell[c]{(1230.7, 4.9),(419.3, 45.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1244\\\hline
s2v200c1400-2&\makecell[c]{(1236.0, 2.1),(169.2, 8.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1239.1, 4.0),(124.7, 15.8)}&\makecell[c]{(1242.9, 2.5),(421.9, 54.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1253\\\hline
s2v200c1400-3&\makecell[c]{(1228.9, 1.4),(172.1, 13.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1231.2, 2.7),(126.2, 13.5)}&\makecell[c]{(1234.7, 2.5),(407.0, 42.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1250\\\hline
s2v200c1400-4&\makecell[c]{(1214.3, 1.8),(174.6, 8.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1218.5, 4.0),(123.5, 14.2)}&\makecell[c]{(1221.0, 3.0),(413.9, 47.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1236\\\hline
s2v200c1400-5&\makecell[c]{(1227.3, 1.3),(180.1, 22.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1230.7, 3.7),(124.0, 14.2)}&\makecell[c]{(1233.8, 1.0),(426.9, 28.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1247\\\hline
s2v200c1400-6&\makecell[c]{(1238.2, 1.3),(182.6, 22.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1243.8, 2.6),(126.5, 15.2)}&\makecell[c]{(1244.3, 2.9),(420.8, 53.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1255\\\hline
s2v200c1400-7&\makecell[c]{(1240.6, 1.7),(179.0, 17.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1242.7, 4.0),(125.3, 12.5)}&\makecell[c]{(1248.8, 2.9),(419.2, 57.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1258\\\hline
s2v200c1500-1&\makecell[c]{(1314.6, 1.7),(184.3, 21.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1319.2, 4.6),(132.0, 17.2)}&\makecell[c]{(1320.9, 3.6),(424.4, 57.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1335\\\hline
s2v200c1500-2&\makecell[c]{(1314.5, 1.4),(181.1, 17.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1317.9, 3.1),(130.6, 19.0)}&\makecell[c]{(1320.5, 2.2),(435.5, 63.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1335\\\hline
s2v200c1500-3&\makecell[c]{(1314.7, 1.6),(182.1, 18.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1317.3, 6.8),(135.1, 23.7)}&\makecell[c]{(1320.7, 3.9),(425.0, 49.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1335\\\hline
s2v200c1500-4&\makecell[c]{(1298.9, 1.4),(183.7, 20.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1303.0, 3.7),(125.2, 12.1)}&\makecell[c]{(1304.9, 3.0),(430.2, 61.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1322\\\hline
s2v200c1500-5&\makecell[c]{(1303.7, 1.9),(189.6, 30.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1304.0, 5.1),(128.4, 17.9)}&\makecell[c]{(1309.1, 3.4),(434.1, 62.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1326\\\hline
s2v200c1500-6&\makecell[c]{(1296.2, 1.7),(185.8, 24.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1299.8, 5.4),(130.9, 17.8)}&\makecell[c]{(1305.0, 4.0),(428.0, 51.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1320\\\hline
s2v200c1500-7&\makecell[c]{(1295.8, 1.5),(178.7, 20.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1297.7, 3.6),(131.0, 18.9)}&\makecell[c]{(1304.4, 5.2),(437.2, 59.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1321\\\hline
s2v200c1600-1&\makecell[c]{(1378.0, 1.6),(188.6, 23.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1380.8, 5.0),(134.7, 15.8)}&\makecell[c]{(1384.2, 4.1),(461.2, 66.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1405\\\hline
s2v200c1600-2&\makecell[c]{(1400.0, 1.2),(188.8, 24.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1402.7, 3.4),(138.6, 24.0)}&\makecell[c]{(1405.0, 2.4),(447.9, 66.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1422\\\hline
s2v200c1600-3&\makecell[c]{(1388.3, 1.2),(184.1, 17.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1391.6, 4.5),(138.8, 22.2)}&\makecell[c]{(1397.7, 6.5),(451.7, 68.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1414\\\hline
s2v200c1600-4&\makecell[c]{(1379.2, 1.8),(187.0, 24.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1384.5, 4.5),(138.8, 19.2)}&\makecell[c]{(1386.0, 5.1),(448.5, 62.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1405\\\hline
s2v200c1600-5&\makecell[c]{(1380.8, 1.9),(186.4, 22.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1383.1, 5.6),(131.8, 16.2)}&\makecell[c]{(1384.9, 3.0),(450.6, 62.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1406\\\hline
s2v200c1600-6&\makecell[c]{(1399.4, 0.8),(190.1, 24.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1402.6, 3.4),(142.5, 16.2)}&\makecell[c]{(1406.2, 4.4),(445.0, 62.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1421\\\hline
s2v200c1600-7&\makecell[c]{(1384.1, 2.0),(193.3, 29.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1385.8, 3.7),(133.1, 18.9)}&\makecell[c]{(1389.5, 3.6),(456.5, 76.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1408\\\hline
s2v200c1700-1&\makecell[c]{(1481.9, 1.3),(207.0, 36.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1485.9, 2.6),(138.9, 23.4)}&\makecell[c]{(1488.4, 4.8),(454.5, 60.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1507\\\hline
s2v200c1700-2&\makecell[c]{(1466.1, 1.6),(193.3, 25.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1471.3, 4.1),(139.9, 19.3)}&\makecell[c]{(1471.4, 3.0),(468.1, 77.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1493\\\hline
s2v200c1700-3&\makecell[c]{(1460.9, 2.9),(191.8, 23.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1463.7, 5.0),(141.6, 25.6)}&\makecell[c]{(1467.9, 4.3),(475.4, 81.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1487\\\hline
s2v200c1700-4&\makecell[c]{(1463.2, 1.5),(192.2, 25.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1466.6, 4.2),(143.1, 25.8)}&\makecell[c]{(1468.9, 4.6),(486.1, 64.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1488\\\hline
s2v200c1700-5&\makecell[c]{(1457.1, 2.5),(196.7, 34.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1460.9, 5.1),(143.2, 22.8)}&\makecell[c]{(1463.0, 5.7),(462.6, 69.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1483\\\hline
s2v200c1700-6&\makecell[c]{(1463.6, 1.6),(193.8, 30.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1469.2, 5.7),(137.2, 20.7)}&\makecell[c]{(1473.8, 2.4),(474.1, 75.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1491\\\hline
s2v200c1700-7&\makecell[c]{(1473.3, 1.6),(194.7, 25.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1475.2, 2.7),(140.4, 20.0)}&\makecell[c]{(1480.6, 4.4),(463.4, 72.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1499\\\hline
s2v200c1800-1&\makecell[c]{(1565.6, 1.9),(197.9, 28.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1572.0, 5.7),(144.9, 24.6)}&\makecell[c]{(1571.5, 6.4),(477.9, 77.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1594\\\hline
s2v200c1800-2&\makecell[c]{(1549.4, 1.5),(199.5, 27.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1550.3, 5.4),(141.5, 22.3)}&\makecell[c]{(1555.2, 3.9),(487.4, 81.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1577\\\hline
s2v200c1800-3&\makecell[c]{(1542.4, 2.1),(197.9, 32.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1548.2, 3.2),(144.2, 21.6)}&\makecell[c]{(1548.7, 4.6),(543.9, 45.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1571\\\hline
s2v200c1800-4&\makecell[c]{(1551.2, 2.7),(196.9, 23.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1553.2, 3.7),(140.3, 19.7)}&\makecell[c]{(1559.1, 6.8),(486.3, 82.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1579\\\hline
s2v200c1800-5&\makecell[c]{(1549.0, 2.7),(199.5, 30.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1553.0, 5.7),(146.7, 23.2)}&\makecell[c]{(1556.6, 5.7),(489.1, 83.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1580\\\hline
s2v200c1800-6&\makecell[c]{(1544.2, 2.4),(212.4, 20.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1547.6, 4.2),(142.8, 20.8)}&\makecell[c]{(1551.7, 4.7),(544.7, 45.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1572\\\hline
s2v200c1800-7&\makecell[c]{(1545.5, 1.9),(199.3, 29.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1548.7, 3.8),(143.2, 21.5)}&\makecell[c]{(1549.6, 5.7),(492.4, 85.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&1574\\\hline


\end{tabular}


==> tables/max3sat70variable.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
&MCTS&$MCTS\_{H1}$&$MCTS\_{H2}$&$MCTS\_{H3}$&\multicolumn{3}{c}{NMC}&\multicolumn{3}{c}{$NMC\_{H1}$}&\multicolumn{3}{c}{$NMC\_{H2}$}&\multicolumn{3}{c}{$NMC\_{H3}$}&\multicolumn{3}{c}{NRPA}&\multicolumn{3}{c}{$GNRPA\_{H1}$}&\multicolumn{3}{c}{$GNRPA\_{H2}$}&\multicolumn{3}{c}{$GNRPA\_{H3}$}\\
\hline
&m=200&m=200&m=200&m=200&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2\\
\hline
statistic&\makecell[c]{(933.2, 3.7)\\(73.5, 10.3)}&\makecell[c]{(943.9, 1.4)\\(303.8, 49.6)}&\makecell[c]{(943.7, 1.9)\\(297.5, 55.9)}&\makecell[c]{(945.0, 2.0)\\(289.0, 50.8)}&\makecell[c]{(875.0, 10.3)\\(0.0, 0.0)}&\makecell[c]{(907.3, 6.2)\\(2.9, 0.7)}&\makecell[c]{(926.1, 4.5)\\(199.8, 36.0)}&\makecell[c]{(929.7, 2.8)\\(0.0, 0.0)}&\makecell[c]{(941.0, 2.1)\\(3.8, 0.7)}&\makecell[c]{(947.2, 1.6)\\(231.3, 35.3)}&\makecell[c]{(930.1, 2.7)\\(0.0, 0.0)}&\makecell[c]{(941.2, 2.0)\\(3.7, 0.7)}&\makecell[c]{(947.1, 1.7)\\(226.5, 32.9)}&\makecell[c]{(935.4, 2.5)\\(0.0, 0.0)}&\makecell[c]{(941.0, 2.1)\\(3.6, 0.7)}&\makecell[c]{(947.2, 1.7)\\(227.5, 38.9)}&\makecell[c]{(873.9, 10.7)\\(0.0, 0.0)}&\makecell[c]{(914.9, 6.3)\\(0.8, 0.1)}&\makecell[c]{(945.7, 3.4)\\(61.2, 12.5)}&\makecell[c]{(929.9, 3.4)\\(0.0, 0.0)}&\makecell[c]{(939.0, 2.7)\\(6.1, 1.2)}&\makecell[c]{(948.4, 2.2)\\(545.9, 95.2)}&\makecell[c]{(931.0, 3.9)\\(0.0, 0.0)}&\makecell[c]{(940.2, 1.8)\\(6.9, 1.4)}&\makecell[c]{(944.7, 1.0)\\(649.5, 128.0)}&\makecell[c]{(935.9, 2.8)\\(0.0, 0.0)}&\makecell[c]{(942.7, 1.2)\\(6.3, 1.1)}&\makecell[c]{(946.1, 0.8)\\(571.4, 104.5)}\\\hline

s3v70c800-1&\makecell[c]{(750.2, 2.5)\\(66.5, 4.1)}&\makecell[c]{(760.0, 0.0)\\(274.4, 17.8)}&\makecell[c]{(759.3, 1.5)\\(247.7, 36.6)}&\makecell[c]{(763.7, 1.3)\\(239.0, 17.0)}&\makecell[c]{(699.0, 10.2)\\(0.0, 0.0)}&\makecell[c]{(728.9, 5.6)\\(2.1, 0.6)}&\makecell[c]{(745.2, 4.0)\\(163.0, 10.1)}&\makecell[c]{(751.9, 1.4)\\(0.0, 0.0)}&\makecell[c]{(758.8, 0.4)\\(3.0, 0.7)}&\makecell[c]{(762.2, 0.7)\\(193.8, 16.4)}&\makecell[c]{(748.0, 2.0)\\(0.0, 0.0)}&\makecell[c]{(759.1, 0.8)\\(2.9, 0.7)}&\makecell[c]{(762.4, 1.0)\\(200.9, 23.7)}&\makecell[c]{(750.7, 2.1)\\(0.0, 0.0)}&\makecell[c]{(759.0, 0.9)\\(2.8, 0.7)}&\makecell[c]{(763.1, 0.8)\\(200.1, 17.4)}&\makecell[c]{(700.0, 7.1)\\(0.0, 0.0)}&\makecell[c]{(730.6, 7.2)\\(0.7, 0.0)}&\makecell[c]{(761.5, 2.3)\\(50.6, 6.2)}&\makecell[c]{(750.5, 3.1)\\(0.0, 0.0)}&\makecell[c]{(756.1, 1.5)\\(4.8, 0.8)}&\makecell[c]{(763.1, 1.3)\\(474.8, 35.2)}&\makecell[c]{(751.7, 2.5)\\(0.0, 0.0)}&\makecell[c]{(755.7, 0.6)\\(4.3, 1.2)}&\makecell[c]{(759.4, 0.8)\\(582.8, 91.7)}&\makecell[c]{(752.4, 1.4)\\(0.0, 0.0)}&\makecell[c]{(757.5, 1.9)\\(5.6, 0.9)}&\makecell[c]{(761.9, 0.3)\\(508.6, 48.7)}\\\hline
s3v70c800-2&\makecell[c]{(750.7, 3.3)\\(69.4, 13.4)}&\makecell[c]{(760.8, 2.2)\\(262.6, 17.4)}&\makecell[c]{(756.8, 2.6)\\(243.5, 18.2)}&\makecell[c]{(759.0, 3.4)\\(241.4, 16.2)}&\makecell[c]{(699.8, 8.4)\\(0.0, 0.0)}&\makecell[c]{(727.6, 5.0)\\(3.4, 1.4)}&\makecell[c]{(743.3, 3.7)\\(222.5, 107.1)}&\makecell[c]{(751.5, 2.9)\\(0.0, 0.0)}&\makecell[c]{(757.0, 0.0)\\(3.5, 0.0)}&\makecell[c]{(760.8, 1.6)\\(202.6, 19.4)}&\makecell[c]{(747.0, 3.8)\\(0.0, 0.0)}&\makecell[c]{(757.9, 1.8)\\(3.0, 0.6)}&\makecell[c]{(761.5, 2.7)\\(197.2, 12.2)}&\makecell[c]{(751.0, 2.3)\\(0.0, 0.0)}&\makecell[c]{(758.3, 2.2)\\(2.3, 0.6)}&\makecell[c]{(761.5, 2.1)\\(193.5, 20.9)}&\makecell[c]{(696.6, 7.7)\\(0.0, 0.0)}&\makecell[c]{(734.8, 4.7)\\(0.6, 0.1)}&\makecell[c]{(759.6, 4.1)\\(54.6, 7.2)}&\makecell[c]{(750.9, 3.5)\\(0.0, 0.0)}&\makecell[c]{(755.4, 1.4)\\(6.8, 1.4)}&\makecell[c]{(761.0, 3.0)\\(490.6, 64.8)}&\makecell[c]{(741.8, 3.6)\\(0.0, 0.0)}&\makecell[c]{(755.3, 2.3)\\(6.0, 1.1)}&\makecell[c]{(758.3, 0.8)\\(603.8, 97.8)}&\makecell[c]{(750.4, 2.3)\\(0.0, 0.0)}&\makecell[c]{(755.4, 1.3)\\(4.8, 1.0)}&\makecell[c]{(758.5, 0.5)\\(495.5, 32.3)}\\\hline
s3v70c800-3&\makecell[c]{(749.4, 3.2)\\(66.5, 6.3)}&\makecell[c]{(755.5, 0.9)\\(276.4, 37.5)}&\makecell[c]{(765.0, 1.8)\\(256.1, 26.3)}&\makecell[c]{(760.0, 1.1)\\(253.0, 24.8)}&\makecell[c]{(701.6, 9.6)\\(0.0, 0.0)}&\makecell[c]{(727.2, 4.8)\\(2.0, 0.6)}&\makecell[c]{(743.8, 3.5)\\(166.5, 10.7)}&\makecell[c]{(746.4, 2.8)\\(0.0, 0.0)}&\makecell[c]{(759.4, 0.9)\\(2.4, 0.6)}&\makecell[c]{(764.3, 1.3)\\(192.9, 12.4)}&\makecell[c]{(755.1, 5.9)\\(0.0, 0.0)}&\makecell[c]{(759.7, 0.9)\\(2.9, 0.8)}&\makecell[c]{(764.2, 1.9)\\(216.9, 26.0)}&\makecell[c]{(754.7, 2.8)\\(0.0, 0.0)}&\makecell[c]{(757.9, 3.4)\\(3.4, 0.1)}&\makecell[c]{(764.3, 2.1)\\(200.2, 15.2)}&\makecell[c]{(699.3, 13.4)\\(0.0, 0.0)}&\makecell[c]{(735.1, 6.1)\\(0.7, 0.0)}&\makecell[c]{(760.4, 4.0)\\(56.8, 13.9)}&\makecell[c]{(746.4, 4.4)\\(0.0, 0.0)}&\makecell[c]{(753.6, 3.6)\\(4.4, 1.0)}&\makecell[c]{(766.9, 3.1)\\(501.1, 68.2)}&\makecell[c]{(745.8, 3.6)\\(0.0, 0.0)}&\makecell[c]{(753.9, 1.3)\\(4.8, 1.3)}&\makecell[c]{(760.3, 1.3)\\(557.2, 61.6)}&\makecell[c]{(753.0, 2.8)\\(0.0, 0.0)}&\makecell[c]{(758.9, 1.4)\\(5.3, 1.0)}&\makecell[c]{(763.1, 1.3)\\(497.5, 40.0)}\\\hline
s3v70c800-4&\makecell[c]{(752.6, 6.5)\\(64.0, 7.0)}&\makecell[c]{(761.7, 0.6)\\(268.5, 43.0)}&\makecell[c]{(763.3, 3.5)\\(253.4, 24.6)}&\makecell[c]{(767.3, 1.8)\\(242.6, 28.4)}&\makecell[c]{(700.6, 8.2)\\(0.0, 0.0)}&\makecell[c]{(729.7, 5.9)\\(2.0, 0.6)}&\makecell[c]{(745.4, 3.9)\\(165.6, 12.7)}&\makecell[c]{(749.3, 3.2)\\(0.0, 0.0)}&\makecell[c]{(758.1, 2.8)\\(3.4, 0.0)}&\makecell[c]{(764.4, 1.6)\\(199.7, 27.9)}&\makecell[c]{(756.0, 2.3)\\(0.0, 0.0)}&\makecell[c]{(757.1, 2.4)\\(3.2, 0.5)}&\makecell[c]{(763.9, 2.2)\\(185.3, 15.2)}&\makecell[c]{(753.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(758.9, 2.8)\\(2.8, 0.7)}&\makecell[c]{(763.9, 2.0)\\(211.1, 48.7)}&\makecell[c]{(698.9, 7.6)\\(0.0, 0.0)}&\makecell[c]{(737.1, 5.6)\\(0.5, 0.2)}&\makecell[c]{(765.2, 1.6)\\(51.5, 6.0)}&\makecell[c]{(752.7, 1.8)\\(0.0, 0.0)}&\makecell[c]{(756.6, 1.6)\\(4.4, 1.1)}&\makecell[c]{(765.6, 3.5)\\(482.1, 44.8)}&\makecell[c]{(749.0, 4.2)\\(0.0, 0.0)}&\makecell[c]{(758.9, 1.6)\\(6.1, 1.0)}&\makecell[c]{(763.2, 1.2)\\(544.9, 47.4)}&\makecell[c]{(753.8, 1.2)\\(0.0, 0.0)}&\makecell[c]{(758.6, 1.8)\\(5.6, 0.6)}&\makecell[c]{(764.0, 0.4)\\(500.4, 50.0)}\\\hline
s3v70c800-5&\makecell[c]{(750.8, 3.5)\\(68.0, 5.3)}&\makecell[c]{(760.2, 1.5)\\(269.9, 31.1)}&\makecell[c]{(758.8, 2.4)\\(251.6, 22.4)}&\makecell[c]{(759.1, 1.9)\\(254.3, 25.8)}&\makecell[c]{(700.8, 8.4)\\(0.0, 0.0)}&\makecell[c]{(728.2, 5.4)\\(2.3, 0.8)}&\makecell[c]{(744.7, 3.7)\\(176.6, 13.4)}&\makecell[c]{(743.3, 1.5)\\(0.0, 0.0)}&\makecell[c]{(755.7, 1.6)\\(3.2, 0.5)}&\makecell[c]{(763.0, 1.2)\\(204.6, 16.9)}&\makecell[c]{(745.3, 2.5)\\(0.0, 0.0)}&\makecell[c]{(755.2, 1.5)\\(2.6, 0.7)}&\makecell[c]{(763.9, 2.3)\\(194.3, 18.1)}&\makecell[c]{(749.9, 1.6)\\(0.0, 0.0)}&\makecell[c]{(755.5, 1.6)\\(2.3, 0.5)}&\makecell[c]{(763.5, 1.0)\\(195.0, 15.2)}&\makecell[c]{(702.1, 11.9)\\(0.0, 0.0)}&\makecell[c]{(735.3, 5.0)\\(0.6, 0.1)}&\makecell[c]{(761.3, 4.5)\\(55.0, 9.7)}&\makecell[c]{(743.9, 2.3)\\(0.0, 0.0)}&\makecell[c]{(754.7, 4.0)\\(6.1, 2.0)}&\makecell[c]{(766.4, 2.4)\\(477.6, 48.4)}&\makecell[c]{(746.3, 5.7)\\(0.0, 0.0)}&\makecell[c]{(754.7, 1.4)\\(5.0, 1.2)}&\makecell[c]{(759.7, 0.9)\\(576.7, 91.8)}&\makecell[c]{(748.6, 3.3)\\(0.0, 0.0)}&\makecell[c]{(755.6, 1.0)\\(5.3, 1.0)}&\makecell[c]{(758.5, 0.7)\\(501.8, 40.2)}\\\hline
s3v70c800-6&\makecell[c]{(755.0, 3.1)\\(64.2, 5.4)}&\makecell[c]{(764.6, 0.8)\\(272.4, 36.1)}&\makecell[c]{(763.7, 1.7)\\(257.7, 27.0)}&\makecell[c]{(760.9, 1.0)\\(239.1, 17.7)}&\makecell[c]{(701.2, 9.7)\\(0.0, 0.0)}&\makecell[c]{(729.3, 6.2)\\(2.1, 0.5)}&\makecell[c]{(747.0, 3.8)\\(165.4, 11.9)}&\makecell[c]{(750.2, 3.9)\\(0.0, 0.0)}&\makecell[c]{(761.1, 3.1)\\(2.6, 0.8)}&\makecell[c]{(766.8, 1.1)\\(188.1, 12.3)}&\makecell[c]{(751.6, 3.0)\\(0.0, 0.0)}&\makecell[c]{(762.1, 3.7)\\(2.4, 0.7)}&\makecell[c]{(767.2, 1.2)\\(195.9, 15.2)}&\makecell[c]{(755.8, 1.8)\\(0.0, 0.0)}&\makecell[c]{(759.8, 4.2)\\(3.4, 0.1)}&\makecell[c]{(766.8, 1.1)\\(193.4, 31.2)}&\makecell[c]{(701.5, 7.5)\\(0.0, 0.0)}&\makecell[c]{(736.5, 5.2)\\(0.3, 0.0)}&\makecell[c]{(765.5, 1.7)\\(52.5, 6.5)}&\makecell[c]{(750.7, 2.4)\\(0.0, 0.0)}&\makecell[c]{(758.6, 3.8)\\(5.1, 0.9)}&\makecell[c]{(767.2, 1.6)\\(475.4, 43.5)}&\makecell[c]{(752.1, 3.7)\\(0.0, 0.0)}&\makecell[c]{(760.9, 1.8)\\(4.6, 1.1)}&\makecell[c]{(764.3, 0.6)\\(604.4, 135.5)}&\makecell[c]{(757.9, 1.1)\\(0.0, 0.0)}&\makecell[c]{(761.2, 1.0)\\(5.6, 0.7)}&\makecell[c]{(764.6, 0.7)\\(500.3, 48.9)}\\\hline
s3v70c800-7&\makecell[c]{(754.8, 2.7)\\(66.7, 8.6)}&\makecell[c]{(761.2, 1.2)\\(255.0, 19.4)}&\makecell[c]{(758.5, 0.7)\\(228.9, 15.3)}&\makecell[c]{(758.9, 1.6)\\(249.1, 29.3)}&\makecell[c]{(701.8, 9.8)\\(0.0, 0.0)}&\makecell[c]{(728.8, 6.5)\\(2.1, 0.6)}&\makecell[c]{(746.4, 4.0)\\(165.0, 10.4)}&\makecell[c]{(749.8, 1.8)\\(0.0, 0.0)}&\makecell[c]{(758.1, 1.7)\\(3.0, 0.7)}&\makecell[c]{(763.3, 1.4)\\(206.2, 17.1)}&\makecell[c]{(754.1, 4.0)\\(0.0, 0.0)}&\makecell[c]{(758.1, 2.3)\\(2.8, 0.7)}&\makecell[c]{(763.4, 0.9)\\(180.3, 10.4)}&\makecell[c]{(755.8, 2.0)\\(0.0, 0.0)}&\makecell[c]{(757.4, 1.3)\\(2.4, 0.8)}&\makecell[c]{(763.0, 1.2)\\(192.9, 19.8)}&\makecell[c]{(699.8, 12.1)\\(0.0, 0.0)}&\makecell[c]{(736.1, 5.5)\\(0.8, 0.2)}&\makecell[c]{(762.4, 2.6)\\(58.2, 9.9)}&\makecell[c]{(747.7, 2.3)\\(0.0, 0.0)}&\makecell[c]{(756.5, 2.2)\\(4.5, 1.2)}&\makecell[c]{(764.5, 3.2)\\(476.9, 30.6)}&\makecell[c]{(754.2, 3.1)\\(0.0, 0.0)}&\makecell[c]{(759.6, 1.4)\\(5.2, 1.5)}&\makecell[c]{(761.3, 0.5)\\(542.3, 51.4)}&\makecell[c]{(756.1, 0.7)\\(0.0, 0.0)}&\makecell[c]{(757.5, 0.7)\\(5.0, 1.3)}&\makecell[c]{(758.5, 0.5)\\(503.7, 58.2)}\\\hline
s3v70c800-8&\makecell[c]{(748.9, 2.5)\\(64.6, 6.1)}&\makecell[c]{(757.5, 2.2)\\(276.5, 24.3)}&\makecell[c]{(758.7, 0.9)\\(257.4, 34.8)}&\makecell[c]{(757.8, 1.1)\\(244.4, 15.5)}&\makecell[c]{(699.4, 8.5)\\(0.0, 0.0)}&\makecell[c]{(728.6, 5.7)\\(2.1, 0.5)}&\makecell[c]{(744.0, 3.8)\\(158.5, 6.0)}&\makecell[c]{(746.6, 4.1)\\(0.0, 0.0)}&\makecell[c]{(755.4, 1.9)\\(2.6, 0.7)}&\makecell[c]{(761.4, 1.2)\\(203.7, 15.6)}&\makecell[c]{(739.1, 3.3)\\(0.1, 0.0)}&\makecell[c]{(755.9, 1.8)\\(4.7, 0.8)}&\makecell[c]{(760.5, 0.7)\\(195.2, 13.2)}&\makecell[c]{(749.1, 1.8)\\(0.0, 0.0)}&\makecell[c]{(755.4, 1.2)\\(3.1, 0.7)}&\makecell[c]{(760.2, 1.3)\\(192.8, 21.1)}&\makecell[c]{(701.3, 10.8)\\(0.0, 0.0)}&\makecell[c]{(732.8, 5.2)\\(0.7, 0.0)}&\makecell[c]{(760.0, 3.0)\\(52.2, 9.8)}&\makecell[c]{(745.1, 3.3)\\(0.0, 0.0)}&\makecell[c]{(753.9, 3.0)\\(5.4, 0.5)}&\makecell[c]{(760.3, 1.5)\\(468.4, 28.1)}&\makecell[c]{(739.9, 4.5)\\(0.0, 0.0)}&\makecell[c]{(754.5, 1.4)\\(4.7, 1.3)}&\makecell[c]{(758.8, 1.0)\\(562.1, 41.0)}&\makecell[c]{(750.1, 2.4)\\(0.0, 0.0)}&\makecell[c]{(754.9, 1.2)\\(4.9, 1.1)}&\makecell[c]{(759.8, 1.9)\\(510.5, 52.5)}\\\hline
s3v70c800-9&\makecell[c]{(752.2, 3.9)\\(63.4, 3.4)}&\makecell[c]{(757.4, 1.9)\\(252.3, 12.1)}&\makecell[c]{(760.8, 1.5)\\(263.2, 19.5)}&\makecell[c]{(759.0, 2.6)\\(242.4, 17.4)}&\makecell[c]{(700.9, 10.0)\\(0.0, 0.0)}&\makecell[c]{(729.0, 5.3)\\(1.8, 0.8)}&\makecell[c]{(745.8, 2.9)\\(177.4, 12.2)}&\makecell[c]{(747.8, 2.6)\\(0.0, 0.0)}&\makecell[c]{(757.6, 1.7)\\(2.5, 0.7)}&\makecell[c]{(761.2, 1.1)\\(192.7, 20.9)}&\makecell[c]{(756.1, 1.4)\\(0.0, 0.0)}&\makecell[c]{(758.8, 2.1)\\(2.6, 0.7)}&\makecell[c]{(761.9, 1.6)\\(199.3, 25.6)}&\makecell[c]{(755.5, 2.1)\\(0.0, 0.0)}&\makecell[c]{(758.0, 1.3)\\(3.0, 0.6)}&\makecell[c]{(761.8, 1.4)\\(192.5, 14.1)}&\makecell[c]{(701.2, 9.7)\\(0.0, 0.0)}&\makecell[c]{(732.9, 5.1)\\(0.7, 0.0)}&\makecell[c]{(760.7, 2.9)\\(56.2, 13.8)}&\makecell[c]{(747.5, 1.5)\\(0.0, 0.0)}&\makecell[c]{(756.4, 2.3)\\(7.0, 2.0)}&\makecell[c]{(762.8, 2.4)\\(489.0, 49.4)}&\makecell[c]{(754.0, 2.8)\\(0.0, 0.0)}&\makecell[c]{(760.1, 1.5)\\(5.0, 1.3)}&\makecell[c]{(762.1, 0.3)\\(574.8, 75.4)}&\makecell[c]{(756.3, 1.7)\\(0.0, 0.0)}&\makecell[c]{(760.0, 0.6)\\(4.6, 1.2)}&\makecell[c]{(762.3, 0.9)\\(493.8, 36.4)}\\\hline
s3v70c800-10&\makecell[c]{(749.8, 2.0)\\(66.6, 4.9)}&\makecell[c]{(763.7, 0.9)\\(283.6, 55.9)}&\makecell[c]{(763.4, 2.7)\\(246.5, 19.6)}&\makecell[c]{(764.3, 1.5)\\(241.6, 20.3)}&\makecell[c]{(700.9, 9.2)\\(0.0, 0.0)}&\makecell[c]{(728.8, 5.2)\\(2.2, 0.6)}&\makecell[c]{(746.2, 3.8)\\(171.1, 12.8)}&\makecell[c]{(739.2, 1.5)\\(0.0, 0.0)}&\makecell[c]{(759.5, 2.9)\\(3.4, 0.0)}&\makecell[c]{(764.7, 1.7)\\(198.9, 12.8)}&\makecell[c]{(750.9, 2.7)\\(0.0, 0.0)}&\makecell[c]{(758.9, 3.6)\\(3.2, 0.5)}&\makecell[c]{(763.6, 1.7)\\(187.2, 13.9)}&\makecell[c]{(759.3, 5.7)\\(0.0, 0.0)}&\makecell[c]{(758.6, 3.3)\\(3.4, 0.0)}&\makecell[c]{(764.4, 1.9)\\(195.0, 24.8)}&\makecell[c]{(696.7, 10.2)\\(0.0, 0.0)}&\makecell[c]{(737.3, 7.4)\\(0.7, 0.0)}&\makecell[c]{(763.5, 4.1)\\(52.1, 5.1)}&\makecell[c]{(741.0, 3.5)\\(0.0, 0.0)}&\makecell[c]{(753.5, 2.2)\\(5.0, 1.1)}&\makecell[c]{(762.5, 1.7)\\(489.8, 53.0)}&\makecell[c]{(750.7, 3.1)\\(0.0, 0.0)}&\makecell[c]{(756.8, 1.3)\\(6.6, 0.0)}&\makecell[c]{(761.4, 1.0)\\(595.4, 94.0)}&\makecell[c]{(759.6, 1.6)\\(0.0, 0.0)}&\makecell[c]{(762.2, 0.6)\\(4.8, 1.2)}&\makecell[c]{(762.7, 0.5)\\(493.3, 23.1)}\\\hline
s3v70c900-1&\makecell[c]{(841.6, 3.0)\\(70.2, 5.9)}&\makecell[c]{(852.7, 0.9)\\(278.0, 31.2)}&\makecell[c]{(848.8, 1.7)\\(285.3, 44.7)}&\makecell[c]{(855.0, 3.0)\\(279.0, 51.1)}&\makecell[c]{(787.0, 9.2)\\(0.0, 0.0)}&\makecell[c]{(817.8, 5.3)\\(2.8, 0.7)}&\makecell[c]{(835.3, 3.7)\\(219.8, 97.4)}&\makecell[c]{(839.9, 3.4)\\(0.0, 0.0)}&\makecell[c]{(851.7, 0.9)\\(3.1, 0.8)}&\makecell[c]{(854.1, 1.5)\\(219.4, 27.3)}&\makecell[c]{(837.6, 2.0)\\(0.0, 0.0)}&\makecell[c]{(851.6, 1.9)\\(3.5, 0.6)}&\makecell[c]{(853.6, 1.0)\\(215.3, 24.9)}&\makecell[c]{(844.0, 2.8)\\(0.0, 0.0)}&\makecell[c]{(851.8, 0.9)\\(3.1, 0.8)}&\makecell[c]{(854.1, 1.1)\\(219.7, 42.3)}&\makecell[c]{(785.6, 6.0)\\(0.0, 0.0)}&\makecell[c]{(820.7, 6.0)\\(0.5, 0.2)}&\makecell[c]{(852.9, 3.7)\\(59.7, 12.6)}&\makecell[c]{(839.7, 3.7)\\(0.0, 0.0)}&\makecell[c]{(845.1, 1.4)\\(5.1, 1.1)}&\makecell[c]{(853.8, 1.6)\\(514.8, 67.7)}&\makecell[c]{(839.0, 3.1)\\(0.0, 0.0)}&\makecell[c]{(846.3, 0.8)\\(5.9, 1.2)}&\makecell[c]{(852.0, 0.0)\\(638.6, 143.2)}&\makecell[c]{(843.0, 2.6)\\(0.0, 0.0)}&\makecell[c]{(848.2, 1.0)\\(5.1, 1.3)}&\makecell[c]{(851.9, 1.4)\\(537.3, 67.5)}\\\hline
s3v70c900-2&\makecell[c]{(843.0, 3.5)\\(71.7, 8.4)}&\makecell[c]{(857.0, 0.0)\\(281.8, 28.9)}&\makecell[c]{(855.9, 2.8)\\(284.6, 45.0)}&\makecell[c]{(856.6, 1.4)\\(271.1, 23.8)}&\makecell[c]{(787.0, 9.7)\\(0.0, 0.0)}&\makecell[c]{(818.8, 6.1)\\(2.5, 0.7)}&\makecell[c]{(836.7, 3.7)\\(176.9, 10.9)}&\makecell[c]{(843.6, 4.5)\\(0.0, 0.0)}&\makecell[c]{(849.3, 2.5)\\(3.6, 0.6)}&\makecell[c]{(857.6, 1.1)\\(208.6, 12.6)}&\makecell[c]{(839.6, 1.8)\\(0.0, 0.0)}&\makecell[c]{(849.2, 2.4)\\(3.2, 0.8)}&\makecell[c]{(857.7, 1.3)\\(210.9, 18.2)}&\makecell[c]{(855.6, 3.2)\\(0.0, 0.0)}&\makecell[c]{(849.0, 2.4)\\(2.4, 0.6)}&\makecell[c]{(858.2, 1.2)\\(210.4, 23.5)}&\makecell[c]{(782.0, 13.2)\\(0.0, 0.0)}&\makecell[c]{(825.7, 3.8)\\(0.7, 0.1)}&\makecell[c]{(856.0, 4.5)\\(56.1, 7.0)}&\makecell[c]{(837.5, 3.5)\\(0.0, 0.0)}&\makecell[c]{(848.1, 1.8)\\(5.9, 0.5)}&\makecell[c]{(858.8, 1.8)\\(510.9, 59.4)}&\makecell[c]{(842.7, 2.0)\\(0.0, 0.0)}&\makecell[c]{(852.1, 2.1)\\(6.9, 0.7)}&\makecell[c]{(855.8, 1.0)\\(614.7, 92.9)}&\makecell[c]{(851.3, 4.8)\\(0.0, 0.0)}&\makecell[c]{(857.3, 1.1)\\(6.3, 1.0)}&\makecell[c]{(858.0, 0.0)\\(540.0, 69.0)}\\\hline
s3v70c900-3&\makecell[c]{(837.9, 3.3)\\(71.5, 9.9)}&\makecell[c]{(851.2, 1.0)\\(290.8, 45.9)}&\makecell[c]{(850.4, 0.5)\\(278.1, 48.9)}&\makecell[c]{(852.7, 2.1)\\(279.8, 49.4)}&\makecell[c]{(787.7, 9.1)\\(0.0, 0.0)}&\makecell[c]{(817.6, 5.1)\\(2.5, 0.6)}&\makecell[c]{(833.9, 3.6)\\(183.1, 10.9)}&\makecell[c]{(834.0, 1.3)\\(0.0, 0.0)}&\makecell[c]{(845.6, 0.5)\\(3.4, 0.7)}&\makecell[c]{(853.0, 1.8)\\(217.5, 23.3)}&\makecell[c]{(841.6, 2.8)\\(0.0, 0.0)}&\makecell[c]{(845.6, 0.5)\\(3.1, 0.8)}&\makecell[c]{(853.9, 2.7)\\(202.8, 6.3)}&\makecell[c]{(837.5, 2.4)\\(0.0, 0.0)}&\makecell[c]{(844.6, 1.1)\\(3.1, 0.9)}&\makecell[c]{(854.0, 2.4)\\(225.1, 40.7)}&\makecell[c]{(789.7, 13.5)\\(0.0, 0.0)}&\makecell[c]{(825.3, 4.2)\\(0.4, 0.1)}&\makecell[c]{(853.5, 3.0)\\(62.7, 13.4)}&\makecell[c]{(838.4, 4.6)\\(0.0, 0.0)}&\makecell[c]{(847.7, 2.6)\\(5.1, 1.0)}&\makecell[c]{(856.7, 2.3)\\(534.8, 74.7)}&\makecell[c]{(835.3, 4.3)\\(0.0, 0.0)}&\makecell[c]{(845.7, 2.5)\\(6.1, 1.3)}&\makecell[c]{(851.2, 1.0)\\(612.4, 106.4)}&\makecell[c]{(841.2, 2.3)\\(0.0, 0.0)}&\makecell[c]{(848.5, 0.8)\\(4.7, 1.3)}&\makecell[c]{(851.8, 1.2)\\(532.6, 61.6)}\\\hline
s3v70c900-4&\makecell[c]{(841.3, 3.0)\\(69.5, 5.4)}&\makecell[c]{(853.9, 1.1)\\(299.2, 87.4)}&\makecell[c]{(854.4, 3.3)\\(286.2, 52.1)}&\makecell[c]{(856.7, 1.7)\\(275.8, 46.9)}&\makecell[c]{(785.0, 8.6)\\(0.0, 0.0)}&\makecell[c]{(817.5, 5.9)\\(2.7, 0.8)}&\makecell[c]{(835.1, 4.5)\\(180.2, 9.8)}&\makecell[c]{(839.4, 2.2)\\(0.0, 0.0)}&\makecell[c]{(847.0, 1.6)\\(2.4, 0.8)}&\makecell[c]{(854.6, 1.7)\\(220.6, 21.9)}&\makecell[c]{(839.2, 2.0)\\(0.0, 0.0)}&\makecell[c]{(847.6, 1.9)\\(3.2, 0.8)}&\makecell[c]{(855.2, 1.3)\\(208.8, 18.2)}&\makecell[c]{(846.8, 1.5)\\(0.0, 0.0)}&\makecell[c]{(849.1, 2.1)\\(3.3, 0.8)}&\makecell[c]{(855.5, 1.6)\\(203.2, 18.3)}&\makecell[c]{(785.8, 8.8)\\(0.0, 0.0)}&\makecell[c]{(827.2, 5.7)\\(0.4, 0.0)}&\makecell[c]{(853.6, 3.6)\\(60.1, 10.4)}&\makecell[c]{(837.3, 3.6)\\(0.0, 0.0)}&\makecell[c]{(845.6, 2.6)\\(3.7, 0.6)}&\makecell[c]{(854.2, 2.5)\\(514.4, 75.5)}&\makecell[c]{(840.9, 3.8)\\(0.0, 0.0)}&\makecell[c]{(846.9, 1.9)\\(5.5, 1.3)}&\makecell[c]{(852.1, 0.9)\\(613.4, 104.6)}&\makecell[c]{(845.6, 2.6)\\(0.0, 0.0)}&\makecell[c]{(850.9, 1.4)\\(6.0, 0.9)}&\makecell[c]{(853.4, 0.5)\\(546.3, 80.5)}\\\hline
s3v70c900-5&\makecell[c]{(843.3, 4.1)\\(69.1, 5.1)}&\makecell[c]{(851.0, 0.9)\\(286.4, 29.0)}&\makecell[c]{(851.5, 0.9)\\(268.6, 26.8)}&\makecell[c]{(851.2, 2.1)\\(278.4, 39.2)}&\makecell[c]{(787.4, 9.0)\\(0.0, 0.0)}&\makecell[c]{(815.6, 6.0)\\(2.7, 0.7)}&\makecell[c]{(835.0, 4.2)\\(183.1, 21.3)}&\makecell[c]{(833.4, 3.4)\\(0.0, 0.0)}&\makecell[c]{(849.9, 1.4)\\(4.6, 1.1)}&\makecell[c]{(855.3, 2.4)\\(218.6, 21.8)}&\makecell[c]{(839.6, 2.8)\\(0.0, 0.0)}&\makecell[c]{(850.6, 2.0)\\(3.6, 1.6)}&\makecell[c]{(854.0, 0.9)\\(209.6, 18.3)}&\makecell[c]{(837.5, 1.6)\\(0.0, 0.0)}&\makecell[c]{(850.7, 1.8)\\(3.4, 0.7)}&\makecell[c]{(855.0, 2.6)\\(210.7, 36.2)}&\makecell[c]{(785.5, 7.9)\\(0.0, 0.0)}&\makecell[c]{(825.4, 8.0)\\(0.6, 0.2)}&\makecell[c]{(851.3, 4.1)\\(58.8, 15.5)}&\makecell[c]{(836.1, 4.7)\\(0.0, 0.0)}&\makecell[c]{(849.6, 2.7)\\(5.0, 1.3)}&\makecell[c]{(856.0, 2.5)\\(520.3, 71.4)}&\makecell[c]{(839.4, 4.5)\\(0.1, 0.0)}&\makecell[c]{(848.9, 1.1)\\(8.4, 1.8)}&\makecell[c]{(852.0, 0.0)\\(621.0, 128.3)}&\makecell[c]{(840.0, 3.1)\\(0.0, 0.0)}&\makecell[c]{(848.8, 2.7)\\(4.7, 1.0)}&\makecell[c]{(854.0, 1.1)\\(538.1, 67.2)}\\\hline
s3v70c900-6&\makecell[c]{(844.2, 3.8)\\(75.3, 10.2)}&\makecell[c]{(849.8, 1.7)\\(292.9, 44.6)}&\makecell[c]{(849.8, 1.8)\\(289.9, 55.7)}&\makecell[c]{(852.2, 1.2)\\(270.2, 28.5)}&\makecell[c]{(788.0, 10.2)\\(0.0, 0.0)}&\makecell[c]{(818.4, 5.6)\\(2.5, 0.7)}&\makecell[c]{(835.4, 4.6)\\(182.8, 13.1)}&\makecell[c]{(837.0, 2.2)\\(0.0, 0.0)}&\makecell[c]{(851.1, 2.6)\\(3.5, 0.5)}&\makecell[c]{(854.5, 1.6)\\(217.7, 28.1)}&\makecell[c]{(832.9, 2.5)\\(0.0, 0.0)}&\makecell[c]{(853.0, 1.9)\\(2.7, 0.8)}&\makecell[c]{(854.9, 0.9)\\(207.0, 16.4)}&\makecell[c]{(840.2, 1.5)\\(0.0, 0.0)}&\makecell[c]{(853.8, 1.8)\\(3.8, 0.1)}&\makecell[c]{(855.2, 1.0)\\(228.8, 50.8)}&\makecell[c]{(784.8, 10.8)\\(0.0, 0.0)}&\makecell[c]{(824.3, 5.3)\\(0.7, 0.0)}&\makecell[c]{(852.5, 3.0)\\(56.7, 5.7)}&\makecell[c]{(840.8, 4.6)\\(0.0, 0.0)}&\makecell[c]{(850.6, 3.4)\\(6.1, 0.1)}&\makecell[c]{(857.9, 1.8)\\(505.6, 62.0)}&\makecell[c]{(834.4, 2.9)\\(0.0, 0.0)}&\makecell[c]{(846.1, 1.8)\\(6.1, 2.1)}&\makecell[c]{(850.2, 0.6)\\(628.8, 128.2)}&\makecell[c]{(844.0, 2.9)\\(0.0, 0.0)}&\makecell[c]{(849.6, 1.2)\\(6.2, 0.9)}&\makecell[c]{(853.5, 0.9)\\(550.9, 96.8)}\\\hline
s3v70c900-7&\makecell[c]{(843.7, 1.5)\\(70.9, 10.2)}&\makecell[c]{(850.9, 2.1)\\(286.8, 32.8)}&\makecell[c]{(853.5, 1.5)\\(274.8, 32.8)}&\makecell[c]{(849.3, 2.1)\\(271.1, 34.2)}&\makecell[c]{(787.5, 9.4)\\(0.0, 0.0)}&\makecell[c]{(817.4, 5.5)\\(2.4, 0.5)}&\makecell[c]{(835.0, 4.0)\\(176.6, 8.9)}&\makecell[c]{(827.2, 1.5)\\(0.0, 0.0)}&\makecell[c]{(847.3, 2.2)\\(3.8, 0.1)}&\makecell[c]{(853.0, 2.2)\\(214.2, 15.8)}&\makecell[c]{(835.0, 3.3)\\(0.0, 0.0)}&\makecell[c]{(847.3, 2.0)\\(3.5, 0.6)}&\makecell[c]{(852.7, 2.0)\\(212.4, 12.9)}&\makecell[c]{(840.7, 1.9)\\(0.0, 0.0)}&\makecell[c]{(848.1, 2.1)\\(3.7, 0.2)}&\makecell[c]{(853.1, 1.1)\\(197.2, 21.2)}&\makecell[c]{(789.6, 10.8)\\(0.0, 0.0)}&\makecell[c]{(824.2, 9.7)\\(0.4, 0.1)}&\makecell[c]{(851.1, 3.3)\\(58.4, 8.4)}&\makecell[c]{(833.0, 3.5)\\(0.0, 0.0)}&\makecell[c]{(844.4, 2.0)\\(5.4, 1.2)}&\makecell[c]{(853.6, 2.3)\\(501.3, 52.6)}&\makecell[c]{(836.3, 3.0)\\(0.0, 0.0)}&\makecell[c]{(846.7, 1.2)\\(6.3, 1.5)}&\makecell[c]{(851.3, 0.8)\\(623.6, 116.7)}&\makecell[c]{(842.8, 2.3)\\(0.1, 0.0)}&\makecell[c]{(848.6, 1.6)\\(5.7, 1.1)}&\makecell[c]{(857.4, 2.3)\\(547.2, 91.0)}\\\hline
s3v70c900-8&\makecell[c]{(840.9, 2.7)\\(69.9, 5.9)}&\makecell[c]{(856.8, 1.0)\\(280.9, 26.0)}&\makecell[c]{(850.2, 1.5)\\(266.6, 32.5)}&\makecell[c]{(852.6, 1.4)\\(274.2, 33.2)}&\makecell[c]{(787.9, 9.1)\\(0.0, 0.0)}&\makecell[c]{(819.4, 5.9)\\(2.7, 0.7)}&\makecell[c]{(836.6, 4.0)\\(180.6, 14.6)}&\makecell[c]{(839.8, 2.1)\\(0.0, 0.0)}&\makecell[c]{(851.9, 1.6)\\(3.8, 0.1)}&\makecell[c]{(855.4, 1.2)\\(211.0, 16.2)}&\makecell[c]{(846.5, 2.4)\\(0.0, 0.0)}&\makecell[c]{(852.6, 1.4)\\(3.5, 0.6)}&\makecell[c]{(855.9, 0.3)\\(217.0, 27.2)}&\makecell[c]{(850.0, 4.2)\\(0.0, 0.0)}&\makecell[c]{(852.3, 2.0)\\(3.6, 0.6)}&\makecell[c]{(855.1, 1.7)\\(201.2, 18.2)}&\makecell[c]{(788.0, 11.2)\\(0.0, 0.0)}&\makecell[c]{(825.4, 5.2)\\(1.2, 0.0)}&\makecell[c]{(852.8, 2.6)\\(55.5, 7.8)}&\makecell[c]{(838.7, 4.1)\\(0.0, 0.0)}&\makecell[c]{(849.8, 1.7)\\(5.8, 0.9)}&\makecell[c]{(856.6, 2.0)\\(512.7, 61.9)}&\makecell[c]{(845.5, 2.1)\\(0.0, 0.0)}&\makecell[c]{(850.8, 0.7)\\(5.4, 1.1)}&\makecell[c]{(853.9, 0.8)\\(627.9, 142.3)}&\makecell[c]{(849.5, 4.1)\\(0.0, 0.0)}&\makecell[c]{(853.9, 0.3)\\(5.2, 1.4)}&\makecell[c]{(855.0, 0.0)\\(536.1, 66.7)}\\\hline
s3v70c900-9&\makecell[c]{(843.0, 3.0)\\(71.3, 9.0)}&\makecell[c]{(853.4, 2.2)\\(287.5, 22.0)}&\makecell[c]{(854.4, 1.7)\\(273.2, 31.3)}&\makecell[c]{(859.9, 1.8)\\(265.3, 22.4)}&\makecell[c]{(787.9, 9.7)\\(0.0, 0.0)}&\makecell[c]{(819.7, 5.7)\\(2.4, 1.0)}&\makecell[c]{(837.4, 4.8)\\(181.2, 11.6)}&\makecell[c]{(836.2, 1.9)\\(0.0, 0.0)}&\makecell[c]{(850.8, 3.4)\\(3.1, 0.8)}&\makecell[c]{(859.4, 1.9)\\(216.0, 20.0)}&\makecell[c]{(841.3, 2.8)\\(0.0, 0.0)}&\makecell[c]{(849.3, 3.1)\\(3.1, 0.8)}&\makecell[c]{(859.0, 2.2)\\(208.2, 19.3)}&\makecell[c]{(840.7, 2.2)\\(0.0, 0.0)}&\makecell[c]{(848.4, 1.8)\\(2.7, 0.7)}&\makecell[c]{(858.0, 2.2)\\(217.0, 24.8)}&\makecell[c]{(783.1, 11.0)\\(0.0, 0.0)}&\makecell[c]{(830.2, 5.9)\\(0.5, 0.2)}&\makecell[c]{(859.9, 2.5)\\(56.1, 8.0)}&\makecell[c]{(837.8, 2.3)\\(0.0, 0.0)}&\makecell[c]{(847.3, 2.0)\\(5.1, 1.2)}&\makecell[c]{(861.0, 4.5)\\(509.7, 58.3)}&\makecell[c]{(844.4, 2.8)\\(0.0, 0.0)}&\makecell[c]{(852.9, 1.7)\\(7.1, 1.2)}&\makecell[c]{(856.5, 1.1)\\(603.1, 73.6)}&\makecell[c]{(847.0, 1.9)\\(0.0, 0.0)}&\makecell[c]{(855.9, 1.8)\\(10.1, 0.9)}&\makecell[c]{(859.9, 0.3)\\(554.8, 176.8)}\\\hline
s3v70c900-10&\makecell[c]{(843.9, 2.8)\\(68.2, 6.8)}&\makecell[c]{(856.5, 2.3)\\(275.9, 22.6)}&\makecell[c]{(847.6, 1.6)\\(286.1, 44.3)}&\makecell[c]{(853.9, 1.1)\\(288.2, 63.1)}&\makecell[c]{(786.9, 9.5)\\(0.0, 0.0)}&\makecell[c]{(816.9, 6.4)\\(2.3, 0.9)}&\makecell[c]{(835.4, 4.6)\\(178.4, 14.0)}&\makecell[c]{(842.3, 3.9)\\(0.0, 0.0)}&\makecell[c]{(854.3, 1.5)\\(3.8, 0.0)}&\makecell[c]{(857.4, 0.8)\\(220.6, 28.4)}&\makecell[c]{(835.8, 2.7)\\(0.0, 0.0)}&\makecell[c]{(854.1, 2.8)\\(3.4, 0.6)}&\makecell[c]{(857.2, 2.0)\\(205.4, 22.0)}&\makecell[c]{(841.1, 1.4)\\(0.0, 0.0)}&\makecell[c]{(854.2, 1.1)\\(3.8, 0.1)}&\makecell[c]{(857.4, 1.1)\\(216.2, 31.1)}&\makecell[c]{(787.6, 11.0)\\(0.0, 0.0)}&\makecell[c]{(823.1, 7.0)\\(0.5, 0.2)}&\makecell[c]{(855.6, 1.9)\\(57.9, 9.1)}&\makecell[c]{(840.8, 2.4)\\(0.0, 0.0)}&\makecell[c]{(848.3, 2.2)\\(5.3, 1.0)}&\makecell[c]{(855.5, 3.5)\\(512.6, 67.7)}&\makecell[c]{(844.9, 4.1)\\(0.0, 0.0)}&\makecell[c]{(851.0, 0.9)\\(6.2, 1.2)}&\makecell[c]{(854.3, 0.5)\\(613.5, 94.9)}&\makecell[c]{(841.5, 2.9)\\(0.0, 0.0)}&\makecell[c]{(850.1, 0.5)\\(6.6, 0.0)}&\makecell[c]{(853.5, 0.8)\\(545.8, 97.5)}\\\hline
s3v70c1000-1&\makecell[c]{(933.2, 3.0)\\(73.6, 11.5)}&\makecell[c]{(939.2, 2.4)\\(303.8, 47.9)}&\makecell[c]{(942.4, 0.5)\\(305.8, 68.0)}&\makecell[c]{(942.1, 2.1)\\(285.7, 37.8)}&\makecell[c]{(876.9, 10.6)\\(0.0, 0.0)}&\makecell[c]{(906.3, 5.7)\\(2.5, 0.8)}&\makecell[c]{(925.2, 4.4)\\(196.8, 14.8)}&\makecell[c]{(931.5, 2.2)\\(0.0, 0.0)}&\makecell[c]{(938.6, 2.1)\\(3.8, 0.8)}&\makecell[c]{(945.2, 1.7)\\(230.6, 26.0)}&\makecell[c]{(933.4, 2.2)\\(0.1, 0.0)}&\makecell[c]{(939.4, 1.7)\\(4.0, 0.7)}&\makecell[c]{(945.0, 1.0)\\(229.3, 26.7)}&\makecell[c]{(931.1, 4.2)\\(0.0, 0.0)}&\makecell[c]{(939.6, 1.6)\\(2.9, 0.7)}&\makecell[c]{(945.0, 1.1)\\(233.8, 38.7)}&\makecell[c]{(873.6, 6.8)\\(0.0, 0.0)}&\makecell[c]{(913.3, 8.8)\\(0.6, 0.2)}&\makecell[c]{(944.9, 2.5)\\(58.9, 8.5)}&\makecell[c]{(929.2, 3.1)\\(0.0, 0.0)}&\makecell[c]{(938.8, 3.1)\\(5.4, 1.2)}&\makecell[c]{(947.9, 1.3)\\(543.4, 95.9)}&\makecell[c]{(929.9, 4.7)\\(0.0, 0.0)}&\makecell[c]{(937.2, 2.4)\\(7.4, 1.1)}&\makecell[c]{(944.0, 0.0)\\(639.9, 118.8)}&\makecell[c]{(928.9, 4.5)\\(0.0, 0.0)}&\makecell[c]{(939.9, 2.0)\\(5.6, 1.3)}&\makecell[c]{(946.0, 0.0)\\(568.7, 96.3)}\\\hline
s3v70c1000-2&\makecell[c]{(934.7, 3.4)\\(73.5, 11.9)}&\makecell[c]{(943.3, 0.9)\\(299.2, 45.4)}&\makecell[c]{(948.9, 1.6)\\(312.1, 89.1)}&\makecell[c]{(954.8, 3.0)\\(276.6, 36.5)}&\makecell[c]{(873.9, 10.3)\\(0.0, 0.0)}&\makecell[c]{(908.9, 6.7)\\(2.6, 0.7)}&\makecell[c]{(927.2, 4.7)\\(196.3, 18.6)}&\makecell[c]{(931.8, 1.6)\\(0.0, 0.0)}&\makecell[c]{(939.6, 3.3)\\(3.9, 0.6)}&\makecell[c]{(948.5, 1.5)\\(235.5, 33.4)}&\makecell[c]{(939.8, 3.1)\\(0.0, 0.0)}&\makecell[c]{(941.8, 1.9)\\(4.3, 0.1)}&\makecell[c]{(948.8, 2.6)\\(229.8, 22.5)}&\makecell[c]{(938.7, 2.5)\\(0.0, 0.0)}&\makecell[c]{(939.3, 3.2)\\(4.0, 0.7)}&\makecell[c]{(949.2, 1.8)\\(226.3, 28.7)}&\makecell[c]{(868.5, 16.4)\\(0.0, 0.0)}&\makecell[c]{(918.3, 5.7)\\(0.7, 0.1)}&\makecell[c]{(949.2, 5.2)\\(64.3, 24.9)}&\makecell[c]{(932.8, 2.7)\\(0.0, 0.0)}&\makecell[c]{(937.7, 3.0)\\(4.8, 1.3)}&\makecell[c]{(948.6, 3.0)\\(538.7, 84.4)}&\makecell[c]{(937.3, 6.4)\\(0.0, 0.0)}&\makecell[c]{(943.9, 2.8)\\(8.0, 0.0)}&\makecell[c]{(949.4, 1.2)\\(651.0, 130.2)}&\makecell[c]{(939.4, 3.1)\\(0.0, 0.0)}&\makecell[c]{(946.0, 0.9)\\(6.7, 0.8)}&\makecell[c]{(948.5, 1.7)\\(564.3, 89.8)}\\\hline
s3v70c1000-3&\makecell[c]{(935.2, 4.8)\\(73.0, 5.7)}&\makecell[c]{(942.4, 2.2)\\(293.8, 28.6)}&\makecell[c]{(945.7, 3.4)\\(297.0, 53.7)}&\makecell[c]{(946.4, 1.6)\\(285.6, 43.7)}&\makecell[c]{(874.1, 9.5)\\(0.0, 0.0)}&\makecell[c]{(906.6, 6.2)\\(3.0, 0.7)}&\makecell[c]{(925.7, 4.1)\\(209.9, 33.2)}&\makecell[c]{(928.0, 3.4)\\(0.0, 0.0)}&\makecell[c]{(942.8, 3.4)\\(3.5, 0.9)}&\makecell[c]{(949.1, 2.2)\\(233.1, 31.9)}&\makecell[c]{(932.2, 1.8)\\(0.0, 0.0)}&\makecell[c]{(942.7, 3.1)\\(3.7, 0.8)}&\makecell[c]{(948.7, 1.5)\\(230.1, 31.1)}&\makecell[c]{(942.6, 1.9)\\(0.0, 0.0)}&\makecell[c]{(941.1, 3.5)\\(3.7, 0.9)}&\makecell[c]{(948.3, 1.6)\\(221.7, 24.4)}&\makecell[c]{(875.4, 13.0)\\(0.0, 0.0)}&\makecell[c]{(914.8, 6.5)\\(0.8, 0.0)}&\makecell[c]{(945.9, 3.2)\\(63.4, 14.4)}&\makecell[c]{(929.3, 4.4)\\(0.0, 0.0)}&\makecell[c]{(941.3, 2.2)\\(4.9, 1.2)}&\makecell[c]{(948.1, 2.0)\\(561.2, 124.9)}&\makecell[c]{(929.6, 3.9)\\(0.0, 0.0)}&\makecell[c]{(942.0, 1.3)\\(5.5, 1.3)}&\makecell[c]{(946.4, 0.8)\\(642.8, 129.5)}&\makecell[c]{(939.5, 3.5)\\(0.0, 0.0)}&\makecell[c]{(945.0, 0.0)\\(7.0, 1.0)}&\makecell[c]{(946.3, 1.2)\\(577.4, 115.9)}\\\hline
s3v70c1000-4&\makecell[c]{(930.5, 4.3)\\(73.0, 12.9)}&\makecell[c]{(936.7, 3.3)\\(310.9, 27.6)}&\makecell[c]{(945.2, 2.4)\\(291.4, 43.4)}&\makecell[c]{(938.7, 2.4)\\(294.6, 67.6)}&\makecell[c]{(875.1, 10.5)\\(0.0, 0.0)}&\makecell[c]{(906.2, 5.9)\\(2.6, 0.5)}&\makecell[c]{(924.5, 4.7)\\(200.9, 22.6)}&\makecell[c]{(921.8, 2.8)\\(0.0, 0.0)}&\makecell[c]{(936.5, 1.0)\\(4.3, 0.0)}&\makecell[c]{(942.4, 2.7)\\(232.2, 32.3)}&\makecell[c]{(927.1, 3.8)\\(0.0, 0.0)}&\makecell[c]{(935.5, 1.0)\\(3.5, 0.9)}&\makecell[c]{(942.3, 2.6)\\(224.7, 31.2)}&\makecell[c]{(931.1, 2.6)\\(0.0, 0.0)}&\makecell[c]{(935.5, 1.0)\\(4.1, 0.5)}&\makecell[c]{(942.3, 2.6)\\(230.7, 37.5)}&\makecell[c]{(874.3, 12.5)\\(0.0, 0.0)}&\makecell[c]{(914.4, 5.1)\\(0.7, 0.2)}&\makecell[c]{(940.8, 4.4)\\(61.6, 11.8)}&\makecell[c]{(928.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(936.4, 2.8)\\(5.6, 1.3)}&\makecell[c]{(947.5, 3.7)\\(545.0, 93.8)}&\makecell[c]{(927.3, 3.9)\\(0.0, 0.0)}&\makecell[c]{(940.7, 2.3)\\(7.0, 1.4)}&\makecell[c]{(944.5, 0.5)\\(657.1, 146.7)}&\makecell[c]{(934.5, 3.5)\\(0.0, 0.0)}&\makecell[c]{(940.9, 1.9)\\(4.4, 1.1)}&\makecell[c]{(946.0, 0.8)\\(563.5, 85.9)}\\\hline
s3v70c1000-5&\makecell[c]{(938.6, 3.4)\\(71.8, 13.0)}&\makecell[c]{(952.4, 0.5)\\(299.1, 36.7)}&\makecell[c]{(950.8, 0.6)\\(292.7, 37.3)}&\makecell[c]{(947.7, 1.6)\\(282.4, 43.6)}&\makecell[c]{(874.6, 11.4)\\(0.0, 0.0)}&\makecell[c]{(908.7, 6.5)\\(2.7, 0.6)}&\makecell[c]{(930.6, 5.4)\\(196.3, 23.3)}&\makecell[c]{(939.6, 3.3)\\(0.0, 0.0)}&\makecell[c]{(947.0, 1.7)\\(3.6, 0.9)}&\makecell[c]{(952.5, 1.4)\\(236.3, 39.3)}&\makecell[c]{(930.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(947.8, 1.2)\\(4.2, 1.4)}&\makecell[c]{(952.1, 0.8)\\(226.9, 29.8)}&\makecell[c]{(940.8, 1.6)\\(0.0, 0.0)}&\makecell[c]{(948.0, 1.3)\\(3.4, 1.0)}&\makecell[c]{(952.7, 1.6)\\(224.2, 26.0)}&\makecell[c]{(876.2, 10.2)\\(0.0, 0.0)}&\makecell[c]{(916.8, 5.1)\\(0.8, 0.0)}&\makecell[c]{(949.9, 4.4)\\(63.0, 14.0)}&\makecell[c]{(937.6, 5.6)\\(0.0, 0.0)}&\makecell[c]{(946.1, 1.8)\\(5.5, 1.0)}&\makecell[c]{(954.9, 2.0)\\(546.4, 78.2)}&\makecell[c]{(935.1, 4.0)\\(0.0, 0.0)}&\makecell[c]{(947.0, 2.1)\\(7.0, 1.5)}&\makecell[c]{(950.0, 1.1)\\(640.4, 112.4)}&\makecell[c]{(941.6, 2.2)\\(0.0, 0.0)}&\makecell[c]{(948.4, 1.4)\\(6.8, 1.9)}&\makecell[c]{(952.1, 0.8)\\(565.1, 95.5)}\\\hline
s3v70c1000-6&\makecell[c]{(931.5, 4.0)\\(75.0, 8.7)}&\makecell[c]{(939.3, 1.2)\\(303.0, 49.2)}&\makecell[c]{(937.6, 2.9)\\(304.1, 65.6)}&\makecell[c]{(941.3, 3.0)\\(286.1, 43.4)}&\makecell[c]{(873.0, 11.3)\\(0.0, 0.0)}&\makecell[c]{(908.0, 5.0)\\(3.0, 0.7)}&\makecell[c]{(924.0, 4.3)\\(199.3, 18.9)}&\makecell[c]{(924.2, 2.0)\\(0.0, 0.0)}&\makecell[c]{(933.1, 3.3)\\(3.9, 0.8)}&\makecell[c]{(943.6, 2.5)\\(227.8, 20.1)}&\makecell[c]{(925.1, 0.9)\\(0.0, 0.0)}&\makecell[c]{(934.8, 3.0)\\(3.0, 0.8)}&\makecell[c]{(943.8, 2.2)\\(232.3, 38.9)}&\makecell[c]{(930.7, 3.6)\\(0.0, 0.0)}&\makecell[c]{(932.9, 2.9)\\(3.2, 0.9)}&\makecell[c]{(943.4, 2.3)\\(221.9, 25.2)}&\makecell[c]{(877.1, 12.7)\\(0.0, 0.0)}&\makecell[c]{(911.9, 6.1)\\(0.8, 0.0)}&\makecell[c]{(942.6, 3.7)\\(57.5, 7.6)}&\makecell[c]{(923.1, 2.7)\\(0.0, 0.0)}&\makecell[c]{(936.4, 3.2)\\(6.1, 1.4)}&\makecell[c]{(945.0, 1.8)\\(552.5, 109.2)}&\makecell[c]{(928.0, 4.9)\\(0.0, 0.0)}&\makecell[c]{(936.2, 1.7)\\(6.8, 1.5)}&\makecell[c]{(939.9, 1.1)\\(644.2, 110.9)}&\makecell[c]{(932.8, 3.5)\\(0.0, 0.0)}&\makecell[c]{(938.6, 1.9)\\(6.9, 0.7)}&\makecell[c]{(942.2, 0.4)\\(564.5, 89.5)}\\\hline
s3v70c1000-7&\makecell[c]{(932.9, 3.0)\\(76.3, 6.2)}&\makecell[c]{(942.6, 1.4)\\(299.2, 42.8)}&\makecell[c]{(940.2, 1.9)\\(300.5, 41.8)}&\makecell[c]{(944.0, 2.6)\\(292.6, 51.7)}&\makecell[c]{(874.9, 10.2)\\(0.0, 0.0)}&\makecell[c]{(906.8, 5.9)\\(2.6, 0.5)}&\makecell[c]{(925.5, 3.8)\\(231.1, 141.2)}&\makecell[c]{(934.2, 1.5)\\(0.0, 0.0)}&\makecell[c]{(940.1, 2.0)\\(4.9, 1.1)}&\makecell[c]{(944.5, 2.5)\\(232.2, 26.7)}&\makecell[c]{(926.2, 2.3)\\(0.0, 0.0)}&\makecell[c]{(941.2, 1.5)\\(4.2, 0.0)}&\makecell[c]{(946.6, 1.2)\\(229.3, 32.1)}&\makecell[c]{(932.1, 1.5)\\(0.0, 0.0)}&\makecell[c]{(941.6, 2.8)\\(4.3, 0.2)}&\makecell[c]{(945.8, 2.1)\\(232.4, 40.8)}&\makecell[c]{(873.5, 10.4)\\(0.0, 0.0)}&\makecell[c]{(917.2, 5.8)\\(0.8, 0.0)}&\makecell[c]{(943.3, 2.0)\\(62.6, 15.2)}&\makecell[c]{(928.0, 2.6)\\(0.0, 0.0)}&\makecell[c]{(937.4, 2.4)\\(5.6, 1.2)}&\makecell[c]{(945.4, 2.3)\\(537.5, 89.9)}&\makecell[c]{(926.2, 2.7)\\(0.0, 0.0)}&\makecell[c]{(934.6, 2.0)\\(8.9, 2.0)}&\makecell[c]{(940.1, 1.0)\\(672.4, 194.6)}&\makecell[c]{(933.0, 1.5)\\(0.0, 0.0)}&\makecell[c]{(939.0, 1.3)\\(6.4, 1.1)}&\makecell[c]{(942.2, 0.9)\\(568.6, 99.6)}\\\hline
s3v70c1000-8&\makecell[c]{(931.6, 5.5)\\(75.8, 10.9)}&\makecell[c]{(941.8, 1.3)\\(308.7, 63.6)}&\makecell[c]{(941.4, 2.9)\\(309.4, 71.3)}&\makecell[c]{(946.1, 2.3)\\(285.8, 45.0)}&\makecell[c]{(876.5, 11.4)\\(0.0, 0.0)}&\makecell[c]{(909.3, 6.6)\\(2.7, 0.6)}&\makecell[c]{(927.3, 4.5)\\(198.5, 18.0)}&\makecell[c]{(920.4, 3.2)\\(0.0, 0.0)}&\makecell[c]{(936.9, 3.4)\\(3.9, 0.7)}&\makecell[c]{(946.2, 1.6)\\(240.0, 47.7)}&\makecell[c]{(928.3, 3.0)\\(0.0, 0.0)}&\makecell[c]{(938.3, 2.4)\\(3.7, 0.7)}&\makecell[c]{(946.6, 2.2)\\(235.3, 43.0)}&\makecell[c]{(938.9, 2.8)\\(0.0, 0.0)}&\makecell[c]{(937.4, 2.1)\\(4.2, 0.0)}&\makecell[c]{(946.9, 1.3)\\(223.7, 18.6)}&\makecell[c]{(872.8, 12.5)\\(0.0, 0.0)}&\makecell[c]{(914.0, 7.7)\\(0.8, 0.0)}&\makecell[c]{(945.3, 3.2)\\(61.5, 12.2)}&\makecell[c]{(924.8, 2.2)\\(0.0, 0.0)}&\makecell[c]{(936.0, 3.2)\\(4.8, 1.3)}&\makecell[c]{(950.6, 1.2)\\(549.4, 100.6)}&\makecell[c]{(930.1, 4.3)\\(0.0, 0.0)}&\makecell[c]{(938.3, 1.6)\\(7.2, 1.1)}&\makecell[c]{(943.7, 1.2)\\(641.6, 119.3)}&\makecell[c]{(936.5, 1.7)\\(0.0, 0.0)}&\makecell[c]{(943.0, 0.8)\\(5.3, 1.2)}&\makecell[c]{(945.7, 0.6)\\(569.4, 100.9)}\\\hline
s3v70c1000-9&\makecell[c]{(931.3, 2.3)\\(76.1, 7.6)}&\makecell[c]{(939.6, 2.8)\\(320.6, 115.0)}&\makecell[c]{(943.7, 2.0)\\(291.4, 54.2)}&\makecell[c]{(942.1, 2.2)\\(296.5, 67.7)}&\makecell[c]{(875.0, 9.6)\\(0.0, 0.0)}&\makecell[c]{(906.6, 5.6)\\(2.8, 0.8)}&\makecell[c]{(925.4, 5.1)\\(197.9, 15.9)}&\makecell[c]{(929.3, 2.8)\\(0.0, 0.0)}&\makecell[c]{(939.0, 1.5)\\(4.2, 0.0)}&\makecell[c]{(945.8, 1.2)\\(236.4, 35.8)}&\makecell[c]{(933.2, 2.4)\\(0.0, 0.0)}&\makecell[c]{(939.8, 1.8)\\(2.3, 0.3)}&\makecell[c]{(943.1, 2.3)\\(239.4, 45.9)}&\makecell[c]{(939.2, 2.7)\\(0.0, 0.0)}&\makecell[c]{(939.7, 2.7)\\(3.8, 0.8)}&\makecell[c]{(943.8, 1.8)\\(234.2, 33.1)}&\makecell[c]{(873.3, 11.3)\\(0.0, 0.0)}&\makecell[c]{(913.6, 6.8)\\(0.8, 0.0)}&\makecell[c]{(942.5, 3.9)\\(59.6, 9.0)}&\makecell[c]{(931.6, 3.2)\\(0.0, 0.0)}&\makecell[c]{(939.2, 1.7)\\(6.7, 0.8)}&\makecell[c]{(946.6, 0.8)\\(551.3, 109.9)}&\makecell[c]{(935.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(941.6, 1.9)\\(6.5, 1.5)}&\makecell[c]{(945.3, 0.6)\\(636.4, 101.8)}&\makecell[c]{(937.4, 1.7)\\(0.0, 0.0)}&\makecell[c]{(941.0, 1.0)\\(6.6, 0.9)}&\makecell[c]{(945.2, 0.4)\\(576.2, 107.6)}\\\hline
s3v70c1000-10&\makecell[c]{(933.8, 4.0)\\(73.6, 8.6)}&\makecell[c]{(944.2, 0.6)\\(300.2, 41.5)}&\makecell[c]{(947.2, 1.5)\\(305.1, 66.1)}&\makecell[c]{(948.4, 0.9)\\(291.6, 62.6)}&\makecell[c]{(874.6, 11.9)\\(0.0, 0.0)}&\makecell[c]{(907.7, 6.6)\\(2.8, 0.7)}&\makecell[c]{(927.5, 4.4)\\(200.2, 19.3)}&\makecell[c]{(932.7, 2.3)\\(0.0, 0.0)}&\makecell[c]{(943.4, 1.8)\\(3.2, 0.9)}&\makecell[c]{(947.5, 1.6)\\(237.3, 38.5)}&\makecell[c]{(931.4, 1.9)\\(0.0, 0.0)}&\makecell[c]{(941.8, 1.1)\\(4.0, 0.8)}&\makecell[c]{(948.1, 1.5)\\(228.7, 27.4)}&\makecell[c]{(938.9, 1.1)\\(0.0, 0.0)}&\makecell[c]{(941.7, 0.9)\\(2.8, 0.8)}&\makecell[c]{(948.7, 1.5)\\(229.8, 32.4)}&\makecell[c]{(872.1, 11.7)\\(0.0, 0.0)}&\makecell[c]{(913.1, 5.3)\\(0.5, 0.1)}&\makecell[c]{(947.3, 2.6)\\(58.7, 10.7)}&\makecell[c]{(932.9, 2.0)\\(0.0, 0.0)}&\makecell[c]{(941.4, 4.0)\\(6.1, 1.1)}&\makecell[c]{(950.2, 1.9)\\(549.5, 100.7)}&\makecell[c]{(931.4, 5.4)\\(0.0, 0.0)}&\makecell[c]{(942.0, 2.4)\\(8.0, 2.1)}&\makecell[c]{(945.7, 1.0)\\(678.3, 202.4)}&\makecell[c]{(937.7, 2.8)\\(0.0, 0.0)}&\makecell[c]{(945.9, 1.1)\\(7.0, 1.0)}&\makecell[c]{(947.5, 1.0)\\(561.9, 85.1)}\\\hline
s3v70c1100-1&\makecell[c]{(1024.9, 3.9)\\(77.1, 14.7)}&\makecell[c]{(1036.9, 0.7)\\(312.9, 53.9)}&\makecell[c]{(1032.3, 1.0)\\(328.6, 94.2)}&\makecell[c]{(1037.6, 1.2)\\(299.0, 58.7)}&\makecell[c]{(962.4, 11.2)\\(0.0, 0.0)}&\makecell[c]{(996.8, 6.6)\\(2.8, 0.9)}&\makecell[c]{(1016.8, 4.2)\\(214.0, 32.3)}&\makecell[c]{(1024.5, 3.1)\\(0.0, 0.0)}&\makecell[c]{(1033.8, 1.8)\\(5.2, 1.3)}&\makecell[c]{(1039.9, 2.8)\\(246.9, 46.9)}&\makecell[c]{(1005.1, 4.2)\\(0.0, 0.0)}&\makecell[c]{(1033.4, 1.2)\\(4.6, 0.0)}&\makecell[c]{(1039.5, 2.2)\\(235.2, 35.9)}&\makecell[c]{(1022.2, 2.6)\\(0.0, 0.0)}&\makecell[c]{(1033.0, 1.9)\\(4.7, 0.3)}&\makecell[c]{(1038.3, 3.1)\\(241.0, 43.0)}&\makecell[c]{(959.6, 9.6)\\(0.0, 0.0)}&\makecell[c]{(1003.2, 7.8)\\(1.4, 0.2)}&\makecell[c]{(1036.0, 3.0)\\(67.4, 18.4)}&\makecell[c]{(1025.3, 2.3)\\(0.0, 0.0)}&\makecell[c]{(1030.6, 2.1)\\(7.2, 0.9)}&\makecell[c]{(1038.0, 2.0)\\(585.3, 143.0)}&\makecell[c]{(1016.1, 4.3)\\(0.0, 0.0)}&\makecell[c]{(1029.5, 1.8)\\(7.2, 1.8)}&\makecell[c]{(1034.5, 1.0)\\(674.3, 138.7)}&\makecell[c]{(1019.9, 1.9)\\(0.0, 0.0)}&\makecell[c]{(1031.3, 1.4)\\(5.8, 1.2)}&\makecell[c]{(1035.5, 0.8)\\(609.1, 136.7)}\\\hline
s3v70c1100-2&\makecell[c]{(1023.3, 3.3)\\(77.5, 12.6)}&\makecell[c]{(1035.2, 0.4)\\(320.5, 60.7)}&\makecell[c]{(1038.2, 0.6)\\(312.0, 58.2)}&\makecell[c]{(1038.8, 0.4)\\(311.2, 73.1)}&\makecell[c]{(962.9, 11.2)\\(0.0, 0.0)}&\makecell[c]{(996.5, 6.4)\\(2.9, 0.6)}&\makecell[c]{(1017.7, 4.2)\\(214.0, 33.9)}&\makecell[c]{(1014.4, 3.7)\\(0.0, 0.0)}&\makecell[c]{(1032.6, 2.3)\\(3.7, 1.0)}&\makecell[c]{(1039.2, 2.1)\\(247.5, 52.0)}&\makecell[c]{(1022.6, 2.6)\\(0.0, 0.0)}&\makecell[c]{(1033.0, 1.3)\\(3.9, 0.8)}&\makecell[c]{(1037.8, 1.2)\\(240.8, 36.7)}&\makecell[c]{(1027.4, 2.5)\\(0.0, 0.0)}&\makecell[c]{(1032.7, 1.7)\\(4.2, 0.8)}&\makecell[c]{(1038.2, 1.8)\\(239.4, 42.1)}&\makecell[c]{(961.6, 14.0)\\(0.0, 0.0)}&\makecell[c]{(1004.1, 7.0)\\(1.5, 0.0)}&\makecell[c]{(1038.5, 4.2)\\(61.9, 14.9)}&\makecell[c]{(1019.4, 4.4)\\(0.0, 0.0)}&\makecell[c]{(1028.3, 3.3)\\(6.4, 1.4)}&\makecell[c]{(1039.9, 3.2)\\(570.1, 109.1)}&\makecell[c]{(1023.9, 3.3)\\(0.0, 0.0)}&\makecell[c]{(1032.2, 1.0)\\(7.2, 1.5)}&\makecell[c]{(1035.4, 0.7)\\(669.8, 135.2)}&\makecell[c]{(1028.7, 1.6)\\(0.0, 0.0)}&\makecell[c]{(1033.4, 1.5)\\(6.6, 1.4)}&\makecell[c]{(1036.5, 0.9)\\(608.6, 131.3)}\\\hline
s3v70c1100-3&\makecell[c]{(1021.7, 3.6)\\(76.4, 13.9)}&\makecell[c]{(1038.9, 1.9)\\(320.3, 67.1)}&\makecell[c]{(1036.9, 1.8)\\(320.6, 71.2)}&\makecell[c]{(1039.5, 2.2)\\(309.1, 67.3)}&\makecell[c]{(962.3, 11.4)\\(0.0, 0.0)}&\makecell[c]{(995.1, 7.3)\\(2.9, 0.6)}&\makecell[c]{(1016.9, 4.8)\\(219.0, 44.7)}&\makecell[c]{(1026.5, 2.5)\\(0.0, 0.0)}&\makecell[c]{(1032.1, 1.7)\\(3.5, 0.8)}&\makecell[c]{(1042.0, 2.7)\\(238.2, 29.3)}&\makecell[c]{(1011.9, 2.1)\\(0.0, 0.0)}&\makecell[c]{(1032.1, 1.7)\\(4.2, 0.8)}&\makecell[c]{(1042.0, 2.7)\\(242.5, 49.5)}&\makecell[c]{(1024.8, 5.1)\\(0.0, 0.0)}&\makecell[c]{(1031.5, 1.2)\\(4.2, 0.8)}&\makecell[c]{(1043.6, 1.8)\\(242.6, 47.7)}&\makecell[c]{(959.6, 11.0)\\(0.0, 0.0)}&\makecell[c]{(1006.9, 6.6)\\(0.8, 0.0)}&\makecell[c]{(1040.6, 1.9)\\(62.1, 9.5)}&\makecell[c]{(1024.7, 4.1)\\(0.0, 0.0)}&\makecell[c]{(1033.5, 3.4)\\(5.8, 1.4)}&\makecell[c]{(1045.5, 1.2)\\(565.5, 105.7)}&\makecell[c]{(1019.3, 6.3)\\(0.0, 0.0)}&\makecell[c]{(1031.5, 4.2)\\(7.7, 1.5)}&\makecell[c]{(1038.6, 1.0)\\(686.8, 171.4)}&\makecell[c]{(1025.4, 5.2)\\(0.0, 0.0)}&\makecell[c]{(1036.5, 1.6)\\(6.7, 1.2)}&\makecell[c]{(1041.5, 1.3)\\(596.5, 117.0)}\\\hline
s3v70c1100-4&\makecell[c]{(1028.9, 3.8)\\(76.0, 9.2)}&\makecell[c]{(1037.5, 2.4)\\(306.8, 37.7)}&\makecell[c]{(1037.8, 0.4)\\(318.5, 66.7)}&\makecell[c]{(1041.7, 1.8)\\(301.9, 63.1)}&\makecell[c]{(960.9, 9.9)\\(0.0, 0.0)}&\makecell[c]{(997.6, 7.4)\\(2.9, 0.6)}&\makecell[c]{(1019.0, 5.6)\\(216.9, 39.0)}&\makecell[c]{(1022.4, 2.5)\\(0.0, 0.0)}&\makecell[c]{(1033.7, 5.7)\\(3.8, 1.0)}&\makecell[c]{(1043.4, 1.7)\\(246.9, 40.8)}&\makecell[c]{(1024.5, 1.7)\\(0.0, 0.0)}&\makecell[c]{(1035.2, 3.7)\\(4.7, 0.1)}&\makecell[c]{(1043.9, 1.2)\\(243.2, 48.8)}&\makecell[c]{(1033.5, 1.7)\\(0.0, 0.0)}&\makecell[c]{(1037.4, 4.5)\\(4.2, 0.8)}&\makecell[c]{(1044.2, 1.2)\\(235.2, 34.2)}&\makecell[c]{(964.4, 12.8)\\(0.0, 0.0)}&\makecell[c]{(1008.1, 8.9)\\(0.8, 0.1)}&\makecell[c]{(1042.4, 4.5)\\(67.6, 17.5)}&\makecell[c]{(1019.8, 5.5)\\(0.0, 0.0)}&\makecell[c]{(1032.7, 3.0)\\(6.0, 1.0)}&\makecell[c]{(1042.6, 2.4)\\(576.7, 120.8)}&\makecell[c]{(1026.1, 3.5)\\(0.0, 0.0)}&\makecell[c]{(1036.3, 1.3)\\(5.8, 1.4)}&\makecell[c]{(1040.5, 0.9)\\(681.4, 141.2)}&\makecell[c]{(1033.7, 2.0)\\(0.0, 0.0)}&\makecell[c]{(1038.9, 0.3)\\(7.1, 1.0)}&\makecell[c]{(1041.8, 0.6)\\(603.6, 134.0)}\\\hline
s3v70c1100-5&\makecell[c]{(1027.6, 4.4)\\(77.2, 10.7)}&\makecell[c]{(1040.3, 0.9)\\(315.2, 52.4)}&\makecell[c]{(1036.5, 1.5)\\(318.8, 78.9)}&\makecell[c]{(1034.9, 2.2)\\(304.1, 59.8)}&\makecell[c]{(962.8, 10.1)\\(0.0, 0.0)}&\makecell[c]{(997.1, 7.2)\\(3.0, 0.6)}&\makecell[c]{(1018.1, 4.7)\\(216.1, 35.1)}&\makecell[c]{(1020.9, 1.5)\\(0.0, 0.0)}&\makecell[c]{(1036.3, 3.0)\\(4.3, 0.8)}&\makecell[c]{(1041.0, 0.6)\\(249.4, 51.6)}&\makecell[c]{(1023.1, 3.9)\\(0.0, 0.0)}&\makecell[c]{(1036.8, 2.4)\\(4.4, 0.8)}&\makecell[c]{(1041.3, 0.8)\\(264.4, 55.0)}&\makecell[c]{(1030.8, 3.6)\\(0.0, 0.0)}&\makecell[c]{(1036.8, 2.4)\\(3.5, 1.0)}&\makecell[c]{(1041.3, 0.8)\\(243.1, 62.8)}&\makecell[c]{(962.3, 10.6)\\(0.0, 0.0)}&\makecell[c]{(1004.2, 6.6)\\(0.9, 0.0)}&\makecell[c]{(1041.8, 3.8)\\(67.6, 18.1)}&\makecell[c]{(1021.6, 2.9)\\(0.0, 0.0)}&\makecell[c]{(1030.2, 3.1)\\(6.2, 1.2)}&\makecell[c]{(1043.1, 2.2)\\(579.9, 127.6)}&\makecell[c]{(1022.4, 2.8)\\(0.0, 0.0)}&\makecell[c]{(1033.4, 2.4)\\(8.1, 1.2)}&\makecell[c]{(1040.7, 1.6)\\(666.2, 118.6)}&\makecell[c]{(1030.2, 3.5)\\(0.0, 0.0)}&\makecell[c]{(1038.1, 0.9)\\(7.5, 0.6)}&\makecell[c]{(1039.6, 1.2)\\(617.8, 175.9)}\\\hline
s3v70c1100-6&\makecell[c]{(1029.3, 3.7)\\(79.5, 11.3)}&\makecell[c]{(1040.7, 0.9)\\(323.3, 70.9)}&\makecell[c]{(1037.9, 2.3)\\(316.5, 65.3)}&\makecell[c]{(1039.5, 1.5)\\(308.1, 68.8)}&\makecell[c]{(966.0, 11.0)\\(0.0, 0.0)}&\makecell[c]{(997.0, 6.4)\\(3.3, 0.8)}&\makecell[c]{(1017.7, 4.5)\\(217.7, 42.1)}&\makecell[c]{(1022.2, 4.3)\\(0.0, 0.0)}&\makecell[c]{(1040.2, 1.8)\\(3.8, 0.9)}&\makecell[c]{(1042.7, 0.6)\\(238.0, 35.3)}&\makecell[c]{(1028.7, 3.8)\\(0.0, 0.0)}&\makecell[c]{(1040.3, 0.9)\\(4.6, 0.1)}&\makecell[c]{(1042.6, 0.7)\\(238.6, 42.5)}&\makecell[c]{(1026.3, 1.6)\\(0.0, 0.0)}&\makecell[c]{(1038.4, 3.9)\\(3.6, 1.0)}&\makecell[c]{(1042.9, 0.3)\\(253.0, 74.8)}&\makecell[c]{(965.2, 9.7)\\(0.0, 0.0)}&\makecell[c]{(1006.9, 6.7)\\(0.9, 0.0)}&\makecell[c]{(1038.9, 2.2)\\(64.2, 12.8)}&\makecell[c]{(1024.0, 4.4)\\(0.0, 0.0)}&\makecell[c]{(1032.7, 3.6)\\(6.1, 1.7)}&\makecell[c]{(1042.1, 2.4)\\(576.5, 123.7)}&\makecell[c]{(1028.4, 4.9)\\(0.1, 0.0)}&\makecell[c]{(1036.0, 2.2)\\(7.2, 0.9)}&\makecell[c]{(1041.5, 1.1)\\(699.8, 187.2)}&\makecell[c]{(1027.6, 3.4)\\(0.0, 0.0)}&\makecell[c]{(1036.5, 1.0)\\(6.5, 1.7)}&\makecell[c]{(1039.8, 1.6)\\(621.1, 191.3)}\\\hline
s3v70c1100-7&\makecell[c]{(1026.9, 6.1)\\(76.5, 8.1)}&\makecell[c]{(1041.7, 0.5)\\(321.7, 68.5)}&\makecell[c]{(1036.3, 1.7)\\(325.7, 78.4)}&\makecell[c]{(1037.8, 1.3)\\(303.3, 53.2)}&\makecell[c]{(963.8, 11.8)\\(0.0, 0.0)}&\makecell[c]{(997.6, 7.1)\\(4.6, 1.5)}&\makecell[c]{(1018.3, 5.0)\\(210.1, 35.8)}&\makecell[c]{(1023.1, 3.0)\\(0.0, 0.0)}&\makecell[c]{(1032.9, 2.2)\\(3.9, 1.0)}&\makecell[c]{(1039.9, 1.7)\\(249.8, 53.2)}&\makecell[c]{(1024.4, 1.5)\\(0.0, 0.0)}&\makecell[c]{(1034.0, 2.6)\\(3.5, 1.1)}&\makecell[c]{(1040.4, 2.1)\\(236.7, 32.7)}&\makecell[c]{(1032.2, 2.7)\\(0.0, 0.0)}&\makecell[c]{(1032.4, 3.4)\\(4.2, 0.7)}&\makecell[c]{(1039.1, 1.8)\\(237.8, 40.1)}&\makecell[c]{(962.1, 11.5)\\(0.0, 0.0)}&\makecell[c]{(1005.8, 2.9)\\(0.8, 0.0)}&\makecell[c]{(1039.1, 2.4)\\(61.3, 10.3)}&\makecell[c]{(1023.2, 3.4)\\(0.0, 0.0)}&\makecell[c]{(1030.3, 1.8)\\(6.7, 1.5)}&\makecell[c]{(1039.5, 1.9)\\(575.7, 117.8)}&\makecell[c]{(1023.2, 4.3)\\(0.1, 0.0)}&\makecell[c]{(1034.4, 2.4)\\(8.6, 2.6)}&\makecell[c]{(1040.0, 1.5)\\(692.0, 178.0)}&\makecell[c]{(1033.3, 2.7)\\(0.0, 0.0)}&\makecell[c]{(1038.2, 0.6)\\(6.4, 1.4)}&\makecell[c]{(1041.1, 0.7)\\(604.0, 124.5)}\\\hline
s3v70c1100-8&\makecell[c]{(1026.8, 4.2)\\(76.4, 9.3)}&\makecell[c]{(1036.7, 0.9)\\(315.4, 52.5)}&\makecell[c]{(1034.0, 2.4)\\(316.6, 64.9)}&\makecell[c]{(1045.2, 5.6)\\(301.8, 59.3)}&\makecell[c]{(962.4, 10.6)\\(0.0, 0.0)}&\makecell[c]{(997.7, 6.8)\\(3.4, 0.7)}&\makecell[c]{(1017.5, 4.5)\\(215.5, 40.4)}&\makecell[c]{(1022.4, 5.0)\\(0.0, 0.0)}&\makecell[c]{(1034.3, 1.4)\\(4.0, 1.0)}&\makecell[c]{(1038.4, 1.4)\\(250.5, 51.8)}&\makecell[c]{(1026.1, 1.7)\\(0.0, 0.0)}&\makecell[c]{(1032.9, 2.2)\\(3.5, 1.0)}&\makecell[c]{(1037.6, 1.5)\\(238.3, 35.2)}&\makecell[c]{(1025.6, 0.9)\\(0.0, 0.0)}&\makecell[c]{(1033.9, 1.2)\\(4.7, 0.1)}&\makecell[c]{(1038.1, 0.9)\\(241.2, 51.1)}&\makecell[c]{(960.2, 12.6)\\(0.0, 0.0)}&\makecell[c]{(1007.7, 7.3)\\(0.6, 0.2)}&\makecell[c]{(1037.1, 1.9)\\(66.0, 15.1)}&\makecell[c]{(1017.5, 2.9)\\(0.0, 0.0)}&\makecell[c]{(1031.1, 2.4)\\(7.5, 0.1)}&\makecell[c]{(1038.2, 1.4)\\(583.4, 133.9)}&\makecell[c]{(1024.0, 3.1)\\(0.0, 0.0)}&\makecell[c]{(1031.1, 0.5)\\(10.1, 2.8)}&\makecell[c]{(1033.8, 1.2)\\(700.3, 177.1)}&\makecell[c]{(1025.9, 0.5)\\(0.0, 0.0)}&\makecell[c]{(1031.5, 1.6)\\(5.7, 1.6)}&\makecell[c]{(1035.3, 0.6)\\(592.1, 111.5)}\\\hline
s3v70c1100-9&\makecell[c]{(1026.2, 4.8)\\(77.2, 10.6)}&\makecell[c]{(1042.2, 1.7)\\(321.7, 65.5)}&\makecell[c]{(1042.1, 0.9)\\(312.1, 61.0)}&\makecell[c]{(1042.0, 2.5)\\(309.4, 66.8)}&\makecell[c]{(961.8, 10.7)\\(0.0, 0.0)}&\makecell[c]{(998.4, 7.5)\\(3.0, 0.7)}&\makecell[c]{(1018.4, 5.7)\\(210.0, 26.3)}&\makecell[c]{(1027.7, 2.7)\\(0.0, 0.0)}&\makecell[c]{(1036.1, 1.8)\\(3.9, 1.0)}&\makecell[c]{(1045.6, 3.6)\\(246.0, 46.3)}&\makecell[c]{(1025.2, 2.6)\\(0.1, 0.0)}&\makecell[c]{(1036.4, 1.8)\\(3.7, 1.1)}&\makecell[c]{(1044.7, 3.1)\\(235.3, 38.5)}&\makecell[c]{(1031.4, 3.4)\\(0.0, 0.0)}&\makecell[c]{(1035.1, 1.7)\\(3.2, 0.8)}&\makecell[c]{(1045.3, 3.5)\\(254.8, 93.9)}&\makecell[c]{(959.1, 9.7)\\(0.0, 0.0)}&\makecell[c]{(1008.6, 8.6)\\(0.8, 0.2)}&\makecell[c]{(1043.2, 5.0)\\(65.4, 15.1)}&\makecell[c]{(1026.7, 3.1)\\(0.0, 0.0)}&\makecell[c]{(1035.4, 3.1)\\(7.1, 1.2)}&\makecell[c]{(1049.7, 3.3)\\(574.5, 123.2)}&\makecell[c]{(1027.9, 3.2)\\(0.0, 0.0)}&\makecell[c]{(1038.4, 2.3)\\(8.2, 1.5)}&\makecell[c]{(1042.0, 1.2)\\(692.8, 171.4)}&\makecell[c]{(1031.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(1041.4, 3.3)\\(5.7, 1.2)}&\makecell[c]{(1047.0, 0.0)\\(597.3, 122.9)}\\\hline
s3v70c1100-10&\makecell[c]{(1020.0, 5.1)\\(76.7, 9.7)}&\makecell[c]{(1035.6, 0.5)\\(319.9, 63.6)}&\makecell[c]{(1034.2, 2.8)\\(320.7, 68.4)}&\makecell[c]{(1035.6, 1.0)\\(304.2, 59.2)}&\makecell[c]{(961.1, 10.5)\\(0.0, 0.0)}&\makecell[c]{(996.7, 6.4)\\(3.1, 0.7)}&\makecell[c]{(1015.0, 4.7)\\(215.9, 31.5)}&\makecell[c]{(1016.9, 1.6)\\(0.0, 0.0)}&\makecell[c]{(1023.7, 2.3)\\(4.0, 0.8)}&\makecell[c]{(1037.0, 1.6)\\(247.8, 42.7)}&\makecell[c]{(1018.3, 1.6)\\(0.0, 0.0)}&\makecell[c]{(1023.6, 1.4)\\(3.4, 1.0)}&\makecell[c]{(1036.4, 1.9)\\(245.6, 47.6)}&\makecell[c]{(1019.6, 2.6)\\(0.0, 0.0)}&\makecell[c]{(1023.3, 1.6)\\(3.9, 0.9)}&\makecell[c]{(1037.2, 2.6)\\(240.3, 37.8)}&\makecell[c]{(963.2, 4.6)\\(0.0, 0.0)}&\makecell[c]{(1003.0, 6.5)\\(0.9, 0.0)}&\makecell[c]{(1038.7, 1.9)\\(66.1, 15.3)}&\makecell[c]{(1019.3, 3.7)\\(0.0, 0.0)}&\makecell[c]{(1028.2, 4.0)\\(8.8, 2.1)}&\makecell[c]{(1037.1, 2.7)\\(578.0, 127.2)}&\makecell[c]{(1015.8, 4.3)\\(0.0, 0.0)}&\makecell[c]{(1027.4, 1.6)\\(6.7, 1.4)}&\makecell[c]{(1030.5, 0.7)\\(674.9, 137.3)}&\makecell[c]{(1021.8, 3.2)\\(0.0, 0.0)}&\makecell[c]{(1031.1, 1.2)\\(7.3, 1.0)}&\makecell[c]{(1036.5, 0.5)\\(605.0, 131.2)}\\\hline
s3v70c1200-1&\makecell[c]{(1115.7, 3.8)\\(78.6, 15.0)}&\makecell[c]{(1124.1, 1.8)\\(333.5, 65.0)}&\makecell[c]{(1124.2, 2.0)\\(337.2, 74.6)}&\makecell[c]{(1126.2, 3.4)\\(333.4, 83.7)}&\makecell[c]{(1050.1, 11.8)\\(0.0, 0.0)}&\makecell[c]{(1084.8, 7.3)\\(3.5, 0.7)}&\makecell[c]{(1105.6, 5.0)\\(218.8, 34.6)}&\makecell[c]{(1114.7, 3.1)\\(0.0, 0.0)}&\makecell[c]{(1124.1, 3.2)\\(4.5, 1.0)}&\makecell[c]{(1128.6, 0.9)\\(259.3, 57.5)}&\makecell[c]{(1112.6, 2.1)\\(0.1, 0.0)}&\makecell[c]{(1125.1, 2.6)\\(5.1, 1.7)}&\makecell[c]{(1128.9, 2.1)\\(253.5, 51.8)}&\makecell[c]{(1114.4, 2.7)\\(0.0, 0.0)}&\makecell[c]{(1124.4, 2.9)\\(3.8, 0.9)}&\makecell[c]{(1129.1, 1.4)\\(255.2, 55.2)}&\makecell[c]{(1046.8, 9.2)\\(0.0, 0.0)}&\makecell[c]{(1091.8, 7.4)\\(0.9, 0.0)}&\makecell[c]{(1127.5, 3.7)\\(65.1, 11.0)}&\makecell[c]{(1114.6, 2.9)\\(0.0, 0.0)}&\makecell[c]{(1122.2, 2.3)\\(6.9, 1.3)}&\makecell[c]{(1128.9, 1.4)\\(602.4, 133.2)}&\makecell[c]{(1111.6, 3.3)\\(0.1, 0.0)}&\makecell[c]{(1119.8, 1.6)\\(8.5, 1.6)}&\makecell[c]{(1124.6, 1.4)\\(730.1, 185.2)}&\makecell[c]{(1115.6, 2.0)\\(0.1, 0.0)}&\makecell[c]{(1125.9, 0.3)\\(6.4, 1.8)}&\makecell[c]{(1126.4, 0.9)\\(638.3, 149.9)}\\\hline
s3v70c1200-2&\makecell[c]{(1111.4, 3.9)\\(80.3, 18.5)}&\makecell[c]{(1127.9, 1.1)\\(367.5, 46.3)}&\makecell[c]{(1127.3, 3.4)\\(335.2, 78.3)}&\makecell[c]{(1129.0, 0.0)\\(324.3, 75.0)}&\makecell[c]{(1048.4, 11.9)\\(0.0, 0.0)}&\makecell[c]{(1085.5, 7.7)\\(3.4, 0.7)}&\makecell[c]{(1106.2, 4.9)\\(221.7, 46.6)}&\makecell[c]{(1113.7, 3.6)\\(0.0, 0.0)}&\makecell[c]{(1126.5, 1.4)\\(5.7, 0.9)}&\makecell[c]{(1131.0, 1.2)\\(260.2, 60.7)}&\makecell[c]{(1108.0, 3.9)\\(0.1, 0.0)}&\makecell[c]{(1126.3, 1.0)\\(5.1, 0.1)}&\makecell[c]{(1130.8, 0.6)\\(261.2, 63.2)}&\makecell[c]{(1115.9, 1.9)\\(0.1, 0.0)}&\makecell[c]{(1126.6, 1.2)\\(4.9, 0.6)}&\makecell[c]{(1131.6, 0.9)\\(264.7, 70.9)}&\makecell[c]{(1046.2, 16.1)\\(0.0, 0.0)}&\makecell[c]{(1097.7, 7.4)\\(0.9, 0.0)}&\makecell[c]{(1128.9, 4.7)\\(65.7, 12.9)}&\makecell[c]{(1118.2, 4.9)\\(0.0, 0.0)}&\makecell[c]{(1127.1, 1.8)\\(6.7, 1.5)}&\makecell[c]{(1131.8, 0.7)\\(607.4, 135.8)}&\makecell[c]{(1112.6, 4.3)\\(0.1, 0.0)}&\makecell[c]{(1121.2, 3.0)\\(7.9, 1.4)}&\makecell[c]{(1126.7, 2.0)\\(712.6, 148.7)}&\makecell[c]{(1115.4, 3.0)\\(0.0, 0.0)}&\makecell[c]{(1126.4, 1.7)\\(7.9, 1.2)}&\makecell[c]{(1128.7, 0.5)\\(642.7, 154.5)}\\\hline
s3v70c1200-3&\makecell[c]{(1112.3, 2.8)\\(78.6, 16.1)}&\makecell[c]{(1122.0, 1.5)\\(343.3, 86.7)}&\makecell[c]{(1122.5, 1.0)\\(331.5, 75.6)}&\makecell[c]{(1126.0, 1.7)\\(333.9, 97.2)}&\makecell[c]{(1051.3, 12.3)\\(0.0, 0.0)}&\makecell[c]{(1085.1, 6.7)\\(3.2, 0.6)}&\makecell[c]{(1105.5, 4.8)\\(221.1, 41.4)}&\makecell[c]{(1108.7, 2.9)\\(0.0, 0.0)}&\makecell[c]{(1123.3, 2.8)\\(4.8, 0.6)}&\makecell[c]{(1129.3, 1.9)\\(265.9, 58.2)}&\makecell[c]{(1105.5, 1.6)\\(0.1, 0.0)}&\makecell[c]{(1122.0, 3.3)\\(4.5, 0.9)}&\makecell[c]{(1128.8, 1.4)\\(251.0, 49.2)}&\makecell[c]{(1113.0, 3.1)\\(0.0, 0.0)}&\makecell[c]{(1123.4, 2.7)\\(4.3, 0.7)}&\makecell[c]{(1128.9, 2.3)\\(256.8, 56.8)}&\makecell[c]{(1050.3, 8.5)\\(0.0, 0.0)}&\makecell[c]{(1097.4, 5.3)\\(0.9, 0.0)}&\makecell[c]{(1127.4, 3.9)\\(69.2, 17.3)}&\makecell[c]{(1109.2, 4.0)\\(0.0, 0.0)}&\makecell[c]{(1117.9, 2.9)\\(7.1, 1.4)}&\makecell[c]{(1127.6, 3.2)\\(605.0, 137.9)}&\makecell[c]{(1110.6, 4.5)\\(0.0, 0.0)}&\makecell[c]{(1121.7, 1.6)\\(7.2, 1.4)}&\makecell[c]{(1125.8, 0.9)\\(703.4, 158.4)}&\makecell[c]{(1114.6, 4.0)\\(0.0, 0.0)}&\makecell[c]{(1123.8, 1.5)\\(8.8, 0.2)}&\makecell[c]{(1127.8, 0.4)\\(627.1, 137.7)}\\\hline
s3v70c1200-4&\makecell[c]{(1114.1, 2.3)\\(79.4, 14.8)}&\makecell[c]{(1118.7, 2.0)\\(338.0, 75.4)}&\makecell[c]{(1122.2, 4.6)\\(341.2, 80.1)}&\makecell[c]{(1121.9, 1.9)\\(332.4, 80.8)}&\makecell[c]{(1049.4, 10.7)\\(0.0, 0.0)}&\makecell[c]{(1083.4, 6.4)\\(3.2, 0.6)}&\makecell[c]{(1104.4, 5.2)\\(220.3, 44.7)}&\makecell[c]{(1108.0, 3.0)\\(0.0, 0.0)}&\makecell[c]{(1118.0, 0.0)\\(4.9, 0.6)}&\makecell[c]{(1126.0, 1.7)\\(266.8, 69.7)}&\makecell[c]{(1109.1, 2.8)\\(0.1, 0.0)}&\makecell[c]{(1119.0, 2.0)\\(4.8, 0.7)}&\makecell[c]{(1125.9, 1.9)\\(251.7, 46.6)}&\makecell[c]{(1114.2, 1.5)\\(0.1, 0.0)}&\makecell[c]{(1119.3, 1.6)\\(6.3, 1.4)}&\makecell[c]{(1127.2, 1.7)\\(257.5, 62.0)}&\makecell[c]{(1047.4, 11.5)\\(0.0, 0.0)}&\makecell[c]{(1092.5, 7.8)\\(1.6, 0.0)}&\makecell[c]{(1126.3, 3.3)\\(66.0, 17.6)}&\makecell[c]{(1111.7, 4.7)\\(0.1, 0.0)}&\makecell[c]{(1121.7, 3.2)\\(7.9, 1.1)}&\makecell[c]{(1129.3, 2.6)\\(596.9, 122.9)}&\makecell[c]{(1111.0, 3.6)\\(0.1, 0.0)}&\makecell[c]{(1119.4, 1.4)\\(7.7, 1.5)}&\makecell[c]{(1124.0, 0.9)\\(704.5, 143.0)}&\makecell[c]{(1116.4, 4.9)\\(0.0, 0.0)}&\makecell[c]{(1122.5, 1.3)\\(7.6, 1.1)}&\makecell[c]{(1126.0, 0.9)\\(644.6, 164.4)}\\\hline
s3v70c1200-5&\makecell[c]{(1113.8, 4.8)\\(78.9, 18.5)}&\makecell[c]{(1123.5, 2.4)\\(336.6, 72.0)}&\makecell[c]{(1126.4, 1.9)\\(336.3, 83.9)}&\makecell[c]{(1124.0, 4.2)\\(333.8, 84.2)}&\makecell[c]{(1051.4, 11.4)\\(0.0, 0.0)}&\makecell[c]{(1085.7, 6.4)\\(3.2, 0.6)}&\makecell[c]{(1107.0, 5.8)\\(221.6, 42.7)}&\makecell[c]{(1114.6, 5.0)\\(0.0, 0.0)}&\makecell[c]{(1125.6, 1.9)\\(4.0, 0.9)}&\makecell[c]{(1129.8, 1.1)\\(260.6, 59.2)}&\makecell[c]{(1116.6, 3.4)\\(0.0, 0.0)}&\makecell[c]{(1125.1, 3.4)\\(4.9, 0.2)}&\makecell[c]{(1129.7, 1.7)\\(251.0, 46.2)}&\makecell[c]{(1122.2, 4.5)\\(0.0, 0.0)}&\makecell[c]{(1126.3, 1.8)\\(3.7, 1.1)}&\makecell[c]{(1129.7, 1.3)\\(252.3, 51.1)}&\makecell[c]{(1050.4, 13.9)\\(0.0, 0.0)}&\makecell[c]{(1093.5, 7.2)\\(0.8, 0.2)}&\makecell[c]{(1129.5, 4.5)\\(66.6, 12.8)}&\makecell[c]{(1115.4, 3.7)\\(0.0, 0.0)}&\makecell[c]{(1123.1, 2.2)\\(7.9, 3.0)}&\makecell[c]{(1132.9, 1.4)\\(606.5, 143.3)}&\makecell[c]{(1111.3, 4.6)\\(0.1, 0.0)}&\makecell[c]{(1122.0, 1.9)\\(8.7, 1.1)}&\makecell[c]{(1126.5, 1.3)\\(694.9, 136.0)}&\makecell[c]{(1119.5, 2.5)\\(0.0, 0.0)}&\makecell[c]{(1126.8, 1.6)\\(6.1, 1.4)}&\makecell[c]{(1130.5, 0.9)\\(634.7, 149.9)}\\\hline
s3v70c1200-6&\makecell[c]{(1112.6, 4.3)\\(78.8, 16.8)}&\makecell[c]{(1126.8, 0.7)\\(335.9, 70.8)}&\makecell[c]{(1123.0, 1.6)\\(346.5, 107.3)}&\makecell[c]{(1126.5, 1.7)\\(341.9, 61.4)}&\makecell[c]{(1050.8, 12.3)\\(0.0, 0.0)}&\makecell[c]{(1085.5, 6.7)\\(3.6, 0.6)}&\makecell[c]{(1105.5, 4.8)\\(221.7, 49.2)}&\makecell[c]{(1111.0, 2.2)\\(0.0, 0.0)}&\makecell[c]{(1123.2, 2.0)\\(5.1, 0.1)}&\makecell[c]{(1129.1, 0.5)\\(258.9, 56.6)}&\makecell[c]{(1100.5, 3.4)\\(0.1, 0.0)}&\makecell[c]{(1123.4, 2.3)\\(4.9, 0.5)}&\makecell[c]{(1128.4, 1.4)\\(255.1, 56.8)}&\makecell[c]{(1110.8, 2.3)\\(0.0, 0.0)}&\makecell[c]{(1122.4, 3.3)\\(3.6, 1.0)}&\makecell[c]{(1128.7, 1.2)\\(257.7, 50.5)}&\makecell[c]{(1048.9, 12.0)\\(0.0, 0.0)}&\makecell[c]{(1098.2, 2.6)\\(0.9, 0.1)}&\makecell[c]{(1125.7, 2.6)\\(69.1, 16.4)}&\makecell[c]{(1109.8, 2.4)\\(0.0, 0.0)}&\makecell[c]{(1118.1, 2.6)\\(7.0, 1.2)}&\makecell[c]{(1129.2, 3.1)\\(614.4, 158.9)}&\makecell[c]{(1109.3, 4.3)\\(0.1, 0.0)}&\makecell[c]{(1123.7, 1.0)\\(7.5, 1.6)}&\makecell[c]{(1128.2, 1.2)\\(777.3, 95.1)}&\makecell[c]{(1112.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(1123.8, 1.6)\\(7.8, 1.5)}&\makecell[c]{(1128.9, 0.7)\\(639.8, 151.3)}\\\hline
s3v70c1200-7&\makecell[c]{(1111.9, 3.3)\\(80.2, 18.4)}&\makecell[c]{(1121.2, 2.0)\\(336.1, 64.7)}&\makecell[c]{(1126.5, 2.7)\\(348.8, 96.4)}&\makecell[c]{(1123.6, 1.9)\\(333.5, 87.7)}&\makecell[c]{(1049.9, 11.3)\\(0.0, 0.0)}&\makecell[c]{(1085.8, 6.2)\\(3.7, 0.8)}&\makecell[c]{(1105.8, 5.0)\\(221.8, 46.8)}&\makecell[c]{(1114.7, 4.5)\\(0.0, 0.0)}&\makecell[c]{(1125.7, 3.3)\\(4.3, 1.0)}&\makecell[c]{(1131.0, 1.1)\\(262.2, 62.1)}&\makecell[c]{(1109.1, 4.9)\\(0.1, 0.0)}&\makecell[c]{(1124.4, 1.9)\\(4.6, 0.8)}&\makecell[c]{(1131.8, 2.1)\\(255.8, 53.6)}&\makecell[c]{(1116.9, 2.9)\\(0.0, 0.0)}&\makecell[c]{(1124.2, 1.7)\\(5.1, 0.2)}&\makecell[c]{(1130.8, 2.2)\\(256.4, 58.4)}&\makecell[c]{(1047.3, 11.5)\\(0.0, 0.0)}&\makecell[c]{(1093.3, 5.0)\\(0.9, 0.0)}&\makecell[c]{(1126.8, 4.9)\\(67.1, 14.8)}&\makecell[c]{(1110.4, 5.5)\\(0.0, 0.0)}&\makecell[c]{(1122.1, 2.3)\\(6.2, 1.3)}&\makecell[c]{(1133.3, 1.5)\\(609.9, 146.7)}&\makecell[c]{(1111.8, 4.1)\\(0.1, 0.0)}&\makecell[c]{(1121.9, 1.3)\\(9.6, 0.1)}&\makecell[c]{(1128.1, 1.6)\\(706.0, 154.2)}&\makecell[c]{(1118.6, 6.5)\\(0.0, 0.0)}&\makecell[c]{(1124.4, 2.9)\\(6.2, 1.6)}&\makecell[c]{(1130.6, 0.7)\\(663.9, 208.2)}\\\hline
s3v70c1200-8&\makecell[c]{(1114.8, 1.9)\\(79.8, 16.5)}&\makecell[c]{(1127.8, 2.6)\\(345.6, 82.8)}&\makecell[c]{(1125.6, 0.8)\\(333.5, 79.4)}&\makecell[c]{(1127.3, 1.3)\\(330.1, 81.2)}&\makecell[c]{(1050.5, 10.6)\\(0.0, 0.0)}&\makecell[c]{(1084.9, 7.0)\\(5.7, 1.3)}&\makecell[c]{(1107.6, 5.4)\\(237.2, 187.9)}&\makecell[c]{(1115.1, 1.9)\\(0.0, 0.0)}&\makecell[c]{(1125.2, 1.7)\\(4.2, 0.9)}&\makecell[c]{(1131.7, 1.7)\\(261.7, 57.0)}&\makecell[c]{(1106.9, 3.3)\\(0.0, 0.0)}&\makecell[c]{(1125.1, 2.1)\\(4.1, 1.1)}&\makecell[c]{(1132.3, 1.9)\\(252.0, 47.5)}&\makecell[c]{(1113.9, 2.3)\\(0.0, 0.0)}&\makecell[c]{(1125.5, 1.7)\\(4.4, 0.9)}&\makecell[c]{(1132.1, 1.7)\\(262.9, 69.3)}&\makecell[c]{(1048.0, 11.6)\\(0.0, 0.0)}&\makecell[c]{(1095.4, 8.5)\\(0.9, 0.0)}&\makecell[c]{(1128.5, 2.5)\\(70.5, 19.3)}&\makecell[c]{(1112.9, 4.0)\\(0.0, 0.0)}&\makecell[c]{(1121.8, 2.7)\\(8.2, 0.9)}&\makecell[c]{(1130.1, 1.8)\\(610.3, 155.9)}&\makecell[c]{(1115.8, 6.1)\\(0.1, 0.0)}&\makecell[c]{(1125.2, 2.0)\\(7.3, 1.2)}&\makecell[c]{(1129.4, 1.3)\\(722.7, 177.1)}&\makecell[c]{(1116.4, 3.8)\\(0.0, 0.0)}&\makecell[c]{(1125.3, 0.5)\\(8.3, 0.9)}&\makecell[c]{(1127.4, 0.7)\\(630.5, 148.9)}\\\hline
s3v70c1200-9&\makecell[c]{(1110.6, 5.0)\\(78.5, 13.2)}&\makecell[c]{(1127.9, 0.8)\\(346.1, 87.2)}&\makecell[c]{(1128.0, 2.0)\\(324.3, 59.5)}&\makecell[c]{(1127.2, 3.0)\\(327.5, 77.0)}&\makecell[c]{(1049.5, 11.7)\\(0.0, 0.0)}&\makecell[c]{(1084.4, 6.1)\\(3.1, 0.8)}&\makecell[c]{(1104.9, 5.4)\\(235.1, 159.3)}&\makecell[c]{(1107.8, 2.6)\\(0.0, 0.0)}&\makecell[c]{(1121.0, 2.2)\\(4.1, 1.2)}&\makecell[c]{(1128.9, 2.1)\\(259.2, 56.6)}&\makecell[c]{(1116.0, 2.7)\\(0.1, 0.0)}&\makecell[c]{(1121.0, 2.2)\\(3.2, 0.8)}&\makecell[c]{(1128.9, 2.1)\\(253.9, 53.4)}&\makecell[c]{(1122.2, 4.4)\\(0.0, 0.0)}&\makecell[c]{(1120.3, 2.1)\\(3.3, 0.9)}&\makecell[c]{(1128.9, 3.0)\\(256.9, 58.2)}&\makecell[c]{(1051.8, 8.0)\\(0.0, 0.0)}&\makecell[c]{(1089.1, 5.9)\\(0.9, 0.1)}&\makecell[c]{(1129.0, 5.7)\\(69.0, 22.0)}&\makecell[c]{(1107.4, 1.9)\\(0.1, 0.0)}&\makecell[c]{(1119.9, 5.8)\\(8.1, 0.4)}&\makecell[c]{(1136.6, 2.2)\\(623.8, 171.2)}&\makecell[c]{(1116.8, 4.3)\\(0.1, 0.0)}&\makecell[c]{(1123.6, 3.0)\\(6.4, 1.6)}&\makecell[c]{(1128.3, 2.1)\\(712.3, 168.5)}&\makecell[c]{(1127.9, 2.9)\\(0.0, 0.0)}&\makecell[c]{(1133.0, 0.0)\\(6.3, 1.7)}&\makecell[c]{(1133.0, 0.0)\\(632.3, 138.2)}\\\hline
s3v70c1200-10&\makecell[c]{(1116.2, 6.2)\\(81.2, 17.3)}&\makecell[c]{(1131.0, 1.3)\\(338.9, 73.0)}&\makecell[c]{(1124.0, 2.4)\\(343.8, 104.1)}&\makecell[c]{(1126.2, 1.8)\\(329.7, 77.5)}&\makecell[c]{(1047.0, 11.8)\\(0.0, 0.0)}&\makecell[c]{(1087.2, 6.4)\\(3.5, 0.8)}&\makecell[c]{(1106.2, 5.1)\\(220.9, 41.6)}&\makecell[c]{(1111.8, 1.9)\\(0.0, 0.0)}&\makecell[c]{(1123.7, 1.4)\\(4.1, 1.2)}&\makecell[c]{(1132.0, 1.6)\\(261.0, 56.7)}&\makecell[c]{(1112.3, 0.9)\\(0.0, 0.0)}&\makecell[c]{(1123.0, 1.2)\\(4.2, 1.1)}&\makecell[c]{(1131.3, 1.8)\\(263.6, 69.7)}&\makecell[c]{(1117.6, 1.6)\\(0.0, 0.0)}&\makecell[c]{(1123.7, 1.4)\\(4.3, 0.9)}&\makecell[c]{(1132.0, 1.6)\\(249.3, 43.5)}&\makecell[c]{(1046.2, 8.1)\\(0.0, 0.0)}&\makecell[c]{(1089.3, 6.5)\\(0.6, 0.2)}&\makecell[c]{(1127.2, 4.9)\\(70.0, 18.0)}&\makecell[c]{(1111.8, 3.7)\\(0.0, 0.0)}&\makecell[c]{(1122.9, 1.8)\\(7.3, 1.3)}&\makecell[c]{(1133.8, 1.2)\\(615.6, 116.6)}&\makecell[c]{(1112.7, 4.6)\\(0.1, 0.0)}&\makecell[c]{(1122.0, 1.8)\\(8.2, 1.8)}&\makecell[c]{(1127.2, 1.2)\\(726.9, 194.1)}&\makecell[c]{(1115.2, 4.1)\\(0.1, 0.0)}&\makecell[c]{(1122.6, 0.7)\\(7.4, 1.4)}&\makecell[c]{(1128.1, 2.1)\\(646.6, 175.0)}\\\hline




\end{tabular}


==> tables/max3sat70variable_sls.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
&WalkSat&$MCTS\_{WalkSat}$&\multicolumn{2}{c}{$NMC\_{WalkSat}$}&$NMC\_{Novelty}$&Best Solver\\
\hline
&flip=$10^{5.5}$&m=200&level 1, flip=$10^{3.5}$&level 2&level 1&-\\
\hline
statistic&\makecell[c]{(952.4, 0.5),(46.3, 7.8)}&\makecell[c]{(947.2, 2.4),(2702.5, 395.6)}&\makecell[c]{(952.0, 0.9),(35.7, 5.8)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&--&953.18\\\hline
s3v70c800-1&\makecell[c]{(769.0, 0.0),(44.3, 10.0)}&\makecell[c]{(763.9, 2.5),(2327.1, 114.0)}&\makecell[c]{(769.0, 0.0),(31.4, 2.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(767.0, 1.1),(153.4, 19.9)}&769\\\hline
s3v70c800-2&\makecell[c]{(765.4, 0.5),(40.9, 3.8)}&\makecell[c]{(759.7, 2.4),(2317.2, 110.6)}&\makecell[c]{(764.8, 1.0),(31.2, 4.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(764.0, 1.8),(153.3, 16.3)}&766\\\hline
s3v70c800-3&\makecell[c]{(770.0, 0.0),(44.6, 11.8)}&\makecell[c]{(766.5, 2.9),(2334.8, 122.3)}&\makecell[c]{(769.6, 0.5),(31.3, 4.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(768.1, 2.0),(148.2, 7.6)}&770\\\hline
s3v70c800-4&\makecell[c]{(772.0, 0.0),(40.9, 4.7)}&\makecell[c]{(766.0, 2.9),(2319.0, 111.0)}&\makecell[c]{(772.0, 0.0),(31.1, 3.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(769.1, 1.6),(149.0, 16.1)}&772\\\hline
s3v70c800-5&\makecell[c]{(768.2, 0.4),(41.4, 8.4)}&\makecell[c]{(763.9, 2.3),(2326.6, 120.0)}&\makecell[c]{(767.5, 0.5),(31.0, 3.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(767.6, 0.9),(151.4, 16.4)}&769\\\hline
s3v70c800-6&\makecell[c]{(770.0, 0.0),(40.8, 5.8)}&\makecell[c]{(762.9, 2.2),(2296.2, 111.7)}&\makecell[c]{(770.0, 0.0),(32.4, 4.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&770\\\hline
s3v70c800-7&\makecell[c]{(768.3, 0.5),(41.4, 6.1)}&\makecell[c]{(763.1, 3.0),(2297.5, 88.8)}&\makecell[c]{(768.2, 0.4),(30.9, 4.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(767.3, 1.6),(149.4, 16.4)}&769\\\hline
s3v70c800-8&\makecell[c]{(765.8, 0.4),(43.3, 6.4)}&\makecell[c]{(760.9, 2.0),(2323.4, 125.5)}&\makecell[c]{(765.3, 0.8),(32.7, 3.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(764.4, 1.6),(156.5, 22.7)}&766\\\hline
s3v70c800-9&\makecell[c]{(767.5, 0.5),(40.2, 2.6)}&\makecell[c]{(759.8, 3.0),(2314.9, 114.7)}&\makecell[c]{(766.3, 1.3),(31.6, 5.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(766.0, 1.1),(153.4, 16.8)}&768\\\hline
s3v70c800-10&\makecell[c]{(769.2, 0.4),(41.4, 5.4)}&\makecell[c]{(765.4, 1.9),(2322.1, 159.2)}&\makecell[c]{(769.1, 0.5),(33.6, 3.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(768.8, 0.7),(152.2, 16.7)}&770\\\hline
s3v70c900-1&\makecell[c]{(861.0, 0.0),(45.6, 7.6)}&\makecell[c]{(853.3, 1.3),(2532.9, 258.9)}&\makecell[c]{(860.2, 0.9),(35.2, 5.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(859.3, 1.1),(174.3, 31.1)}&861\\\hline
s3v70c900-2&\makecell[c]{(861.7, 0.5),(44.1, 6.9)}&\makecell[c]{(857.3, 2.5),(2571.2, 308.7)}&\makecell[c]{(861.5, 0.5),(33.1, 3.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(859.9, 1.4),(184.5, 21.0)}&862\\\hline
s3v70c900-3&\makecell[c]{(860.8, 0.4),(43.1, 4.7)}&\makecell[c]{(854.3, 2.5),(2524.0, 273.3)}&\makecell[c]{(860.2, 1.0),(32.8, 4.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(859.3, 2.1),(172.3, 30.4)}&861\\\hline
s3v70c900-4&\makecell[c]{(860.5, 0.5),(43.2, 8.3)}&\makecell[c]{(858.2, 1.0),(2516.2, 228.2)}&\makecell[c]{(859.5, 0.8),(34.3, 5.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(857.9, 1.5),(170.5, 25.2)}&861\\\hline
s3v70c900-5&\makecell[c]{(859.4, 0.5),(42.8, 5.0)}&\makecell[c]{(857.1, 0.5),(2528.1, 265.5)}&\makecell[c]{(858.9, 0.5),(33.1, 4.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(857.6, 1.9),(173.5, 28.3)}&860\\\hline
s3v70c900-6&\makecell[c]{(858.8, 0.4),(44.6, 7.4)}&\makecell[c]{(855.6, 2.7),(2524.6, 255.2)}&\makecell[c]{(857.9, 1.1),(34.5, 2.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(858.3, 1.0),(178.9, 38.6)}&859\\\hline
s3v70c900-7&\makecell[c]{(859.4, 0.7),(44.5, 7.4)}&\makecell[c]{(851.1, 2.6),(2495.8, 238.7)}&\makecell[c]{(859.1, 0.9),(35.5, 7.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(857.3, 2.1),(169.1, 24.5)}&860\\\hline
s3v70c900-8&\makecell[c]{(857.9, 0.3),(43.6, 4.6)}&\makecell[c]{(854.2, 1.6),(2486.9, 226.7)}&\makecell[c]{(857.4, 0.8),(33.2, 3.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(857.5, 0.9),(174.7, 33.4)}&858\\\hline
s3v70c900-9&\makecell[c]{(865.0, 0.0),(44.8, 10.4)}&\makecell[c]{(861.3, 1.1),(2546.1, 272.9)}&\makecell[c]{(864.9, 0.3),(32.2, 4.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(863.2, 1.1),(169.7, 21.8)}&865\\\hline
s3v70c900-10&\makecell[c]{(861.0, 0.0),(42.2, 3.5)}&\makecell[c]{(854.8, 2.5),(2526.9, 236.5)}&\makecell[c]{(859.8, 0.9),(34.6, 6.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(858.6, 1.7),(172.5, 27.3)}&861\\\hline
s3v70c1000-1&\makecell[c]{(953.0, 0.0),(48.3, 9.7)}&\makecell[c]{(947.0, 2.3),(2708.6, 438.2)}&\makecell[c]{(951.6, 1.4),(35.9, 7.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(951.4, 1.9),(188.3, 40.3)}&953\\\hline
s3v70c1000-2&\makecell[c]{(956.9, 0.3),(45.5, 6.2)}&\makecell[c]{(951.4, 2.2),(2677.3, 400.3)}&\makecell[c]{(956.5, 0.7),(35.0, 5.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(956.3, 1.8),(177.8, 30.3)}&957\\\hline
s3v70c1000-3&\makecell[c]{(954.5, 0.5),(45.4, 7.2)}&\makecell[c]{(947.4, 3.8),(2740.8, 475.4)}&\makecell[c]{(954.3, 1.4),(33.8, 3.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(952.9, 2.0),(192.2, 36.8)}&955\\\hline
s3v70c1000-4&\makecell[c]{(951.9, 0.8),(50.7, 4.4)}&\makecell[c]{(944.9, 4.0),(2747.2, 458.5)}&\makecell[c]{(951.2, 2.0),(34.4, 4.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(949.4, 1.9),(195.6, 45.6)}&953\\\hline
s3v70c1000-5&\makecell[c]{(957.7, 0.5),(43.6, 5.0)}&\makecell[c]{(951.5, 3.4),(2711.5, 422.7)}&\makecell[c]{(957.2, 0.6),(36.3, 6.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(955.7, 2.3),(189.5, 37.8)}&958\\\hline
s3v70c1000-6&\makecell[c]{(948.2, 0.6),(45.7, 6.8)}&\makecell[c]{(944.5, 3.1),(2730.1, 459.2)}&\makecell[c]{(947.8, 1.2),(37.1, 6.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(947.8, 1.7),(194.1, 35.5)}&950\\\hline
s3v70c1000-7&\makecell[c]{(949.6, 0.8),(46.1, 9.8)}&\makecell[c]{(944.2, 3.6),(2671.5, 396.0)}&\makecell[c]{(949.9, 1.4),(36.7, 7.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(949.0, 2.3),(189.7, 35.9)}&951\\\hline
s3v70c1000-8&\makecell[c]{(951.3, 0.5),(45.6, 8.1)}&\makecell[c]{(947.4, 1.5),(2722.9, 426.8)}&\makecell[c]{(951.3, 0.5),(36.3, 7.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(950.5, 1.1),(190.6, 37.5)}&952\\\hline
s3v70c1000-9&\makecell[c]{(949.5, 0.5),(44.7, 8.0)}&\makecell[c]{(944.5, 1.9),(2763.4, 473.7)}&\makecell[c]{(948.9, 0.5),(35.1, 4.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(948.8, 1.0),(197.2, 41.2)}&951\\\hline
s3v70c1000-10&\makecell[c]{(954.6, 0.5),(46.3, 8.3)}&\makecell[c]{(951.8, 3.2),(2679.9, 405.0)}&\makecell[c]{(954.6, 0.7),(35.7, 6.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(954.0, 1.3),(178.6, 29.4)}&955\\\hline
s3v70c1100-1&\makecell[c]{(1043.6, 0.5),(47.9, 10.2)}&\makecell[c]{(1034.8, 2.0),(2928.7, 582.8)}&\makecell[c]{(1043.0, 1.3),(37.4, 6.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1042.0, 1.6),(208.6, 50.2)}&1044\\\hline
s3v70c1100-2&\makecell[c]{(1044.0, 0.8),(47.4, 8.2)}&\makecell[c]{(1038.5, 2.2),(2912.4, 466.4)}&\makecell[c]{(1043.6, 1.1),(37.4, 6.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1043.7, 1.9),(205.2, 46.4)}&1045\\\hline
s3v70c1100-3&\makecell[c]{(1045.6, 0.5),(47.5, 8.5)}&\makecell[c]{(1041.0, 3.1),(2908.0, 421.9)}&\makecell[c]{(1045.4, 0.7),(36.1, 8.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1046.0, 1.5),(203.8, 43.0)}&1047\\\hline
s3v70c1100-4&\makecell[c]{(1047.3, 0.5),(47.4, 9.1)}&\makecell[c]{(1042.2, 2.9),(2877.6, 552.2)}&\makecell[c]{(1047.0, 0.4),(39.5, 8.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1046.7, 2.1),(209.1, 49.4)}&1048\\\hline
s3v70c1100-5&\makecell[c]{(1046.2, 0.4),(45.4, 7.0)}&\makecell[c]{(1038.2, 2.2),(2848.1, 537.0)}&\makecell[c]{(1045.9, 0.8),(37.7, 7.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1045.9, 0.7),(204.3, 44.9)}&1047\\\hline
s3v70c1100-6&\makecell[c]{(1044.6, 1.2),(48.0, 9.5)}&\makecell[c]{(1039.0, 3.3),(2919.3, 519.3)}&\makecell[c]{(1045.4, 1.5),(38.4, 8.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1044.1, 2.1),(209.2, 44.1)}&1047\\\hline
s3v70c1100-7&\makecell[c]{(1045.4, 0.8),(59.5, 9.4)}&\makecell[c]{(1038.7, 2.2),(2903.9, 561.3)}&\makecell[c]{(1045.7, 1.1),(36.7, 6.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1044.7, 2.3),(205.2, 40.9)}&1047\\\hline
s3v70c1100-8&\makecell[c]{(1047.9, 0.5),(46.6, 7.8)}&\makecell[c]{(1040.7, 1.9),(2879.1, 521.1)}&\makecell[c]{(1047.7, 1.6),(37.8, 7.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1046.0, 3.8),(208.9, 48.2)}&1049\\\hline
s3v70c1100-9&\makecell[c]{(1051.5, 0.5),(48.4, 10.2)}&\makecell[c]{(1049.9, 2.9),(2859.0, 535.3)}&\makecell[c]{(1051.7, 0.6),(35.7, 4.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1050.2, 2.9),(202.6, 43.2)}&1052\\\hline
s3v70c1100-10&\makecell[c]{(1041.1, 0.7),(49.2, 10.3)}&\makecell[c]{(1035.8, 2.6),(2973.7, 592.9)}&\makecell[c]{(1040.9, 0.9),(38.5, 4.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1040.7, 1.1),(214.3, 47.2)}&1042\\\hline
s3v70c1200-1&\makecell[c]{(1132.9, 0.9),(49.1, 10.0)}&\makecell[c]{(1126.9, 2.7),(3042.7, 612.5)}&\makecell[c]{(1132.3, 1.0),(41.8, 9.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1131.7, 1.7),(251.1, 52.9)}&1134\\\hline
s3v70c1200-2&\makecell[c]{(1135.4, 1.0),(49.6, 8.5)}&\makecell[c]{(1130.6, 2.4),(3026.8, 630.1)}&\makecell[c]{(1133.7, 1.2),(38.8, 7.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1135.1, 1.3),(227.6, 49.5)}&1137\\\hline
s3v70c1200-3&\makecell[c]{(1133.6, 0.5),(49.9, 7.7)}&\makecell[c]{(1129.7, 2.5),(3039.3, 621.1)}&\makecell[c]{(1133.3, 0.8),(41.6, 10.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1134.3, 1.3),(227.2, 52.1)}&1135\\\hline
s3v70c1200-4&\makecell[c]{(1131.8, 0.6),(49.1, 9.4)}&\makecell[c]{(1127.2, 3.9),(3070.5, 643.4)}&\makecell[c]{(1131.4, 1.4),(40.2, 8.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1131.9, 1.6),(226.4, 49.1)}&1133\\\hline
s3v70c1200-5&\makecell[c]{(1133.6, 0.7),(52.5, 12.2)}&\makecell[c]{(1129.1, 2.0),(3033.2, 636.7)}&\makecell[c]{(1133.8, 0.9),(39.1, 7.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1132.9, 1.1),(233.1, 49.6)}&1135\\\hline
s3v70c1200-6&\makecell[c]{(1132.4, 0.5),(49.7, 9.9)}&\makecell[c]{(1128.7, 1.8),(3072.4, 682.4)}&\makecell[c]{(1131.9, 1.8),(38.3, 6.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1133.0, 1.5),(226.4, 52.8)}&1134\\\hline
s3v70c1200-7&\makecell[c]{(1137.2, 0.7),(50.2, 11.4)}&\makecell[c]{(1128.2, 2.4),(3047.7, 641.4)}&\makecell[c]{(1136.5, 1.7),(39.5, 8.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1135.9, 1.5),(230.5, 54.5)}&1138\\\hline
s3v70c1200-8&\makecell[c]{(1134.6, 1.3),(50.5, 11.0)}&\makecell[c]{(1130.8, 1.3),(3087.1, 642.5)}&\makecell[c]{(1133.4, 2.1),(39.0, 7.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1134.1, 2.1),(230.1, 53.8)}&1137\\\hline
s3v70c1200-9&\makecell[c]{(1138.2, 0.7),(52.7, 13.1)}&\makecell[c]{(1134.4, 1.3),(3033.3, 613.1)}&\makecell[c]{(1137.6, 1.5),(41.4, 4.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1137.3, 1.7),(227.1, 51.7)}&1139\\\hline
s3v70c1200-10&\makecell[c]{(1135.7, 0.6),(57.3, 4.5)}&\makecell[c]{(1132.6, 1.1),(3077.5, 669.7)}&\makecell[c]{(1134.6, 1.7),(39.9, 7.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(1134.5, 3.2),(229.1, 56.7)}&1137\\\hline



\end{tabular}


==> tables/max3sat80variable.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
&MCTS&$MCTS\_{H1}$&$MCTS\_{H2}$&$MCTS\_{H3}$&\multicolumn{3}{c}{NMC}&\multicolumn{3}{c}{$NMC\_{H1}$}&\multicolumn{3}{c}{$NMC\_{H2}$}&\multicolumn{3}{c}{$NMC\_{H3}$}&\multicolumn{3}{c}{NRPA}&\multicolumn{3}{c}{$GNRPA\_{H1}$}&\multicolumn{3}{c}{$GNRPA\_{H2}$}&\multicolumn{3}{c}{$GNRPA\_{H3}$}\\
\hline
&m=200&m=200&m=200&m=200&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2\\
\hline
statistic&\makecell[c]{(736.1, 3.3)\\(73.7, 13.0)}&\makecell[c]{(745.3, 1.1)\\(282.1, 45.6)}&\makecell[c]{(745.4, 1.7)\\(261.8, 44.7)}&\makecell[c]{(746.9, 1.7)\\(251.3, 38.0)}&\makecell[c]{(682.5, 9.0)\\(0.0, 0.0)}&\makecell[c]{(711.4, 5.5)\\(2.5, 0.7)}&\makecell[c]{(728.4, 3.9)\\(196.4, 31.4)}&\makecell[c]{(732.8, 2.3)\\(0.0, 0.0)}&\makecell[c]{(743.0, 2.0)\\(3.3, 0.7)}&\makecell[c]{(748.8, 1.3)\\(233.5, 37.8)}&\makecell[c]{(734.6, 2.2)\\(0.0, 0.0)}&\makecell[c]{(743.0, 2.0)\\(3.4, 0.7)}&\makecell[c]{(748.6, 1.4)\\(231.1, 42.6)}&\makecell[c]{(738.9, 2.3)\\(0.0, 0.0)}&\makecell[c]{(742.8, 1.9)\\(3.6, 0.6)}&\makecell[c]{(748.7, 1.3)\\(229.9, 41.1)}&\makecell[c]{(682.9, 8.6)\\(0.0, 0.0)}&\makecell[c]{(718.9, 5.1)\\(0.6, 0.0)}&\makecell[c]{(746.8, 2.9)\\(53.6, 8.6)}&\makecell[c]{(732.3, 3.3)\\(0.0, 0.0)}&\makecell[c]{(740.8, 2.1)\\(5.0, 0.8)}&\makecell[c]{(749.2, 1.6)\\(467.5, 54.6)}&\makecell[c]{(734.2, 3.0)\\(0.0, 0.0)}&\makecell[c]{(741.7, 1.5)\\(5.7, 1.1)}&\makecell[c]{(745.9, 1.0)\\(561.1, 88.4)}&\makecell[c]{(738.7, 2.3)\\(0.0, 0.0)}&\makecell[c]{(744.3, 1.2)\\(5.0, 1.1)}&\makecell[c]{(747.3, 0.6)\\(492.0, 59.5)}\\\hline
s3v80c600-1&\makecell[c]{(567.8, 2.2)\\(68.1, 8.4)}&\makecell[c]{(575.7, 2.2)\\(232.6, 22.1)}&\makecell[c]{(581.6, 2.1)\\(211.4, 13.1)}&\makecell[c]{(577.5, 0.8)\\(180.4, 20.1)}&\makecell[c]{(525.7, 7.4)\\(0.0, 0.0)}&\makecell[c]{(550.1, 4.4)\\(2.0, 0.6)}&\makecell[c]{(564.6, 3.2)\\(163.3, 21.8)}&\makecell[c]{(568.4, 3.6)\\(0.0, 0.0)}&\makecell[c]{(577.5, 2.3)\\(3.1, 0.0)}&\makecell[c]{(579.8, 0.6)\\(202.0, 19.5)}&\makecell[c]{(568.3, 1.7)\\(0.0, 0.0)}&\makecell[c]{(577.9, 2.4)\\(4.1, 0.9)}&\makecell[c]{(579.8, 0.4)\\(195.1, 30.1)}&\makecell[c]{(571.2, 1.2)\\(0.0, 0.0)}&\makecell[c]{(578.5, 1.5)\\(2.9, 0.2)}&\makecell[c]{(579.8, 0.7)\\(201.7, 34.9)}&\makecell[c]{(525.8, 6.8)\\(0.0, 0.0)}&\makecell[c]{(555.1, 5.9)\\(0.5, 0.0)}&\makecell[c]{(578.4, 1.9)\\(45.0, 6.4)}&\makecell[c]{(568.3, 2.6)\\(0.0, 0.0)}&\makecell[c]{(575.4, 1.1)\\(3.8, 0.9)}&\makecell[c]{(579.9, 0.5)\\(377.7, 16.0)}&\makecell[c]{(566.7, 2.0)\\(0.0, 0.0)}&\makecell[c]{(573.0, 0.8)\\(4.6, 1.0)}&\makecell[c]{(574.9, 0.7)\\(529.9, 152.5)}&\makecell[c]{(571.8, 1.2)\\(0.0, 0.0)}&\makecell[c]{(574.2, 1.0)\\(4.1, 1.0)}&\makecell[c]{(575.5, 0.9)\\(396.6, 17.5)}\\\hline
s3v80c600-2&\makecell[c]{(569.8, 3.3)\\(64.4, 6.3)}&\makecell[c]{(576.1, 0.5)\\(232.4, 15.2)}&\makecell[c]{(576.8, 0.7)\\(186.5, 18.9)}&\makecell[c]{(577.9, 1.9)\\(194.1, 15.1)}&\makecell[c]{(525.4, 7.4)\\(0.0, 0.0)}&\makecell[c]{(549.8, 4.9)\\(2.1, 0.6)}&\makecell[c]{(563.0, 2.7)\\(159.9, 10.2)}&\makecell[c]{(566.3, 2.0)\\(0.0, 0.0)}&\makecell[c]{(575.6, 1.7)\\(2.5, 0.6)}&\makecell[c]{(580.5, 0.8)\\(199.1, 15.4)}&\makecell[c]{(570.3, 2.1)\\(0.0, 0.0)}&\makecell[c]{(575.7, 0.6)\\(2.6, 0.6)}&\makecell[c]{(580.1, 0.9)\\(190.3, 20.2)}&\makecell[c]{(570.7, 0.9)\\(0.0, 0.0)}&\makecell[c]{(575.7, 1.4)\\(4.4, 0.7)}&\makecell[c]{(580.5, 0.5)\\(196.0, 20.8)}&\makecell[c]{(523.8, 8.8)\\(0.0, 0.0)}&\makecell[c]{(556.0, 5.2)\\(0.5, 0.0)}&\makecell[c]{(577.7, 2.5)\\(44.0, 5.6)}&\makecell[c]{(564.5, 1.6)\\(0.0, 0.0)}&\makecell[c]{(574.6, 1.9)\\(4.6, 2.1)}&\makecell[c]{(580.1, 0.9)\\(384.4, 25.6)}&\makecell[c]{(566.2, 3.0)\\(0.0, 0.0)}&\makecell[c]{(575.7, 2.0)\\(3.2, 0.8)}&\makecell[c]{(577.9, 0.5)\\(480.7, 45.8)}&\makecell[c]{(569.3, 1.6)\\(0.0, 0.0)}&\makecell[c]{(576.1, 1.3)\\(4.8, 0.1)}&\makecell[c]{(578.2, 0.6)\\(415.2, 55.1)}\\\hline
s3v80c600-3&\makecell[c]{(572.5, 2.2)\\(70.0, 17.9)}&\makecell[c]{(577.3, 0.6)\\(222.9, 18.5)}&\makecell[c]{(580.2, 1.7)\\(184.8, 17.2)}&\makecell[c]{(579.4, 1.3)\\(193.0, 18.9)}&\makecell[c]{(524.6, 7.6)\\(0.0, 0.0)}&\makecell[c]{(551.2, 4.4)\\(1.8, 0.5)}&\makecell[c]{(566.3, 3.5)\\(161.5, 10.6)}&\makecell[c]{(568.6, 1.6)\\(0.0, 0.0)}&\makecell[c]{(573.7, 2.5)\\(2.6, 0.6)}&\makecell[c]{(584.1, 2.0)\\(198.4, 18.2)}&\makecell[c]{(574.1, 1.4)\\(0.0, 0.0)}&\makecell[c]{(576.1, 4.4)\\(2.6, 0.6)}&\makecell[c]{(583.9, 1.8)\\(201.0, 22.1)}&\makecell[c]{(574.6, 0.7)\\(0.0, 0.0)}&\makecell[c]{(574.4, 2.7)\\(3.0, 0.1)}&\makecell[c]{(584.9, 1.4)\\(200.6, 17.3)}&\makecell[c]{(525.5, 6.7)\\(0.0, 0.0)}&\makecell[c]{(557.4, 6.0)\\(0.4, 0.1)}&\makecell[c]{(581.0, 2.6)\\(49.9, 8.9)}&\makecell[c]{(565.7, 3.2)\\(0.0, 0.0)}&\makecell[c]{(573.0, 2.0)\\(4.4, 0.7)}&\makecell[c]{(584.5, 2.0)\\(388.0, 32.1)}&\makecell[c]{(571.0, 2.3)\\(0.0, 0.0)}&\makecell[c]{(576.0, 0.8)\\(4.6, 1.0)}&\makecell[c]{(579.2, 0.7)\\(460.1, 46.6)}&\makecell[c]{(575.4, 0.9)\\(0.0, 0.0)}&\makecell[c]{(578.4, 0.8)\\(4.1, 1.7)}&\makecell[c]{(580.8, 0.9)\\(414.1, 19.1)}\\\hline
s3v80c600-4&\makecell[c]{(573.8, 3.5)\\(67.5, 10.0)}&\makecell[c]{(578.7, 0.9)\\(220.5, 20.4)}&\makecell[c]{(579.0, 0.8)\\(207.9, 29.4)}&\makecell[c]{(579.8, 1.2)\\(202.6, 29.1)}&\makecell[c]{(524.5, 8.5)\\(0.0, 0.0)}&\makecell[c]{(551.2, 5.4)\\(1.7, 0.5)}&\makecell[c]{(565.3, 3.3)\\(161.0, 11.7)}&\makecell[c]{(567.7, 1.7)\\(0.0, 0.0)}&\makecell[c]{(577.9, 2.0)\\(2.9, 0.0)}&\makecell[c]{(581.8, 1.4)\\(192.5, 16.4)}&\makecell[c]{(570.9, 1.5)\\(0.0, 0.0)}&\makecell[c]{(576.1, 1.6)\\(2.2, 0.8)}&\makecell[c]{(582.0, 0.8)\\(188.9, 24.1)}&\makecell[c]{(576.1, 3.3)\\(0.0, 0.0)}&\makecell[c]{(577.3, 1.1)\\(2.8, 0.5)}&\makecell[c]{(581.5, 1.1)\\(191.3, 16.7)}&\makecell[c]{(524.2, 6.8)\\(0.0, 0.0)}&\makecell[c]{(559.9, 6.7)\\(0.6, 0.0)}&\makecell[c]{(580.4, 3.3)\\(42.6, 4.0)}&\makecell[c]{(569.1, 3.3)\\(0.0, 0.0)}&\makecell[c]{(575.8, 2.4)\\(4.4, 0.0)}&\makecell[c]{(582.5, 0.9)\\(382.2, 17.8)}&\makecell[c]{(568.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(576.7, 2.1)\\(5.3, 0.1)}&\makecell[c]{(580.8, 1.1)\\(452.5, 50.7)}&\makecell[c]{(574.7, 1.3)\\(0.0, 0.0)}&\makecell[c]{(578.7, 1.3)\\(3.6, 1.0)}&\makecell[c]{(583.1, 0.8)\\(405.9, 26.8)}\\\hline
s3v80c600-5&\makecell[c]{(576.8, 3.5)\\(68.0, 14.8)}&\makecell[c]{(586.0, 0.0)\\(235.5, 19.5)}&\makecell[c]{(580.4, 0.5)\\(206.6, 31.4)}&\makecell[c]{(581.2, 0.7)\\(187.2, 16.9)}&\makecell[c]{(525.3, 8.7)\\(0.0, 0.0)}&\makecell[c]{(550.5, 4.5)\\(1.6, 0.7)}&\makecell[c]{(565.9, 3.2)\\(156.1, 9.1)}&\makecell[c]{(570.9, 2.4)\\(0.0, 0.0)}&\makecell[c]{(579.3, 1.3)\\(2.5, 0.6)}&\makecell[c]{(586.0, 0.0)\\(203.4, 17.0)}&\makecell[c]{(569.1, 2.5)\\(0.0, 0.0)}&\makecell[c]{(579.3, 0.6)\\(3.0, 0.0)}&\makecell[c]{(585.9, 0.3)\\(190.7, 25.8)}&\makecell[c]{(573.8, 1.0)\\(0.0, 0.0)}&\makecell[c]{(579.1, 0.3)\\(1.9, 0.7)}&\makecell[c]{(586.0, 0.0)\\(186.4, 15.9)}&\makecell[c]{(523.4, 7.1)\\(0.0, 0.0)}&\makecell[c]{(556.3, 3.4)\\(0.4, 0.1)}&\makecell[c]{(580.8, 1.9)\\(45.5, 6.2)}&\makecell[c]{(573.3, 3.7)\\(0.0, 0.0)}&\makecell[c]{(579.7, 1.7)\\(3.9, 0.6)}&\makecell[c]{(584.6, 0.9)\\(376.6, 20.2)}&\makecell[c]{(569.6, 2.0)\\(0.0, 0.0)}&\makecell[c]{(576.0, 2.2)\\(5.1, 0.5)}&\makecell[c]{(580.1, 0.9)\\(455.7, 36.7)}&\makecell[c]{(573.5, 1.6)\\(0.0, 0.0)}&\makecell[c]{(577.7, 0.5)\\(4.1, 0.8)}&\makecell[c]{(581.0, 0.8)\\(397.6, 23.1)}\\\hline
s3v80c600-6&\makecell[c]{(570.0, 2.0)\\(68.9, 9.9)}&\makecell[c]{(575.0, 1.7)\\(216.8, 13.6)}&\makecell[c]{(580.0, 0.0)\\(219.1, 30.7)}&\makecell[c]{(582.4, 1.2)\\(183.8, 15.0)}&\makecell[c]{(524.5, 7.8)\\(0.0, 0.0)}&\makecell[c]{(548.4, 4.7)\\(2.0, 0.6)}&\makecell[c]{(562.8, 3.2)\\(157.8, 8.5)}&\makecell[c]{(568.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(576.7, 1.3)\\(2.6, 0.5)}&\makecell[c]{(580.9, 1.0)\\(192.0, 19.4)}&\makecell[c]{(566.2, 1.3)\\(0.0, 0.0)}&\makecell[c]{(577.0, 1.0)\\(1.6, 0.3)}&\makecell[c]{(580.4, 0.8)\\(204.4, 18.6)}&\makecell[c]{(570.6, 1.8)\\(0.0, 0.0)}&\makecell[c]{(576.1, 1.6)\\(3.9, 1.5)}&\makecell[c]{(581.0, 1.4)\\(195.0, 20.7)}&\makecell[c]{(525.8, 8.0)\\(0.0, 0.0)}&\makecell[c]{(558.0, 3.0)\\(0.5, 0.0)}&\makecell[c]{(577.8, 2.1)\\(45.5, 4.4)}&\makecell[c]{(568.9, 3.6)\\(0.0, 0.0)}&\makecell[c]{(575.2, 0.7)\\(4.4, 0.1)}&\makecell[c]{(581.2, 1.6)\\(387.6, 23.6)}&\makecell[c]{(567.5, 2.4)\\(0.0, 0.0)}&\makecell[c]{(575.6, 1.0)\\(4.2, 1.1)}&\makecell[c]{(579.1, 0.5)\\(457.9, 46.1)}&\makecell[c]{(571.0, 2.1)\\(0.0, 0.0)}&\makecell[c]{(575.3, 1.1)\\(4.0, 1.1)}&\makecell[c]{(578.7, 0.8)\\(411.1, 21.4)}\\\hline
s3v80c600-7&\makecell[c]{(572.3, 2.3)\\(66.0, 5.3)}&\makecell[c]{(579.4, 1.8)\\(267.3, 55.0)}&\makecell[c]{(583.8, 1.8)\\(204.1, 18.5)}&\makecell[c]{(580.2, 2.4)\\(191.4, 15.4)}&\makecell[c]{(524.2, 9.0)\\(0.0, 0.0)}&\makecell[c]{(550.3, 4.6)\\(1.7, 0.5)}&\makecell[c]{(565.2, 3.5)\\(160.5, 9.6)}&\makecell[c]{(563.9, 2.5)\\(0.0, 0.0)}&\makecell[c]{(574.2, 1.9)\\(2.7, 0.6)}&\makecell[c]{(581.4, 2.0)\\(191.2, 17.8)}&\makecell[c]{(571.9, 2.4)\\(0.0, 0.0)}&\makecell[c]{(574.5, 2.0)\\(2.7, 0.5)}&\makecell[c]{(580.9, 2.1)\\(186.2, 12.9)}&\makecell[c]{(577.8, 2.6)\\(0.0, 0.0)}&\makecell[c]{(574.1, 1.6)\\(3.0, 0.1)}&\makecell[c]{(580.3, 1.4)\\(195.8, 19.3)}&\makecell[c]{(520.9, 7.5)\\(0.0, 0.0)}&\makecell[c]{(556.7, 3.9)\\(0.5, 0.0)}&\makecell[c]{(581.8, 1.5)\\(48.7, 11.9)}&\makecell[c]{(565.9, 3.9)\\(0.0, 0.0)}&\makecell[c]{(573.6, 1.6)\\(4.5, 0.1)}&\makecell[c]{(581.5, 2.5)\\(408.9, 37.9)}&\makecell[c]{(569.4, 2.3)\\(0.0, 0.0)}&\makecell[c]{(576.6, 1.5)\\(4.3, 1.0)}&\makecell[c]{(582.6, 1.3)\\(478.2, 39.1)}&\makecell[c]{(575.6, 2.5)\\(0.0, 0.0)}&\makecell[c]{(580.2, 1.0)\\(4.4, 0.7)}&\makecell[c]{(582.1, 0.3)\\(403.0, 9.6)}\\\hline
s3v80c600-8&\makecell[c]{(569.7, 3.6)\\(65.2, 5.7)}&\makecell[c]{(574.9, 0.5)\\(252.4, 41.4)}&\makecell[c]{(575.7, 1.7)\\(209.1, 26.7)}&\makecell[c]{(580.6, 2.8)\\(191.9, 11.8)}&\makecell[c]{(525.0, 8.3)\\(0.0, 0.0)}&\makecell[c]{(549.1, 4.7)\\(1.7, 0.6)}&\makecell[c]{(564.2, 3.3)\\(166.5, 11.7)}&\makecell[c]{(565.9, 1.9)\\(0.0, 0.0)}&\makecell[c]{(573.3, 1.5)\\(2.6, 0.6)}&\makecell[c]{(576.5, 0.8)\\(204.8, 16.0)}&\makecell[c]{(569.8, 1.6)\\(0.0, 0.0)}&\makecell[c]{(573.7, 1.4)\\(2.9, 0.3)}&\makecell[c]{(577.7, 2.1)\\(198.2, 15.7)}&\makecell[c]{(571.3, 1.5)\\(0.0, 0.0)}&\makecell[c]{(573.9, 1.8)\\(3.1, 0.1)}&\makecell[c]{(577.7, 1.6)\\(177.3, 12.8)}&\makecell[c]{(525.3, 8.2)\\(0.0, 0.0)}&\makecell[c]{(553.4, 4.5)\\(0.5, 0.0)}&\makecell[c]{(579.4, 2.5)\\(46.3, 11.0)}&\makecell[c]{(563.4, 1.7)\\(0.0, 0.0)}&\makecell[c]{(570.2, 2.0)\\(3.3, 0.9)}&\makecell[c]{(579.2, 1.2)\\(372.1, 16.4)}&\makecell[c]{(568.1, 1.8)\\(0.0, 0.0)}&\makecell[c]{(573.5, 1.1)\\(4.4, 1.1)}&\makecell[c]{(576.0, 0.6)\\(469.5, 51.4)}&\makecell[c]{(572.8, 1.5)\\(0.0, 0.0)}&\makecell[c]{(576.0, 0.0)\\(4.3, 0.8)}&\makecell[c]{(576.1, 0.3)\\(413.6, 32.3)}\\\hline
s3v80c600-9&\makecell[c]{(570.9, 2.8)\\(63.6, 6.7)}&\makecell[c]{(581.7, 1.2)\\(231.4, 21.7)}&\makecell[c]{(581.0, 0.0)\\(189.9, 17.5)}&\makecell[c]{(583.6, 1.8)\\(196.8, 18.5)}&\makecell[c]{(525.0, 8.2)\\(0.0, 0.0)}&\makecell[c]{(551.2, 5.0)\\(1.8, 0.6)}&\makecell[c]{(567.1, 3.4)\\(160.5, 9.0)}&\makecell[c]{(572.5, 0.8)\\(0.0, 0.0)}&\makecell[c]{(577.9, 1.4)\\(2.9, 0.4)}&\makecell[c]{(581.6, 0.8)\\(199.0, 16.0)}&\makecell[c]{(573.0, 1.3)\\(0.0, 0.0)}&\makecell[c]{(576.7, 1.2)\\(2.2, 0.7)}&\makecell[c]{(582.7, 1.6)\\(188.9, 13.7)}&\makecell[c]{(577.3, 2.9)\\(0.0, 0.0)}&\makecell[c]{(577.0, 1.9)\\(2.7, 0.5)}&\makecell[c]{(583.1, 0.8)\\(198.2, 19.9)}&\makecell[c]{(528.2, 9.3)\\(0.0, 0.0)}&\makecell[c]{(557.5, 5.7)\\(0.3, 0.1)}&\makecell[c]{(580.4, 2.5)\\(44.8, 5.9)}&\makecell[c]{(568.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(574.5, 2.4)\\(4.4, 0.6)}&\makecell[c]{(584.4, 1.7)\\(386.8, 37.8)}&\makecell[c]{(572.2, 2.2)\\(0.0, 0.0)}&\makecell[c]{(576.8, 1.2)\\(4.8, 1.0)}&\makecell[c]{(580.8, 1.2)\\(478.4, 61.0)}&\makecell[c]{(576.2, 1.8)\\(0.0, 0.0)}&\makecell[c]{(579.5, 0.7)\\(3.8, 0.8)}&\makecell[c]{(580.7, 0.9)\\(406.4, 22.5)}\\\hline
s3v80c600-10&\makecell[c]{(571.8, 2.5)\\(66.6, 5.2)}&\makecell[c]{(576.5, 1.1)\\(233.0, 50.8)}&\makecell[c]{(576.7, 1.3)\\(218.3, 21.0)}&\makecell[c]{(578.2, 0.4)\\(195.2, 23.1)}&\makecell[c]{(525.1, 9.0)\\(0.0, 0.0)}&\makecell[c]{(548.3, 4.6)\\(2.1, 0.6)}&\makecell[c]{(563.1, 3.3)\\(173.3, 12.6)}&\makecell[c]{(569.9, 1.6)\\(0.0, 0.0)}&\makecell[c]{(576.3, 1.9)\\(2.9, 0.0)}&\makecell[c]{(581.1, 1.6)\\(189.7, 9.5)}&\makecell[c]{(568.6, 2.2)\\(0.0, 0.0)}&\makecell[c]{(576.2, 1.2)\\(3.0, 0.0)}&\makecell[c]{(581.3, 1.3)\\(185.6, 14.4)}&\makecell[c]{(568.3, 1.6)\\(0.0, 0.0)}&\makecell[c]{(576.6, 1.4)\\(2.5, 0.6)}&\makecell[c]{(580.9, 1.3)\\(185.2, 18.6)}&\makecell[c]{(525.8, 6.5)\\(0.0, 0.0)}&\makecell[c]{(556.4, 4.3)\\(0.5, 0.0)}&\makecell[c]{(578.3, 3.3)\\(44.3, 3.3)}&\makecell[c]{(569.3, 3.0)\\(0.0, 0.0)}&\makecell[c]{(576.8, 2.1)\\(3.9, 0.7)}&\makecell[c]{(580.9, 1.9)\\(406.4, 30.6)}&\makecell[c]{(569.8, 1.9)\\(0.0, 0.0)}&\makecell[c]{(573.9, 2.3)\\(4.4, 1.0)}&\makecell[c]{(577.9, 1.0)\\(472.6, 68.5)}&\makecell[c]{(570.2, 1.8)\\(0.0, 0.0)}&\makecell[c]{(577.0, 1.0)\\(3.1, 0.9)}&\makecell[c]{(580.5, 1.0)\\(411.3, 24.8)}\\\hline
s3v80c600-1&\makecell[c]{(567.8, 2.2)\\(68.1, 8.4)}&\makecell[c]{(575.7, 2.2)\\(232.6, 22.1)}&\makecell[c]{(581.6, 2.1)\\(211.4, 13.1)}&\makecell[c]{(577.5, 0.8)\\(180.4, 20.1)}&\makecell[c]{(525.7, 7.4)\\(0.0, 0.0)}&\makecell[c]{(550.1, 4.4)\\(2.0, 0.6)}&\makecell[c]{(564.6, 3.2)\\(163.3, 21.8)}&\makecell[c]{(568.4, 3.6)\\(0.0, 0.0)}&\makecell[c]{(577.5, 2.3)\\(3.1, 0.0)}&\makecell[c]{(579.8, 0.6)\\(202.0, 19.5)}&\makecell[c]{(568.3, 1.7)\\(0.0, 0.0)}&\makecell[c]{(577.9, 2.4)\\(4.1, 0.9)}&\makecell[c]{(579.8, 0.4)\\(195.1, 30.1)}&\makecell[c]{(571.2, 1.2)\\(0.0, 0.0)}&\makecell[c]{(578.5, 1.5)\\(2.9, 0.2)}&\makecell[c]{(579.8, 0.7)\\(201.7, 34.9)}&\makecell[c]{(525.8, 6.8)\\(0.0, 0.0)}&\makecell[c]{(555.1, 5.9)\\(0.5, 0.0)}&\makecell[c]{(578.4, 1.9)\\(45.0, 6.4)}&\makecell[c]{(568.3, 2.6)\\(0.0, 0.0)}&\makecell[c]{(575.4, 1.1)\\(3.8, 0.9)}&\makecell[c]{(579.9, 0.5)\\(377.7, 16.0)}&\makecell[c]{(566.7, 2.0)\\(0.0, 0.0)}&\makecell[c]{(573.0, 0.8)\\(4.6, 1.0)}&\makecell[c]{(574.9, 0.7)\\(529.9, 152.5)}&\makecell[c]{(571.8, 1.2)\\(0.0, 0.0)}&\makecell[c]{(574.2, 1.0)\\(4.1, 1.0)}&\makecell[c]{(575.5, 0.9)\\(396.6, 17.5)}\\\hline
s3v80c600-2&\makecell[c]{(569.8, 3.3)\\(64.4, 6.3)}&\makecell[c]{(576.1, 0.5)\\(232.4, 15.2)}&\makecell[c]{(576.8, 0.7)\\(186.5, 18.9)}&\makecell[c]{(577.9, 1.9)\\(194.1, 15.1)}&\makecell[c]{(525.4, 7.4)\\(0.0, 0.0)}&\makecell[c]{(549.8, 4.9)\\(2.1, 0.6)}&\makecell[c]{(563.0, 2.7)\\(159.9, 10.2)}&\makecell[c]{(566.3, 2.0)\\(0.0, 0.0)}&\makecell[c]{(575.6, 1.7)\\(2.5, 0.6)}&\makecell[c]{(580.5, 0.8)\\(199.1, 15.4)}&\makecell[c]{(570.3, 2.1)\\(0.0, 0.0)}&\makecell[c]{(575.7, 0.6)\\(2.6, 0.6)}&\makecell[c]{(580.1, 0.9)\\(190.3, 20.2)}&\makecell[c]{(570.7, 0.9)\\(0.0, 0.0)}&\makecell[c]{(575.7, 1.4)\\(4.4, 0.7)}&\makecell[c]{(580.5, 0.5)\\(196.0, 20.8)}&\makecell[c]{(523.8, 8.8)\\(0.0, 0.0)}&\makecell[c]{(556.0, 5.2)\\(0.5, 0.0)}&\makecell[c]{(577.7, 2.5)\\(44.0, 5.6)}&\makecell[c]{(564.5, 1.6)\\(0.0, 0.0)}&\makecell[c]{(574.6, 1.9)\\(4.6, 2.1)}&\makecell[c]{(580.1, 0.9)\\(384.4, 25.6)}&\makecell[c]{(566.2, 3.0)\\(0.0, 0.0)}&\makecell[c]{(575.7, 2.0)\\(3.2, 0.8)}&\makecell[c]{(577.9, 0.5)\\(480.7, 45.8)}&\makecell[c]{(569.3, 1.6)\\(0.0, 0.0)}&\makecell[c]{(576.1, 1.3)\\(4.8, 0.1)}&\makecell[c]{(578.2, 0.6)\\(415.2, 55.1)}\\\hline
s3v80c600-3&\makecell[c]{(572.5, 2.2)\\(70.0, 17.9)}&\makecell[c]{(577.3, 0.6)\\(222.9, 18.5)}&\makecell[c]{(580.2, 1.7)\\(184.8, 17.2)}&\makecell[c]{(579.4, 1.3)\\(193.0, 18.9)}&\makecell[c]{(524.6, 7.6)\\(0.0, 0.0)}&\makecell[c]{(551.2, 4.4)\\(1.8, 0.5)}&\makecell[c]{(566.3, 3.5)\\(161.5, 10.6)}&\makecell[c]{(568.6, 1.6)\\(0.0, 0.0)}&\makecell[c]{(573.7, 2.5)\\(2.6, 0.6)}&\makecell[c]{(584.1, 2.0)\\(198.4, 18.2)}&\makecell[c]{(574.1, 1.4)\\(0.0, 0.0)}&\makecell[c]{(576.1, 4.4)\\(2.6, 0.6)}&\makecell[c]{(583.9, 1.8)\\(201.0, 22.1)}&\makecell[c]{(574.6, 0.7)\\(0.0, 0.0)}&\makecell[c]{(574.4, 2.7)\\(3.0, 0.1)}&\makecell[c]{(584.9, 1.4)\\(200.6, 17.3)}&\makecell[c]{(525.5, 6.7)\\(0.0, 0.0)}&\makecell[c]{(557.4, 6.0)\\(0.4, 0.1)}&\makecell[c]{(581.0, 2.6)\\(49.9, 8.9)}&\makecell[c]{(565.7, 3.2)\\(0.0, 0.0)}&\makecell[c]{(573.0, 2.0)\\(4.4, 0.7)}&\makecell[c]{(584.5, 2.0)\\(388.0, 32.1)}&\makecell[c]{(571.0, 2.3)\\(0.0, 0.0)}&\makecell[c]{(576.0, 0.8)\\(4.6, 1.0)}&\makecell[c]{(579.2, 0.7)\\(460.1, 46.6)}&\makecell[c]{(575.4, 0.9)\\(0.0, 0.0)}&\makecell[c]{(578.4, 0.8)\\(4.1, 1.7)}&\makecell[c]{(580.8, 0.9)\\(414.1, 19.1)}\\\hline
s3v80c600-4&\makecell[c]{(573.8, 3.5)\\(67.5, 10.0)}&\makecell[c]{(578.7, 0.9)\\(220.5, 20.4)}&\makecell[c]{(579.0, 0.8)\\(207.9, 29.4)}&\makecell[c]{(579.8, 1.2)\\(202.6, 29.1)}&\makecell[c]{(524.5, 8.5)\\(0.0, 0.0)}&\makecell[c]{(551.2, 5.4)\\(1.7, 0.5)}&\makecell[c]{(565.3, 3.3)\\(161.0, 11.7)}&\makecell[c]{(567.7, 1.7)\\(0.0, 0.0)}&\makecell[c]{(577.9, 2.0)\\(2.9, 0.0)}&\makecell[c]{(581.8, 1.4)\\(192.5, 16.4)}&\makecell[c]{(570.9, 1.5)\\(0.0, 0.0)}&\makecell[c]{(576.1, 1.6)\\(2.2, 0.8)}&\makecell[c]{(582.0, 0.8)\\(188.9, 24.1)}&\makecell[c]{(576.1, 3.3)\\(0.0, 0.0)}&\makecell[c]{(577.3, 1.1)\\(2.8, 0.5)}&\makecell[c]{(581.5, 1.1)\\(191.3, 16.7)}&\makecell[c]{(524.2, 6.8)\\(0.0, 0.0)}&\makecell[c]{(559.9, 6.7)\\(0.6, 0.0)}&\makecell[c]{(580.4, 3.3)\\(42.6, 4.0)}&\makecell[c]{(569.1, 3.3)\\(0.0, 0.0)}&\makecell[c]{(575.8, 2.4)\\(4.4, 0.0)}&\makecell[c]{(582.5, 0.9)\\(382.2, 17.8)}&\makecell[c]{(568.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(576.7, 2.1)\\(5.3, 0.1)}&\makecell[c]{(580.8, 1.1)\\(452.5, 50.7)}&\makecell[c]{(574.7, 1.3)\\(0.0, 0.0)}&\makecell[c]{(578.7, 1.3)\\(3.6, 1.0)}&\makecell[c]{(583.1, 0.8)\\(405.9, 26.8)}\\\hline
s3v80c600-5&\makecell[c]{(576.8, 3.5)\\(68.0, 14.8)}&\makecell[c]{(586.0, 0.0)\\(235.5, 19.5)}&\makecell[c]{(580.4, 0.5)\\(206.6, 31.4)}&\makecell[c]{(581.2, 0.7)\\(187.2, 16.9)}&\makecell[c]{(525.3, 8.7)\\(0.0, 0.0)}&\makecell[c]{(550.5, 4.5)\\(1.6, 0.7)}&\makecell[c]{(565.9, 3.2)\\(156.1, 9.1)}&\makecell[c]{(570.9, 2.4)\\(0.0, 0.0)}&\makecell[c]{(579.3, 1.3)\\(2.5, 0.6)}&\makecell[c]{(586.0, 0.0)\\(203.4, 17.0)}&\makecell[c]{(569.1, 2.5)\\(0.0, 0.0)}&\makecell[c]{(579.3, 0.6)\\(3.0, 0.0)}&\makecell[c]{(585.9, 0.3)\\(190.7, 25.8)}&\makecell[c]{(573.8, 1.0)\\(0.0, 0.0)}&\makecell[c]{(579.1, 0.3)\\(1.9, 0.7)}&\makecell[c]{(586.0, 0.0)\\(186.4, 15.9)}&\makecell[c]{(523.4, 7.1)\\(0.0, 0.0)}&\makecell[c]{(556.3, 3.4)\\(0.4, 0.1)}&\makecell[c]{(580.8, 1.9)\\(45.5, 6.2)}&\makecell[c]{(573.3, 3.7)\\(0.0, 0.0)}&\makecell[c]{(579.7, 1.7)\\(3.9, 0.6)}&\makecell[c]{(584.6, 0.9)\\(376.6, 20.2)}&\makecell[c]{(569.6, 2.0)\\(0.0, 0.0)}&\makecell[c]{(576.0, 2.2)\\(5.1, 0.5)}&\makecell[c]{(580.1, 0.9)\\(455.7, 36.7)}&\makecell[c]{(573.5, 1.6)\\(0.0, 0.0)}&\makecell[c]{(577.7, 0.5)\\(4.1, 0.8)}&\makecell[c]{(581.0, 0.8)\\(397.6, 23.1)}\\\hline
s3v80c600-6&\makecell[c]{(570.0, 2.0)\\(68.9, 9.9)}&\makecell[c]{(575.0, 1.7)\\(216.8, 13.6)}&\makecell[c]{(580.0, 0.0)\\(219.1, 30.7)}&\makecell[c]{(582.4, 1.2)\\(183.8, 15.0)}&\makecell[c]{(524.5, 7.8)\\(0.0, 0.0)}&\makecell[c]{(548.4, 4.7)\\(2.0, 0.6)}&\makecell[c]{(562.8, 3.2)\\(157.8, 8.5)}&\makecell[c]{(568.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(576.7, 1.3)\\(2.6, 0.5)}&\makecell[c]{(580.9, 1.0)\\(192.0, 19.4)}&\makecell[c]{(566.2, 1.3)\\(0.0, 0.0)}&\makecell[c]{(577.0, 1.0)\\(1.6, 0.3)}&\makecell[c]{(580.4, 0.8)\\(204.4, 18.6)}&\makecell[c]{(570.6, 1.8)\\(0.0, 0.0)}&\makecell[c]{(576.1, 1.6)\\(3.9, 1.5)}&\makecell[c]{(581.0, 1.4)\\(195.0, 20.7)}&\makecell[c]{(525.8, 8.0)\\(0.0, 0.0)}&\makecell[c]{(558.0, 3.0)\\(0.5, 0.0)}&\makecell[c]{(577.8, 2.1)\\(45.5, 4.4)}&\makecell[c]{(568.9, 3.6)\\(0.0, 0.0)}&\makecell[c]{(575.2, 0.7)\\(4.4, 0.1)}&\makecell[c]{(581.2, 1.6)\\(387.6, 23.6)}&\makecell[c]{(567.5, 2.4)\\(0.0, 0.0)}&\makecell[c]{(575.6, 1.0)\\(4.2, 1.1)}&\makecell[c]{(579.1, 0.5)\\(457.9, 46.1)}&\makecell[c]{(571.0, 2.1)\\(0.0, 0.0)}&\makecell[c]{(575.3, 1.1)\\(4.0, 1.1)}&\makecell[c]{(578.7, 0.8)\\(411.1, 21.4)}\\\hline
s3v80c600-7&\makecell[c]{(572.3, 2.3)\\(66.0, 5.3)}&\makecell[c]{(579.4, 1.8)\\(267.3, 55.0)}&\makecell[c]{(583.8, 1.8)\\(204.1, 18.5)}&\makecell[c]{(580.2, 2.4)\\(191.4, 15.4)}&\makecell[c]{(524.2, 9.0)\\(0.0, 0.0)}&\makecell[c]{(550.3, 4.6)\\(1.7, 0.5)}&\makecell[c]{(565.2, 3.5)\\(160.5, 9.6)}&\makecell[c]{(563.9, 2.5)\\(0.0, 0.0)}&\makecell[c]{(574.2, 1.9)\\(2.7, 0.6)}&\makecell[c]{(581.4, 2.0)\\(191.2, 17.8)}&\makecell[c]{(571.9, 2.4)\\(0.0, 0.0)}&\makecell[c]{(574.5, 2.0)\\(2.7, 0.5)}&\makecell[c]{(580.9, 2.1)\\(186.2, 12.9)}&\makecell[c]{(577.8, 2.6)\\(0.0, 0.0)}&\makecell[c]{(574.1, 1.6)\\(3.0, 0.1)}&\makecell[c]{(580.3, 1.4)\\(195.8, 19.3)}&\makecell[c]{(520.9, 7.5)\\(0.0, 0.0)}&\makecell[c]{(556.7, 3.9)\\(0.5, 0.0)}&\makecell[c]{(581.8, 1.5)\\(48.7, 11.9)}&\makecell[c]{(565.9, 3.9)\\(0.0, 0.0)}&\makecell[c]{(573.6, 1.6)\\(4.5, 0.1)}&\makecell[c]{(581.5, 2.5)\\(408.9, 37.9)}&\makecell[c]{(569.4, 2.3)\\(0.0, 0.0)}&\makecell[c]{(576.6, 1.5)\\(4.3, 1.0)}&\makecell[c]{(582.6, 1.3)\\(478.2, 39.1)}&\makecell[c]{(575.6, 2.5)\\(0.0, 0.0)}&\makecell[c]{(580.2, 1.0)\\(4.4, 0.7)}&\makecell[c]{(582.1, 0.3)\\(403.0, 9.6)}\\\hline
s3v80c600-8&\makecell[c]{(569.7, 3.6)\\(65.2, 5.7)}&\makecell[c]{(574.9, 0.5)\\(252.4, 41.4)}&\makecell[c]{(575.7, 1.7)\\(209.1, 26.7)}&\makecell[c]{(580.6, 2.8)\\(191.9, 11.8)}&\makecell[c]{(525.0, 8.3)\\(0.0, 0.0)}&\makecell[c]{(549.1, 4.7)\\(1.7, 0.6)}&\makecell[c]{(564.2, 3.3)\\(166.5, 11.7)}&\makecell[c]{(565.9, 1.9)\\(0.0, 0.0)}&\makecell[c]{(573.3, 1.5)\\(2.6, 0.6)}&\makecell[c]{(576.5, 0.8)\\(204.8, 16.0)}&\makecell[c]{(569.8, 1.6)\\(0.0, 0.0)}&\makecell[c]{(573.7, 1.4)\\(2.9, 0.3)}&\makecell[c]{(577.7, 2.1)\\(198.2, 15.7)}&\makecell[c]{(571.3, 1.5)\\(0.0, 0.0)}&\makecell[c]{(573.9, 1.8)\\(3.1, 0.1)}&\makecell[c]{(577.7, 1.6)\\(177.3, 12.8)}&\makecell[c]{(525.3, 8.2)\\(0.0, 0.0)}&\makecell[c]{(553.4, 4.5)\\(0.5, 0.0)}&\makecell[c]{(579.4, 2.5)\\(46.3, 11.0)}&\makecell[c]{(563.4, 1.7)\\(0.0, 0.0)}&\makecell[c]{(570.2, 2.0)\\(3.3, 0.9)}&\makecell[c]{(579.2, 1.2)\\(372.1, 16.4)}&\makecell[c]{(568.1, 1.8)\\(0.0, 0.0)}&\makecell[c]{(573.5, 1.1)\\(4.4, 1.1)}&\makecell[c]{(576.0, 0.6)\\(469.5, 51.4)}&\makecell[c]{(572.8, 1.5)\\(0.0, 0.0)}&\makecell[c]{(576.0, 0.0)\\(4.3, 0.8)}&\makecell[c]{(576.1, 0.3)\\(413.6, 32.3)}\\\hline
s3v80c600-9&\makecell[c]{(570.9, 2.8)\\(63.6, 6.7)}&\makecell[c]{(581.7, 1.2)\\(231.4, 21.7)}&\makecell[c]{(581.0, 0.0)\\(189.9, 17.5)}&\makecell[c]{(583.6, 1.8)\\(196.8, 18.5)}&\makecell[c]{(525.0, 8.2)\\(0.0, 0.0)}&\makecell[c]{(551.2, 5.0)\\(1.8, 0.6)}&\makecell[c]{(567.1, 3.4)\\(160.5, 9.0)}&\makecell[c]{(572.5, 0.8)\\(0.0, 0.0)}&\makecell[c]{(577.9, 1.4)\\(2.9, 0.4)}&\makecell[c]{(581.6, 0.8)\\(199.0, 16.0)}&\makecell[c]{(573.0, 1.3)\\(0.0, 0.0)}&\makecell[c]{(576.7, 1.2)\\(2.2, 0.7)}&\makecell[c]{(582.7, 1.6)\\(188.9, 13.7)}&\makecell[c]{(577.3, 2.9)\\(0.0, 0.0)}&\makecell[c]{(577.0, 1.9)\\(2.7, 0.5)}&\makecell[c]{(583.1, 0.8)\\(198.2, 19.9)}&\makecell[c]{(528.2, 9.3)\\(0.0, 0.0)}&\makecell[c]{(557.5, 5.7)\\(0.3, 0.1)}&\makecell[c]{(580.4, 2.5)\\(44.8, 5.9)}&\makecell[c]{(568.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(574.5, 2.4)\\(4.4, 0.6)}&\makecell[c]{(584.4, 1.7)\\(386.8, 37.8)}&\makecell[c]{(572.2, 2.2)\\(0.0, 0.0)}&\makecell[c]{(576.8, 1.2)\\(4.8, 1.0)}&\makecell[c]{(580.8, 1.2)\\(478.4, 61.0)}&\makecell[c]{(576.2, 1.8)\\(0.0, 0.0)}&\makecell[c]{(579.5, 0.7)\\(3.8, 0.8)}&\makecell[c]{(580.7, 0.9)\\(406.4, 22.5)}\\\hline
s3v80c600-10&\makecell[c]{(571.8, 2.5)\\(66.6, 5.2)}&\makecell[c]{(576.5, 1.1)\\(233.0, 50.8)}&\makecell[c]{(576.7, 1.3)\\(218.3, 21.0)}&\makecell[c]{(578.2, 0.4)\\(195.2, 23.1)}&\makecell[c]{(525.1, 9.0)\\(0.0, 0.0)}&\makecell[c]{(548.3, 4.6)\\(2.1, 0.6)}&\makecell[c]{(563.1, 3.3)\\(173.3, 12.6)}&\makecell[c]{(569.9, 1.6)\\(0.0, 0.0)}&\makecell[c]{(576.3, 1.9)\\(2.9, 0.0)}&\makecell[c]{(581.1, 1.6)\\(189.7, 9.5)}&\makecell[c]{(568.6, 2.2)\\(0.0, 0.0)}&\makecell[c]{(576.2, 1.2)\\(3.0, 0.0)}&\makecell[c]{(581.3, 1.3)\\(185.6, 14.4)}&\makecell[c]{(568.3, 1.6)\\(0.0, 0.0)}&\makecell[c]{(576.6, 1.4)\\(2.5, 0.6)}&\makecell[c]{(580.9, 1.3)\\(185.2, 18.6)}&\makecell[c]{(525.8, 6.5)\\(0.0, 0.0)}&\makecell[c]{(556.4, 4.3)\\(0.5, 0.0)}&\makecell[c]{(578.3, 3.3)\\(44.3, 3.3)}&\makecell[c]{(569.3, 3.0)\\(0.0, 0.0)}&\makecell[c]{(576.8, 2.1)\\(3.9, 0.7)}&\makecell[c]{(580.9, 1.9)\\(406.4, 30.6)}&\makecell[c]{(569.8, 1.9)\\(0.0, 0.0)}&\makecell[c]{(573.9, 2.3)\\(4.4, 1.0)}&\makecell[c]{(577.9, 1.0)\\(472.6, 68.5)}&\makecell[c]{(570.2, 1.8)\\(0.0, 0.0)}&\makecell[c]{(577.0, 1.0)\\(3.1, 0.9)}&\makecell[c]{(580.5, 1.0)\\(411.3, 24.8)}\\\hline
s3v80c800-1&\makecell[c]{(751.1, 3.8)\\(74.9, 7.7)}&\makecell[c]{(764.6, 2.8)\\(297.5, 50.9)}&\makecell[c]{(762.1, 1.8)\\(289.9, 70.7)}&\makecell[c]{(769.3, 0.9)\\(256.3, 21.6)}&\makecell[c]{(701.5, 8.1)\\(0.0, 0.0)}&\makecell[c]{(728.1, 5.3)\\(2.2, 0.9)}&\makecell[c]{(745.5, 4.3)\\(209.3, 29.8)}&\makecell[c]{(749.3, 3.9)\\(0.0, 0.0)}&\makecell[c]{(765.4, 2.6)\\(2.0, 0.2)}&\makecell[c]{(767.2, 0.4)\\(246.7, 47.5)}&\makecell[c]{(744.0, 1.9)\\(0.0, 0.0)}&\makecell[c]{(762.9, 2.6)\\(3.0, 0.9)}&\makecell[c]{(766.8, 1.0)\\(252.6, 89.5)}&\makecell[c]{(758.3, 2.8)\\(0.0, 0.0)}&\makecell[c]{(763.9, 2.2)\\(3.4, 0.8)}&\makecell[c]{(766.9, 0.7)\\(240.1, 28.5)}&\makecell[c]{(700.9, 7.1)\\(0.0, 0.0)}&\makecell[c]{(735.6, 7.1)\\(0.7, 0.0)}&\makecell[c]{(765.7, 3.7)\\(58.8, 9.5)}&\makecell[c]{(744.7, 3.8)\\(0.0, 0.0)}&\makecell[c]{(757.6, 3.5)\\(5.8, 0.1)}&\makecell[c]{(767.4, 1.4)\\(478.4, 36.9)}&\makecell[c]{(745.7, 2.6)\\(0.0, 0.0)}&\makecell[c]{(756.9, 2.1)\\(10.0, 1.5)}&\makecell[c]{(762.6, 1.3)\\(584.1, 75.6)}&\makecell[c]{(753.9, 3.9)\\(0.0, 0.0)}&\makecell[c]{(760.2, 1.7)\\(5.0, 1.3)}&\makecell[c]{(765.3, 1.6)\\(523.3, 68.1)}\\\hline
s3v80c800-2&\makecell[c]{(749.7, 3.3)\\(74.2, 9.6)}&\makecell[c]{(763.7, 1.3)\\(292.4, 36.6)}&\makecell[c]{(762.1, 1.9)\\(271.4, 35.5)}&\makecell[c]{(760.0, 1.7)\\(266.2, 22.1)}&\makecell[c]{(699.8, 8.5)\\(0.0, 0.0)}&\makecell[c]{(728.2, 4.9)\\(2.4, 0.6)}&\makecell[c]{(744.1, 3.0)\\(205.9, 24.9)}&\makecell[c]{(747.8, 1.2)\\(0.0, 0.0)}&\makecell[c]{(755.8, 2.3)\\(3.8, 0.4)}&\makecell[c]{(761.9, 1.4)\\(238.5, 35.8)}&\makecell[c]{(738.2, 3.0)\\(0.0, 0.0)}&\makecell[c]{(757.5, 1.7)\\(2.9, 0.8)}&\makecell[c]{(761.7, 1.3)\\(236.8, 42.2)}&\makecell[c]{(753.5, 3.2)\\(0.0, 0.0)}&\makecell[c]{(756.1, 2.1)\\(3.7, 0.4)}&\makecell[c]{(761.7, 1.7)\\(230.8, 28.2)}&\makecell[c]{(700.6, 10.7)\\(0.0, 0.0)}&\makecell[c]{(734.8, 3.2)\\(0.7, 0.0)}&\makecell[c]{(759.8, 3.5)\\(52.2, 4.7)}&\makecell[c]{(749.0, 2.7)\\(0.0, 0.0)}&\makecell[c]{(756.7, 2.2)\\(5.4, 0.8)}&\makecell[c]{(764.9, 1.6)\\(496.6, 50.7)}&\makecell[c]{(746.8, 2.6)\\(0.0, 0.0)}&\makecell[c]{(755.0, 1.8)\\(5.8, 1.2)}&\makecell[c]{(759.2, 0.7)\\(585.9, 96.7)}&\makecell[c]{(752.4, 2.3)\\(0.0, 0.0)}&\makecell[c]{(759.7, 2.3)\\(5.8, 0.7)}&\makecell[c]{(763.1, 0.3)\\(520.1, 79.5)}\\\hline
s3v80c800-3&\makecell[c]{(754.5, 3.4)\\(76.8, 13.8)}&\makecell[c]{(762.0, 0.8)\\(291.2, 48.6)}&\makecell[c]{(764.5, 2.8)\\(258.2, 26.3)}&\makecell[c]{(768.9, 0.3)\\(268.7, 34.0)}&\makecell[c]{(700.7, 10.4)\\(0.0, 0.0)}&\makecell[c]{(730.8, 5.6)\\(2.3, 0.6)}&\makecell[c]{(748.6, 3.6)\\(213.4, 33.6)}&\makecell[c]{(743.7, 1.7)\\(0.0, 0.0)}&\makecell[c]{(758.0, 2.3)\\(3.9, 0.1)}&\makecell[c]{(766.6, 1.7)\\(232.0, 30.6)}&\makecell[c]{(756.0, 1.9)\\(0.0, 0.0)}&\makecell[c]{(759.1, 3.5)\\(3.8, 0.1)}&\makecell[c]{(766.3, 0.9)\\(241.8, 46.1)}&\makecell[c]{(762.1, 2.4)\\(0.0, 0.0)}&\makecell[c]{(759.3, 3.2)\\(3.9, 0.1)}&\makecell[c]{(766.1, 1.6)\\(235.2, 39.9)}&\makecell[c]{(698.7, 7.1)\\(0.0, 0.0)}&\makecell[c]{(738.0, 5.2)\\(0.7, 0.0)}&\makecell[c]{(768.1, 2.6)\\(51.5, 4.8)}&\makecell[c]{(746.4, 3.6)\\(0.0, 0.0)}&\makecell[c]{(757.5, 3.0)\\(5.6, 0.1)}&\makecell[c]{(767.9, 2.3)\\(497.2, 46.7)}&\makecell[c]{(754.6, 3.0)\\(0.0, 0.0)}&\makecell[c]{(761.1, 1.1)\\(6.0, 1.2)}&\makecell[c]{(765.3, 0.8)\\(577.8, 82.8)}&\makecell[c]{(758.5, 2.7)\\(0.0, 0.0)}&\makecell[c]{(761.9, 1.7)\\(6.1, 1.6)}&\makecell[c]{(767.9, 0.3)\\(502.5, 42.2)}\\\hline
s3v80c800-4&\makecell[c]{(752.2, 2.7)\\(74.5, 11.3)}&\makecell[c]{(768.8, 0.6)\\(298.9, 43.9)}&\makecell[c]{(765.5, 3.0)\\(276.0, 41.6)}&\makecell[c]{(769.2, 2.9)\\(263.0, 29.3)}&\makecell[c]{(699.7, 9.4)\\(0.0, 0.0)}&\makecell[c]{(729.9, 5.1)\\(2.3, 0.7)}&\makecell[c]{(746.9, 3.9)\\(205.7, 25.7)}&\makecell[c]{(755.0, 1.8)\\(0.0, 0.0)}&\makecell[c]{(767.3, 1.1)\\(3.0, 0.9)}&\makecell[c]{(770.6, 1.0)\\(236.2, 35.6)}&\makecell[c]{(754.3, 1.2)\\(0.0, 0.0)}&\makecell[c]{(766.1, 2.2)\\(3.7, 0.5)}&\makecell[c]{(770.6, 1.0)\\(239.4, 41.6)}&\makecell[c]{(756.4, 2.0)\\(0.0, 0.0)}&\makecell[c]{(767.1, 1.5)\\(2.9, 0.7)}&\makecell[c]{(770.9, 0.8)\\(244.3, 61.4)}&\makecell[c]{(698.0, 6.3)\\(0.0, 0.0)}&\makecell[c]{(739.3, 5.1)\\(0.7, 0.0)}&\makecell[c]{(766.2, 2.8)\\(53.4, 8.0)}&\makecell[c]{(753.2, 3.6)\\(0.0, 0.0)}&\makecell[c]{(762.8, 3.1)\\(5.5, 0.5)}&\makecell[c]{(773.2, 1.3)\\(495.3, 52.9)}&\makecell[c]{(750.8, 3.8)\\(0.0, 0.0)}&\makecell[c]{(758.4, 1.6)\\(6.3, 1.1)}&\makecell[c]{(763.4, 1.5)\\(575.3, 52.8)}&\makecell[c]{(756.6, 3.4)\\(0.0, 0.0)}&\makecell[c]{(765.0, 1.0)\\(4.8, 1.2)}&\makecell[c]{(766.3, 0.6)\\(508.2, 41.6)}\\\hline
s3v80c800-5&\makecell[c]{(752.0, 5.7)\\(74.3, 13.7)}&\makecell[c]{(761.4, 2.0)\\(286.6, 17.1)}&\makecell[c]{(762.5, 3.0)\\(271.0, 34.1)}&\makecell[c]{(768.7, 0.5)\\(267.0, 37.7)}&\makecell[c]{(700.4, 9.1)\\(0.0, 0.0)}&\makecell[c]{(728.5, 5.5)\\(2.7, 0.9)}&\makecell[c]{(744.6, 3.8)\\(211.9, 44.2)}&\makecell[c]{(753.8, 1.1)\\(0.0, 0.0)}&\makecell[c]{(760.0, 1.8)\\(2.9, 0.8)}&\makecell[c]{(765.4, 2.2)\\(252.3, 56.6)}&\makecell[c]{(755.6, 4.6)\\(0.0, 0.0)}&\makecell[c]{(760.6, 1.7)\\(4.8, 1.5)}&\makecell[c]{(764.1, 1.2)\\(246.5, 56.7)}&\makecell[c]{(756.7, 2.2)\\(0.0, 0.0)}&\makecell[c]{(759.5, 1.9)\\(2.9, 0.7)}&\makecell[c]{(764.9, 1.1)\\(236.4, 47.5)}&\makecell[c]{(699.3, 10.7)\\(0.0, 0.0)}&\makecell[c]{(733.4, 4.5)\\(0.5, 0.2)}&\makecell[c]{(763.9, 3.6)\\(56.6, 6.5)}&\makecell[c]{(752.6, 3.7)\\(0.0, 0.0)}&\makecell[c]{(759.1, 1.5)\\(5.2, 0.8)}&\makecell[c]{(766.9, 1.9)\\(484.0, 35.2)}&\makecell[c]{(751.3, 3.0)\\(0.0, 0.0)}&\makecell[c]{(760.9, 1.0)\\(6.6, 0.6)}&\makecell[c]{(761.6, 0.8)\\(567.3, 66.0)}&\makecell[c]{(755.3, 4.0)\\(0.0, 0.0)}&\makecell[c]{(760.7, 1.0)\\(5.2, 1.2)}&\makecell[c]{(763.0, 0.0)\\(506.2, 39.1)}\\\hline
s3v80c800-6&\makecell[c]{(756.8, 1.5)\\(75.6, 10.9)}&\makecell[c]{(763.0, 1.3)\\(311.3, 86.6)}&\makecell[c]{(761.7, 2.3)\\(274.0, 30.7)}&\makecell[c]{(766.9, 2.2)\\(271.3, 33.9)}&\makecell[c]{(699.5, 8.1)\\(0.0, 0.0)}&\makecell[c]{(729.0, 5.7)\\(2.5, 0.6)}&\makecell[c]{(746.1, 3.9)\\(206.7, 23.6)}&\makecell[c]{(753.2, 1.9)\\(0.0, 0.0)}&\makecell[c]{(762.5, 2.5)\\(3.9, 0.1)}&\makecell[c]{(767.0, 1.5)\\(245.0, 45.4)}&\makecell[c]{(763.1, 2.1)\\(0.0, 0.0)}&\makecell[c]{(760.9, 2.0)\\(2.8, 0.8)}&\makecell[c]{(766.4, 1.4)\\(239.1, 44.5)}&\makecell[c]{(758.4, 1.7)\\(0.0, 0.0)}&\makecell[c]{(761.4, 0.5)\\(3.2, 0.8)}&\makecell[c]{(766.3, 1.7)\\(228.3, 32.8)}&\makecell[c]{(698.4, 11.7)\\(0.0, 0.0)}&\makecell[c]{(737.7, 4.1)\\(0.7, 0.0)}&\makecell[c]{(765.3, 2.4)\\(55.6, 8.1)}&\makecell[c]{(752.0, 3.7)\\(0.1, 0.0)}&\makecell[c]{(759.9, 1.8)\\(6.6, 1.5)}&\makecell[c]{(766.4, 1.4)\\(485.7, 46.7)}&\makecell[c]{(756.0, 2.4)\\(0.0, 0.0)}&\makecell[c]{(760.2, 1.2)\\(6.5, 0.8)}&\makecell[c]{(764.8, 0.7)\\(589.5, 102.6)}&\makecell[c]{(758.2, 0.9)\\(0.0, 0.0)}&\makecell[c]{(761.7, 0.8)\\(5.3, 0.9)}&\makecell[c]{(765.0, 0.0)\\(504.6, 68.6)}\\\hline
s3v80c800-7&\makecell[c]{(751.2, 2.5)\\(75.4, 11.0)}&\makecell[c]{(768.1, 0.8)\\(290.5, 35.1)}&\makecell[c]{(760.8, 2.4)\\(279.2, 35.6)}&\makecell[c]{(768.4, 1.5)\\(281.3, 53.9)}&\makecell[c]{(700.5, 7.9)\\(0.0, 0.0)}&\makecell[c]{(729.8, 5.4)\\(2.9, 0.4)}&\makecell[c]{(747.0, 4.8)\\(206.2, 22.3)}&\makecell[c]{(753.3, 2.1)\\(0.0, 0.0)}&\makecell[c]{(763.3, 2.3)\\(3.4, 0.8)}&\makecell[c]{(768.9, 1.6)\\(245.4, 43.6)}&\makecell[c]{(752.9, 2.3)\\(0.0, 0.0)}&\makecell[c]{(763.3, 2.1)\\(2.8, 0.9)}&\makecell[c]{(768.9, 1.6)\\(238.8, 38.7)}&\makecell[c]{(754.0, 2.4)\\(0.0, 0.0)}&\makecell[c]{(763.1, 2.3)\\(3.0, 0.8)}&\makecell[c]{(769.2, 0.9)\\(236.0, 36.8)}&\makecell[c]{(702.6, 7.4)\\(0.0, 0.0)}&\makecell[c]{(741.5, 6.2)\\(0.7, 0.0)}&\makecell[c]{(768.6, 3.8)\\(53.4, 6.8)}&\makecell[c]{(749.0, 4.0)\\(0.0, 0.0)}&\makecell[c]{(761.3, 2.6)\\(5.6, 0.5)}&\makecell[c]{(770.5, 1.4)\\(489.9, 39.2)}&\makecell[c]{(755.3, 3.3)\\(0.0, 0.0)}&\makecell[c]{(760.6, 0.7)\\(5.4, 1.2)}&\makecell[c]{(764.7, 1.0)\\(591.7, 99.0)}&\makecell[c]{(756.2, 2.6)\\(0.0, 0.0)}&\makecell[c]{(763.7, 2.1)\\(4.9, 1.2)}&\makecell[c]{(767.0, 0.0)\\(510.4, 48.2)}\\\hline
s3v80c800-8&\makecell[c]{(757.2, 4.5)\\(75.6, 9.9)}&\makecell[c]{(765.4, 0.7)\\(298.1, 48.1)}&\makecell[c]{(771.1, 0.3)\\(274.6, 37.1)}&\makecell[c]{(764.7, 1.7)\\(261.5, 19.8)}&\makecell[c]{(699.5, 10.4)\\(0.0, 0.0)}&\makecell[c]{(730.9, 5.3)\\(2.7, 0.7)}&\makecell[c]{(748.3, 3.8)\\(215.8, 38.9)}&\makecell[c]{(750.1, 2.2)\\(0.0, 0.0)}&\makecell[c]{(761.8, 3.2)\\(4.2, 1.1)}&\makecell[c]{(772.5, 1.4)\\(238.7, 40.1)}&\makecell[c]{(756.5, 2.5)\\(0.0, 0.0)}&\makecell[c]{(765.1, 4.1)\\(3.5, 0.7)}&\makecell[c]{(772.4, 1.3)\\(248.8, 74.1)}&\makecell[c]{(759.4, 1.7)\\(0.0, 0.0)}&\makecell[c]{(759.6, 3.1)\\(2.7, 0.8)}&\makecell[c]{(771.6, 2.5)\\(235.4, 40.8)}&\makecell[c]{(705.4, 5.0)\\(0.0, 0.0)}&\makecell[c]{(738.6, 6.8)\\(0.4, 0.1)}&\makecell[c]{(767.8, 3.1)\\(55.1, 5.6)}&\makecell[c]{(754.0, 2.8)\\(0.0, 0.0)}&\makecell[c]{(761.6, 2.5)\\(5.3, 0.8)}&\makecell[c]{(771.8, 1.8)\\(477.5, 19.3)}&\makecell[c]{(753.9, 2.7)\\(0.0, 0.0)}&\makecell[c]{(763.2, 1.9)\\(4.5, 1.1)}&\makecell[c]{(766.5, 1.6)\\(575.9, 81.9)}&\makecell[c]{(760.3, 0.6)\\(0.0, 0.0)}&\makecell[c]{(766.1, 1.1)\\(5.8, 0.8)}&\makecell[c]{(769.1, 0.5)\\(504.9, 42.9)}\\\hline
s3v80c800-9&\makecell[c]{(756.8, 3.2)\\(74.2, 12.8)}&\makecell[c]{(766.4, 1.5)\\(288.5, 35.6)}&\makecell[c]{(770.1, 1.1)\\(271.0, 30.3)}&\makecell[c]{(766.9, 1.0)\\(261.7, 28.6)}&\makecell[c]{(701.0, 8.5)\\(0.0, 0.0)}&\makecell[c]{(730.7, 6.3)\\(2.4, 0.5)}&\makecell[c]{(749.0, 3.8)\\(210.0, 31.0)}&\makecell[c]{(752.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(765.5, 1.4)\\(4.1, 1.0)}&\makecell[c]{(770.5, 2.1)\\(240.1, 28.6)}&\makecell[c]{(754.8, 2.0)\\(0.0, 0.0)}&\makecell[c]{(765.1, 2.2)\\(3.4, 0.7)}&\makecell[c]{(770.5, 2.0)\\(236.4, 34.8)}&\makecell[c]{(762.2, 2.8)\\(0.1, 0.0)}&\makecell[c]{(763.1, 2.1)\\(4.8, 1.3)}&\makecell[c]{(768.7, 1.3)\\(231.0, 32.5)}&\makecell[c]{(704.1, 8.2)\\(0.0, 0.0)}&\makecell[c]{(734.8, 5.0)\\(0.7, 0.0)}&\makecell[c]{(767.2, 2.5)\\(55.5, 7.5)}&\makecell[c]{(751.3, 3.4)\\(0.0, 0.0)}&\makecell[c]{(761.5, 2.1)\\(4.5, 1.2)}&\makecell[c]{(770.9, 0.9)\\(491.7, 42.5)}&\makecell[c]{(757.6, 4.6)\\(0.0, 0.0)}&\makecell[c]{(763.3, 1.7)\\(5.9, 1.1)}&\makecell[c]{(767.0, 0.4)\\(574.1, 47.1)}&\makecell[c]{(761.9, 2.3)\\(0.0, 0.0)}&\makecell[c]{(767.3, 1.3)\\(4.1, 0.9)}&\makecell[c]{(769.9, 0.5)\\(528.8, 80.9)}\\\hline
s3v80c800-10&\makecell[c]{(754.7, 3.5)\\(74.7, 15.1)}&\makecell[c]{(766.9, 1.5)\\(285.1, 32.7)}&\makecell[c]{(762.1, 3.8)\\(270.3, 21.8)}&\makecell[c]{(767.0, 1.0)\\(255.8, 18.4)}&\makecell[c]{(700.9, 8.9)\\(0.0, 0.0)}&\makecell[c]{(730.2, 5.5)\\(2.7, 0.8)}&\makecell[c]{(748.1, 4.5)\\(203.2, 19.8)}&\makecell[c]{(752.5, 2.6)\\(0.0, 0.0)}&\makecell[c]{(761.0, 1.4)\\(3.8, 1.4)}&\makecell[c]{(768.1, 2.3)\\(234.5, 27.3)}&\makecell[c]{(753.3, 2.9)\\(0.0, 0.0)}&\makecell[c]{(761.4, 0.9)\\(3.7, 0.5)}&\makecell[c]{(767.0, 2.1)\\(247.5, 70.1)}&\makecell[c]{(761.1, 1.5)\\(0.0, 0.0)}&\makecell[c]{(762.2, 1.2)\\(3.0, 0.8)}&\makecell[c]{(767.4, 1.0)\\(234.1, 36.4)}&\makecell[c]{(698.7, 9.9)\\(0.0, 0.0)}&\makecell[c]{(734.9, 6.0)\\(0.7, 0.0)}&\makecell[c]{(766.9, 2.0)\\(56.9, 7.5)}&\makecell[c]{(750.3, 2.1)\\(0.0, 0.0)}&\makecell[c]{(757.7, 1.6)\\(4.5, 1.3)}&\makecell[c]{(767.6, 2.2)\\(486.6, 38.4)}&\makecell[c]{(756.4, 2.3)\\(0.0, 0.0)}&\makecell[c]{(762.6, 1.9)\\(5.5, 1.1)}&\makecell[c]{(766.4, 0.5)\\(566.1, 77.5)}&\makecell[c]{(760.6, 1.2)\\(0.0, 0.0)}&\makecell[c]{(766.5, 1.9)\\(5.5, 1.0)}&\makecell[c]{(770.1, 0.5)\\(507.6, 39.0)}\\\hline
s3v80c900-1&\makecell[c]{(843.8, 4.1)\\(80.0, 14.8)}&\makecell[c]{(854.4, 1.6)\\(309.0, 46.1)}&\makecell[c]{(852.0, 2.0)\\(304.2, 64.0)}&\makecell[c]{(856.6, 2.8)\\(292.8, 52.5)}&\makecell[c]{(787.7, 9.2)\\(0.0, 0.0)}&\makecell[c]{(818.0, 6.2)\\(3.1, 0.9)}&\makecell[c]{(836.2, 4.0)\\(220.4, 40.7)}&\makecell[c]{(840.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(854.7, 4.1)\\(3.7, 0.9)}&\makecell[c]{(860.4, 0.5)\\(261.3, 56.4)}&\makecell[c]{(846.6, 1.7)\\(0.0, 0.0)}&\makecell[c]{(854.1, 3.0)\\(5.1, 1.7)}&\makecell[c]{(859.4, 1.7)\\(258.3, 61.5)}&\makecell[c]{(841.0, 4.4)\\(0.0, 0.0)}&\makecell[c]{(852.2, 4.1)\\(4.5, 0.0)}&\makecell[c]{(860.5, 0.7)\\(250.3, 44.6)}&\makecell[c]{(788.2, 6.5)\\(0.0, 0.0)}&\makecell[c]{(826.0, 6.7)\\(0.8, 0.0)}&\makecell[c]{(857.3, 3.7)\\(58.0, 8.9)}&\makecell[c]{(838.7, 3.0)\\(0.0, 0.0)}&\makecell[c]{(852.1, 1.3)\\(4.5, 1.3)}&\makecell[c]{(860.1, 0.9)\\(525.6, 78.4)}&\makecell[c]{(842.1, 4.0)\\(0.0, 0.0)}&\makecell[c]{(849.3, 0.9)\\(5.0, 1.3)}&\makecell[c]{(856.2, 1.5)\\(616.3, 106.1)}&\makecell[c]{(842.6, 4.7)\\(0.0, 0.0)}&\makecell[c]{(855.6, 2.0)\\(5.6, 1.1)}&\makecell[c]{(858.5, 0.9)\\(548.9, 80.8)}\\\hline
s3v80c900-2&\makecell[c]{(843.4, 3.6)\\(76.9, 14.2)}&\makecell[c]{(850.2, 1.2)\\(315.0, 64.0)}&\makecell[c]{(850.3, 1.3)\\(312.9, 102.3)}&\makecell[c]{(854.9, 1.8)\\(292.0, 53.0)}&\makecell[c]{(785.6, 9.7)\\(0.0, 0.0)}&\makecell[c]{(818.1, 6.2)\\(2.9, 0.7)}&\makecell[c]{(836.7, 3.6)\\(215.9, 27.8)}&\makecell[c]{(844.3, 2.0)\\(0.0, 0.0)}&\makecell[c]{(850.9, 2.9)\\(2.7, 0.7)}&\makecell[c]{(856.4, 0.9)\\(257.2, 54.2)}&\makecell[c]{(844.9, 1.4)\\(0.0, 0.0)}&\makecell[c]{(851.5, 2.5)\\(4.2, 0.7)}&\makecell[c]{(856.1, 1.2)\\(250.1, 48.4)}&\makecell[c]{(845.5, 2.8)\\(0.0, 0.0)}&\makecell[c]{(851.1, 3.2)\\(2.8, 0.7)}&\makecell[c]{(856.1, 0.8)\\(258.2, 68.4)}&\makecell[c]{(788.4, 9.8)\\(0.0, 0.0)}&\makecell[c]{(829.1, 6.6)\\(0.4, 0.0)}&\makecell[c]{(856.5, 2.7)\\(57.7, 10.0)}&\makecell[c]{(837.7, 3.3)\\(0.0, 0.0)}&\makecell[c]{(846.8, 3.0)\\(4.3, 1.2)}&\makecell[c]{(859.6, 2.7)\\(515.3, 57.9)}&\makecell[c]{(846.0, 1.4)\\(0.0, 0.0)}&\makecell[c]{(850.4, 1.8)\\(6.1, 1.7)}&\makecell[c]{(855.0, 0.8)\\(611.6, 96.8)}&\makecell[c]{(846.4, 3.6)\\(0.0, 0.0)}&\makecell[c]{(854.6, 1.9)\\(6.2, 1.0)}&\makecell[c]{(856.4, 0.9)\\(544.4, 72.8)}\\\hline
s3v80c900-3&\makecell[c]{(847.9, 3.0)\\(80.3, 16.7)}&\makecell[c]{(860.0, 0.4)\\(324.2, 75.9)}&\makecell[c]{(857.5, 2.9)\\(298.4, 53.9)}&\makecell[c]{(854.6, 1.3)\\(294.6, 56.8)}&\makecell[c]{(787.6, 9.2)\\(0.0, 0.0)}&\makecell[c]{(819.5, 6.1)\\(2.7, 0.6)}&\makecell[c]{(837.8, 4.6)\\(220.6, 39.0)}&\makecell[c]{(837.3, 2.4)\\(0.0, 0.0)}&\makecell[c]{(855.4, 2.9)\\(3.3, 0.9)}&\makecell[c]{(862.1, 1.9)\\(260.2, 57.6)}&\makecell[c]{(840.5, 1.9)\\(0.0, 0.0)}&\makecell[c]{(857.1, 1.8)\\(3.6, 0.9)}&\makecell[c]{(862.2, 1.8)\\(251.5, 46.7)}&\makecell[c]{(848.3, 2.9)\\(0.0, 0.0)}&\makecell[c]{(856.1, 1.3)\\(4.4, 0.1)}&\makecell[c]{(861.1, 1.6)\\(253.4, 52.7)}&\makecell[c]{(784.0, 6.8)\\(0.0, 0.0)}&\makecell[c]{(828.2, 7.0)\\(0.7, 0.0)}&\makecell[c]{(858.3, 2.8)\\(61.5, 15.5)}&\makecell[c]{(841.4, 3.1)\\(0.0, 0.0)}&\makecell[c]{(852.2, 3.5)\\(4.8, 1.3)}&\makecell[c]{(861.0, 1.9)\\(523.7, 73.1)}&\makecell[c]{(839.9, 4.3)\\(0.0, 0.0)}&\makecell[c]{(850.4, 1.9)\\(5.8, 1.6)}&\makecell[c]{(854.3, 1.1)\\(615.4, 93.8)}&\makecell[c]{(849.5, 1.3)\\(0.0, 0.0)}&\makecell[c]{(855.2, 1.7)\\(6.5, 1.0)}&\makecell[c]{(859.5, 0.8)\\(549.5, 80.8)}\\\hline
s3v80c900-4&\makecell[c]{(842.5, 3.3)\\(80.9, 17.6)}&\makecell[c]{(852.3, 2.5)\\(311.5, 51.2)}&\makecell[c]{(853.3, 2.7)\\(297.9, 52.5)}&\makecell[c]{(851.6, 2.1)\\(290.3, 50.6)}&\makecell[c]{(787.1, 10.5)\\(0.0, 0.0)}&\makecell[c]{(816.6, 5.4)\\(3.0, 0.7)}&\makecell[c]{(834.3, 3.7)\\(217.7, 30.0)}&\makecell[c]{(835.9, 1.3)\\(0.0, 0.0)}&\makecell[c]{(850.2, 4.3)\\(3.8, 0.8)}&\makecell[c]{(857.9, 1.4)\\(251.7, 44.0)}&\makecell[c]{(842.7, 1.3)\\(0.0, 0.0)}&\makecell[c]{(850.7, 1.7)\\(3.8, 0.9)}&\makecell[c]{(858.1, 0.9)\\(252.3, 53.3)}&\makecell[c]{(843.8, 1.3)\\(0.0, 0.0)}&\makecell[c]{(850.4, 1.5)\\(4.1, 0.8)}&\makecell[c]{(857.9, 1.3)\\(258.9, 60.8)}&\makecell[c]{(789.6, 10.6)\\(0.0, 0.0)}&\makecell[c]{(828.5, 4.9)\\(0.7, 0.0)}&\makecell[c]{(854.8, 3.1)\\(58.0, 8.6)}&\makecell[c]{(834.9, 3.0)\\(0.0, 0.0)}&\makecell[c]{(845.5, 2.2)\\(5.6, 1.1)}&\makecell[c]{(855.6, 2.2)\\(515.4, 64.7)}&\makecell[c]{(843.8, 2.8)\\(0.0, 0.0)}&\makecell[c]{(847.9, 1.5)\\(6.3, 1.3)}&\makecell[c]{(851.9, 0.9)\\(618.2, 101.2)}&\makecell[c]{(843.1, 1.9)\\(0.0, 0.0)}&\makecell[c]{(851.2, 0.6)\\(5.7, 1.3)}&\makecell[c]{(854.2, 0.7)\\(548.8, 82.8)}\\\hline
s3v80c900-5&\makecell[c]{(847.5, 3.9)\\(78.1, 15.3)}&\makecell[c]{(859.3, 2.0)\\(312.8, 56.5)}&\makecell[c]{(858.7, 1.4)\\(312.5, 86.6)}&\makecell[c]{(863.2, 2.4)\\(294.4, 28.3)}&\makecell[c]{(787.6, 10.0)\\(0.0, 0.0)}&\makecell[c]{(818.6, 6.4)\\(3.0, 0.8)}&\makecell[c]{(838.5, 4.8)\\(218.9, 33.9)}&\makecell[c]{(843.6, 5.3)\\(0.0, 0.0)}&\makecell[c]{(853.6, 3.2)\\(3.6, 0.9)}&\makecell[c]{(860.1, 1.4)\\(260.2, 54.9)}&\makecell[c]{(848.5, 1.3)\\(0.0, 0.0)}&\makecell[c]{(853.4, 2.4)\\(3.0, 0.9)}&\makecell[c]{(860.4, 1.0)\\(265.2, 69.2)}&\makecell[c]{(852.3, 2.8)\\(0.0, 0.0)}&\makecell[c]{(854.5, 2.6)\\(4.1, 0.8)}&\makecell[c]{(860.1, 0.8)\\(259.7, 57.7)}&\makecell[c]{(786.2, 10.0)\\(0.0, 0.0)}&\makecell[c]{(828.7, 4.4)\\(0.7, 0.0)}&\makecell[c]{(860.6, 3.0)\\(56.1, 7.9)}&\makecell[c]{(843.5, 3.0)\\(0.0, 0.0)}&\makecell[c]{(852.3, 1.8)\\(6.5, 0.5)}&\makecell[c]{(862.4, 2.1)\\(531.8, 94.0)}&\makecell[c]{(848.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(857.4, 2.1)\\(6.2, 1.5)}&\makecell[c]{(860.4, 0.8)\\(622.5, 111.1)}&\makecell[c]{(852.8, 1.2)\\(0.0, 0.0)}&\makecell[c]{(860.3, 1.4)\\(6.3, 0.7)}&\makecell[c]{(862.0, 0.0)\\(577.3, 115.6)}\\\hline
s3v80c900-6&\makecell[c]{(846.2, 2.7)\\(79.8, 20.6)}&\makecell[c]{(860.9, 0.3)\\(315.7, 58.4)}&\makecell[c]{(861.9, 1.4)\\(304.3, 57.9)}&\makecell[c]{(860.4, 1.6)\\(295.6, 58.4)}&\makecell[c]{(788.0, 8.6)\\(0.0, 0.0)}&\makecell[c]{(820.5, 6.7)\\(3.2, 0.7)}&\makecell[c]{(839.7, 5.1)\\(221.3, 42.1)}&\makecell[c]{(844.0, 1.8)\\(0.0, 0.0)}&\makecell[c]{(858.5, 1.9)\\(4.3, 1.8)}&\makecell[c]{(863.5, 1.9)\\(259.5, 51.9)}&\makecell[c]{(848.0, 3.7)\\(0.0, 0.0)}&\makecell[c]{(856.8, 3.8)\\(3.7, 0.8)}&\makecell[c]{(862.8, 1.0)\\(260.2, 46.9)}&\makecell[c]{(852.7, 3.3)\\(0.0, 0.0)}&\makecell[c]{(857.6, 2.8)\\(3.5, 1.0)}&\makecell[c]{(862.9, 1.6)\\(258.1, 62.8)}&\makecell[c]{(789.2, 10.1)\\(0.0, 0.0)}&\makecell[c]{(825.3, 6.5)\\(0.8, 0.0)}&\makecell[c]{(863.5, 1.6)\\(59.3, 9.7)}&\makecell[c]{(843.2, 3.7)\\(0.0, 0.0)}&\makecell[c]{(854.4, 2.6)\\(5.5, 1.2)}&\makecell[c]{(863.5, 1.7)\\(513.4, 58.3)}&\makecell[c]{(847.8, 3.9)\\(0.0, 0.0)}&\makecell[c]{(857.6, 0.7)\\(6.8, 1.2)}&\makecell[c]{(861.2, 1.3)\\(635.3, 124.3)}&\makecell[c]{(853.4, 1.5)\\(0.0, 0.0)}&\makecell[c]{(860.6, 1.3)\\(4.9, 1.5)}&\makecell[c]{(863.4, 0.5)\\(552.7, 87.1)}\\\hline
s3v80c900-7&\makecell[c]{(847.2, 5.5)\\(75.8, 14.3)}&\makecell[c]{(858.0, 2.7)\\(302.9, 33.4)}&\makecell[c]{(858.2, 1.7)\\(293.1, 53.8)}&\makecell[c]{(854.0, 1.1)\\(301.3, 60.2)}&\makecell[c]{(787.3, 9.5)\\(0.0, 0.0)}&\makecell[c]{(818.7, 6.6)\\(2.7, 0.5)}&\makecell[c]{(837.8, 4.9)\\(221.5, 45.2)}&\makecell[c]{(845.3, 1.0)\\(0.0, 0.0)}&\makecell[c]{(853.5, 0.9)\\(3.7, 0.9)}&\makecell[c]{(861.3, 1.7)\\(261.3, 56.6)}&\makecell[c]{(850.7, 2.1)\\(0.0, 0.0)}&\makecell[c]{(853.6, 0.5)\\(4.4, 0.1)}&\makecell[c]{(861.2, 1.5)\\(260.9, 65.6)}&\makecell[c]{(845.3, 2.4)\\(0.0, 0.0)}&\makecell[c]{(853.4, 0.5)\\(4.4, 0.0)}&\makecell[c]{(860.3, 1.8)\\(252.2, 49.8)}&\makecell[c]{(790.4, 7.1)\\(0.0, 0.0)}&\makecell[c]{(829.3, 4.6)\\(0.5, 0.2)}&\makecell[c]{(858.7, 4.8)\\(60.0, 10.9)}&\makecell[c]{(843.2, 3.9)\\(0.0, 0.0)}&\makecell[c]{(853.9, 1.9)\\(4.8, 1.0)}&\makecell[c]{(862.0, 2.5)\\(519.1, 72.5)}&\makecell[c]{(844.9, 3.9)\\(0.1, 0.0)}&\makecell[c]{(852.3, 1.2)\\(7.7, 2.4)}&\makecell[c]{(857.8, 1.6)\\(615.5, 89.3)}&\makecell[c]{(846.4, 3.5)\\(0.0, 0.0)}&\makecell[c]{(855.7, 2.0)\\(6.3, 1.1)}&\makecell[c]{(860.0, 0.0)\\(555.1, 94.5)}\\\hline
s3v80c900-8&\makecell[c]{(846.0, 4.4)\\(77.3, 13.4)}&\makecell[c]{(863.9, 0.7)\\(308.0, 50.4)}&\makecell[c]{(860.2, 1.2)\\(305.8, 67.6)}&\makecell[c]{(861.4, 0.8)\\(288.7, 48.2)}&\makecell[c]{(786.6, 8.8)\\(0.0, 0.0)}&\makecell[c]{(819.6, 6.7)\\(3.2, 0.7)}&\makecell[c]{(838.2, 4.6)\\(221.0, 32.9)}&\makecell[c]{(846.1, 2.2)\\(0.0, 0.0)}&\makecell[c]{(856.1, 3.1)\\(3.6, 0.8)}&\makecell[c]{(865.4, 1.2)\\(256.3, 51.3)}&\makecell[c]{(844.6, 1.7)\\(0.0, 0.0)}&\makecell[c]{(855.1, 2.8)\\(4.1, 0.7)}&\makecell[c]{(863.6, 3.0)\\(250.9, 45.1)}&\makecell[c]{(851.0, 1.5)\\(0.0, 0.0)}&\makecell[c]{(856.5, 2.8)\\(4.4, 0.0)}&\makecell[c]{(864.8, 1.1)\\(250.3, 52.6)}&\makecell[c]{(793.2, 9.5)\\(0.0, 0.0)}&\makecell[c]{(823.6, 6.9)\\(0.7, 0.0)}&\makecell[c]{(859.3, 2.8)\\(60.5, 11.2)}&\makecell[c]{(846.6, 3.2)\\(0.0, 0.0)}&\makecell[c]{(855.8, 2.8)\\(4.7, 1.0)}&\makecell[c]{(866.5, 0.5)\\(516.4, 70.5)}&\makecell[c]{(848.5, 2.9)\\(0.0, 0.0)}&\makecell[c]{(856.2, 1.5)\\(5.6, 1.2)}&\makecell[c]{(861.9, 0.8)\\(622.6, 115.5)}&\makecell[c]{(850.4, 2.7)\\(0.0, 0.0)}&\makecell[c]{(854.6, 1.0)\\(5.3, 1.4)}&\makecell[c]{(863.1, 0.3)\\(543.7, 82.0)}\\\hline
s3v80c900-9&\makecell[c]{(847.2, 3.6)\\(78.6, 13.4)}&\makecell[c]{(856.7, 1.0)\\(314.2, 54.6)}&\makecell[c]{(853.2, 3.4)\\(296.7, 48.9)}&\makecell[c]{(855.2, 1.6)\\(296.2, 67.5)}&\makecell[c]{(786.5, 10.5)\\(0.0, 0.0)}&\makecell[c]{(818.9, 6.1)\\(2.7, 0.8)}&\makecell[c]{(836.2, 4.7)\\(220.4, 37.9)}&\makecell[c]{(846.6, 2.2)\\(0.0, 0.0)}&\makecell[c]{(852.9, 1.4)\\(3.5, 0.9)}&\makecell[c]{(859.3, 0.6)\\(257.9, 50.8)}&\makecell[c]{(841.7, 1.8)\\(0.0, 0.0)}&\makecell[c]{(852.2, 1.1)\\(3.7, 0.9)}&\makecell[c]{(858.9, 1.4)\\(266.9, 75.3)}&\makecell[c]{(853.0, 3.0)\\(0.0, 0.0)}&\makecell[c]{(853.2, 2.3)\\(4.0, 0.9)}&\makecell[c]{(858.3, 1.2)\\(264.8, 71.7)}&\makecell[c]{(784.5, 12.6)\\(0.0, 0.0)}&\makecell[c]{(824.9, 5.6)\\(0.7, 0.1)}&\makecell[c]{(858.6, 3.8)\\(58.7, 8.2)}&\makecell[c]{(846.0, 3.8)\\(0.0, 0.0)}&\makecell[c]{(852.2, 1.3)\\(4.6, 1.0)}&\makecell[c]{(857.5, 1.4)\\(521.9, 69.8)}&\makecell[c]{(843.2, 1.9)\\(0.0, 0.0)}&\makecell[c]{(852.5, 1.5)\\(6.2, 1.6)}&\makecell[c]{(857.2, 1.5)\\(607.0, 79.9)}&\makecell[c]{(849.0, 5.5)\\(0.0, 0.0)}&\makecell[c]{(856.4, 0.9)\\(5.5, 1.4)}&\makecell[c]{(860.2, 0.7)\\(558.9, 101.4)}\\\hline
s3v80c900-10&\makecell[c]{(849.1, 3.1)\\(77.9, 10.4)}&\makecell[c]{(856.6, 0.5)\\(305.2, 43.2)}&\makecell[c]{(855.8, 2.2)\\(298.5, 53.4)}&\makecell[c]{(855.6, 2.0)\\(298.2, 56.0)}&\makecell[c]{(787.3, 9.6)\\(0.0, 0.0)}&\makecell[c]{(820.1, 5.5)\\(2.8, 0.5)}&\makecell[c]{(838.8, 4.0)\\(220.2, 39.6)}&\makecell[c]{(842.3, 2.2)\\(0.0, 0.0)}&\makecell[c]{(855.7, 2.1)\\(3.9, 0.8)}&\makecell[c]{(860.9, 0.9)\\(257.7, 50.5)}&\makecell[c]{(851.5, 0.8)\\(0.0, 0.0)}&\makecell[c]{(855.0, 2.0)\\(3.7, 0.9)}&\makecell[c]{(860.9, 0.9)\\(253.4, 52.9)}&\makecell[c]{(851.9, 3.2)\\(0.0, 0.0)}&\makecell[c]{(855.6, 1.8)\\(6.5, 1.1)}&\makecell[c]{(860.4, 1.3)\\(252.3, 56.3)}&\makecell[c]{(791.3, 8.8)\\(0.0, 0.0)}&\makecell[c]{(827.6, 4.7)\\(0.8, 0.0)}&\makecell[c]{(857.7, 2.6)\\(63.8, 11.0)}&\makecell[c]{(840.8, 4.2)\\(0.0, 0.0)}&\makecell[c]{(851.1, 2.4)\\(6.9, 0.4)}&\makecell[c]{(860.2, 1.1)\\(530.1, 95.2)}&\makecell[c]{(850.7, 3.7)\\(0.0, 0.0)}&\makecell[c]{(855.1, 0.9)\\(5.7, 1.6)}&\makecell[c]{(858.1, 0.8)\\(642.9, 125.2)}&\makecell[c]{(852.6, 2.0)\\(0.0, 0.0)}&\makecell[c]{(856.5, 0.8)\\(5.7, 1.3)}&\makecell[c]{(858.9, 0.3)\\(546.3, 80.2)}\\\hline
s3v80c1000-1&\makecell[c]{(936.8, 3.9)\\(81.7, 18.5)}&\makecell[c]{(945.3, 1.7)\\(332.7, 69.1)}&\makecell[c]{(948.0, 1.7)\\(331.7, 86.5)}&\makecell[c]{(947.4, 2.6)\\(314.6, 75.6)}&\makecell[c]{(874.5, 9.1)\\(0.0, 0.0)}&\makecell[c]{(906.4, 6.5)\\(3.3, 1.1)}&\makecell[c]{(926.8, 4.5)\\(227.6, 61.0)}&\makecell[c]{(926.8, 3.3)\\(0.0, 0.0)}&\makecell[c]{(944.3, 2.1)\\(7.0, 1.2)}&\makecell[c]{(948.8, 0.7)\\(273.2, 66.0)}&\makecell[c]{(919.4, 2.6)\\(0.0, 0.0)}&\makecell[c]{(945.3, 1.8)\\(4.4, 0.8)}&\makecell[c]{(948.6, 0.7)\\(268.3, 59.2)}&\makecell[c]{(930.5, 2.4)\\(0.0, 0.0)}&\makecell[c]{(943.9, 2.0)\\(3.5, 0.8)}&\makecell[c]{(948.6, 1.0)\\(281.8, 93.8)}&\makecell[c]{(876.3, 7.1)\\(0.0, 0.0)}&\makecell[c]{(912.9, 5.6)\\(0.8, 0.0)}&\makecell[c]{(947.7, 3.2)\\(62.6, 16.5)}&\makecell[c]{(924.9, 1.8)\\(0.0, 0.0)}&\makecell[c]{(936.6, 2.3)\\(6.7, 0.6)}&\makecell[c]{(949.9, 2.1)\\(549.6, 98.6)}&\makecell[c]{(929.9, 4.7)\\(0.0, 0.0)}&\makecell[c]{(942.9, 2.0)\\(7.2, 1.4)}&\makecell[c]{(947.9, 1.2)\\(668.5, 161.0)}&\makecell[c]{(934.1, 3.5)\\(0.0, 0.0)}&\makecell[c]{(944.2, 2.5)\\(6.1, 1.1)}&\makecell[c]{(952.1, 1.1)\\(576.2, 110.2)}\\\hline
s3v80c1000-2&\makecell[c]{(934.9, 4.8)\\(81.5, 18.2)}&\makecell[c]{(944.8, 1.0)\\(335.5, 79.5)}&\makecell[c]{(950.5, 1.9)\\(316.7, 60.1)}&\makecell[c]{(949.8, 0.4)\\(316.8, 66.7)}&\makecell[c]{(874.8, 11.0)\\(0.0, 0.0)}&\makecell[c]{(908.9, 5.7)\\(3.2, 0.7)}&\makecell[c]{(928.5, 4.6)\\(227.0, 59.4)}&\makecell[c]{(939.6, 4.7)\\(0.0, 0.0)}&\makecell[c]{(945.3, 0.6)\\(3.3, 0.9)}&\makecell[c]{(950.9, 1.8)\\(269.4, 56.1)}&\makecell[c]{(928.5, 3.7)\\(0.0, 0.0)}&\makecell[c]{(945.6, 0.5)\\(4.5, 0.8)}&\makecell[c]{(950.4, 2.7)\\(265.2, 55.0)}&\makecell[c]{(943.5, 2.7)\\(0.0, 0.0)}&\makecell[c]{(944.7, 1.7)\\(4.9, 0.1)}&\makecell[c]{(950.1, 1.8)\\(270.1, 60.7)}&\makecell[c]{(877.4, 13.1)\\(0.0, 0.0)}&\makecell[c]{(921.8, 4.4)\\(0.8, 0.0)}&\makecell[c]{(948.3, 3.3)\\(60.9, 12.7)}&\makecell[c]{(939.7, 3.7)\\(0.0, 0.0)}&\makecell[c]{(943.8, 1.2)\\(5.8, 1.2)}&\makecell[c]{(951.0, 1.0)\\(553.8, 102.1)}&\makecell[c]{(938.8, 4.4)\\(0.0, 0.0)}&\makecell[c]{(944.3, 0.8)\\(6.3, 1.6)}&\makecell[c]{(951.6, 1.7)\\(649.2, 129.3)}&\makecell[c]{(945.5, 2.0)\\(0.0, 0.0)}&\makecell[c]{(948.8, 1.0)\\(6.3, 1.3)}&\makecell[c]{(952.6, 1.4)\\(609.3, 76.0)}\\\hline
s3v80c1000-3&\makecell[c]{(934.1, 5.7)\\(79.4, 18.0)}&\makecell[c]{(951.0, 0.0)\\(325.6, 60.2)}&\makecell[c]{(948.4, 2.9)\\(330.5, 80.3)}&\makecell[c]{(950.6, 2.2)\\(315.5, 74.3)}&\makecell[c]{(877.3, 9.9)\\(0.0, 0.0)}&\makecell[c]{(909.6, 6.3)\\(3.0, 0.8)}&\makecell[c]{(927.3, 4.2)\\(230.6, 73.3)}&\makecell[c]{(933.0, 2.8)\\(0.0, 0.0)}&\makecell[c]{(944.5, 2.5)\\(3.8, 1.0)}&\makecell[c]{(953.4, 1.7)\\(274.7, 67.5)}&\makecell[c]{(936.1, 1.5)\\(0.0, 0.0)}&\makecell[c]{(944.7, 2.8)\\(4.2, 0.8)}&\makecell[c]{(953.5, 1.8)\\(268.2, 58.3)}&\makecell[c]{(945.9, 6.1)\\(0.0, 0.0)}&\makecell[c]{(945.6, 2.0)\\(3.6, 1.0)}&\makecell[c]{(953.8, 2.1)\\(281.9, 93.8)}&\makecell[c]{(870.4, 10.0)\\(0.0, 0.0)}&\makecell[c]{(918.2, 3.5)\\(0.8, 0.0)}&\makecell[c]{(951.1, 4.4)\\(63.6, 12.9)}&\makecell[c]{(932.3, 2.7)\\(0.0, 0.0)}&\makecell[c]{(942.3, 2.5)\\(5.2, 1.0)}&\makecell[c]{(952.9, 3.9)\\(565.0, 118.3)}&\makecell[c]{(934.1, 4.5)\\(0.0, 0.0)}&\makecell[c]{(945.3, 1.7)\\(6.3, 1.3)}&\makecell[c]{(949.9, 1.1)\\(651.3, 128.7)}&\makecell[c]{(943.4, 5.6)\\(0.0, 0.0)}&\makecell[c]{(949.7, 0.9)\\(6.1, 1.5)}&\makecell[c]{(950.0, 0.0)\\(574.7, 113.2)}\\\hline
s3v80c1000-4&\makecell[c]{(933.9, 3.1)\\(82.3, 21.7)}&\makecell[c]{(948.7, 0.9)\\(337.8, 81.9)}&\makecell[c]{(937.6, 4.1)\\(318.3, 62.4)}&\makecell[c]{(945.9, 0.3)\\(319.1, 75.6)}&\makecell[c]{(876.3, 9.3)\\(0.0, 0.0)}&\makecell[c]{(906.6, 5.5)\\(3.4, 1.0)}&\makecell[c]{(925.0, 4.8)\\(230.7, 72.9)}&\makecell[c]{(929.9, 0.9)\\(0.0, 0.0)}&\makecell[c]{(943.9, 1.5)\\(3.6, 1.0)}&\makecell[c]{(948.3, 1.2)\\(274.0, 57.9)}&\makecell[c]{(934.1, 4.1)\\(0.0, 0.0)}&\makecell[c]{(943.2, 2.2)\\(4.3, 0.9)}&\makecell[c]{(947.0, 1.8)\\(274.6, 69.8)}&\makecell[c]{(936.5, 3.4)\\(0.0, 0.0)}&\makecell[c]{(944.6, 1.9)\\(4.2, 0.8)}&\makecell[c]{(948.6, 2.3)\\(272.4, 63.0)}&\makecell[c]{(875.1, 10.2)\\(0.0, 0.0)}&\makecell[c]{(913.5, 5.7)\\(0.6, 0.2)}&\makecell[c]{(945.1, 3.0)\\(62.3, 11.8)}&\makecell[c]{(927.4, 3.9)\\(0.0, 0.0)}&\makecell[c]{(936.5, 2.0)\\(5.7, 1.4)}&\makecell[c]{(948.7, 2.0)\\(550.2, 107.1)}&\makecell[c]{(926.1, 5.1)\\(0.0, 0.0)}&\makecell[c]{(937.8, 2.9)\\(7.3, 1.3)}&\makecell[c]{(944.1, 0.9)\\(643.8, 113.0)}&\makecell[c]{(935.0, 2.6)\\(0.0, 0.0)}&\makecell[c]{(942.6, 1.3)\\(6.8, 1.3)}&\makecell[c]{(946.6, 1.2)\\(591.6, 126.8)}\\\hline
s3v80c1000-5&\makecell[c]{(939.2, 4.5)\\(82.8, 23.7)}&\makecell[c]{(946.8, 1.0)\\(326.6, 69.4)}&\makecell[c]{(946.9, 1.4)\\(328.7, 82.0)}&\makecell[c]{(950.2, 3.4)\\(312.7, 66.2)}&\makecell[c]{(873.7, 8.5)\\(0.0, 0.0)}&\makecell[c]{(907.7, 6.6)\\(3.0, 0.7)}&\makecell[c]{(928.0, 5.1)\\(227.6, 57.2)}&\makecell[c]{(933.1, 4.3)\\(0.0, 0.0)}&\makecell[c]{(943.4, 1.7)\\(4.1, 1.1)}&\makecell[c]{(951.2, 1.1)\\(274.7, 65.8)}&\makecell[c]{(935.7, 2.2)\\(0.0, 0.0)}&\makecell[c]{(943.8, 2.4)\\(3.9, 1.0)}&\makecell[c]{(951.3, 2.3)\\(274.4, 79.8)}&\makecell[c]{(941.4, 2.6)\\(0.0, 0.0)}&\makecell[c]{(942.9, 2.3)\\(4.6, 0.8)}&\makecell[c]{(951.8, 1.8)\\(265.9, 53.0)}&\makecell[c]{(874.5, 10.3)\\(0.0, 0.0)}&\makecell[c]{(915.2, 5.4)\\(0.8, 0.0)}&\makecell[c]{(949.6, 3.1)\\(60.5, 11.6)}&\makecell[c]{(936.2, 3.0)\\(0.0, 0.0)}&\makecell[c]{(943.8, 2.1)\\(6.8, 2.3)}&\makecell[c]{(949.4, 1.9)\\(557.9, 119.4)}&\makecell[c]{(934.3, 1.8)\\(0.0, 0.0)}&\makecell[c]{(945.5, 1.2)\\(5.6, 1.4)}&\makecell[c]{(951.0, 1.2)\\(657.4, 138.1)}&\makecell[c]{(939.7, 3.4)\\(0.0, 0.0)}&\makecell[c]{(944.0, 1.1)\\(7.0, 0.9)}&\makecell[c]{(950.3, 0.6)\\(578.5, 108.0)}\\\hline
s3v80c1000-6&\makecell[c]{(932.6, 3.3)\\(81.3, 18.2)}&\makecell[c]{(947.0, 0.4)\\(332.5, 75.3)}&\makecell[c]{(946.9, 2.5)\\(336.7, 88.8)}&\makecell[c]{(953.4, 3.4)\\(313.2, 72.7)}&\makecell[c]{(877.1, 10.1)\\(0.0, 0.0)}&\makecell[c]{(907.3, 6.6)\\(2.9, 0.9)}&\makecell[c]{(927.8, 4.4)\\(229.3, 67.0)}&\makecell[c]{(925.7, 1.7)\\(0.0, 0.0)}&\makecell[c]{(946.4, 1.9)\\(3.9, 1.1)}&\makecell[c]{(951.8, 1.8)\\(273.4, 68.8)}&\makecell[c]{(940.1, 2.9)\\(0.0, 0.0)}&\makecell[c]{(946.5, 3.6)\\(4.5, 0.7)}&\makecell[c]{(952.0, 1.4)\\(262.6, 56.2)}&\makecell[c]{(941.0, 2.8)\\(0.0, 0.0)}&\makecell[c]{(947.3, 2.8)\\(4.2, 0.9)}&\makecell[c]{(953.8, 2.0)\\(268.2, 63.4)}&\makecell[c]{(877.8, 9.6)\\(0.0, 0.0)}&\makecell[c]{(917.5, 5.2)\\(0.8, 0.0)}&\makecell[c]{(950.1, 4.8)\\(63.2, 13.1)}&\makecell[c]{(927.2, 4.4)\\(0.0, 0.0)}&\makecell[c]{(936.9, 3.0)\\(5.4, 1.0)}&\makecell[c]{(952.0, 2.8)\\(559.3, 115.2)}&\makecell[c]{(940.3, 2.3)\\(0.0, 0.0)}&\makecell[c]{(945.0, 1.0)\\(8.0, 0.7)}&\makecell[c]{(950.5, 0.9)\\(670.1, 167.1)}&\makecell[c]{(941.2, 1.4)\\(0.0, 0.0)}&\makecell[c]{(947.7, 1.2)\\(5.5, 1.5)}&\makecell[c]{(949.9, 0.3)\\(565.4, 89.3)}\\\hline
s3v80c1000-7&\makecell[c]{(941.3, 3.8)\\(81.5, 20.9)}&\makecell[c]{(948.9, 1.2)\\(331.1, 73.8)}&\makecell[c]{(949.0, 1.5)\\(321.1, 72.6)}&\makecell[c]{(953.5, 1.8)\\(308.2, 69.0)}&\makecell[c]{(875.5, 10.8)\\(0.0, 0.0)}&\makecell[c]{(908.0, 6.8)\\(3.4, 0.8)}&\makecell[c]{(929.4, 4.8)\\(230.2, 77.7)}&\makecell[c]{(936.8, 3.0)\\(0.0, 0.0)}&\makecell[c]{(949.7, 3.6)\\(3.9, 1.0)}&\makecell[c]{(954.5, 1.5)\\(272.3, 61.2)}&\makecell[c]{(937.2, 4.6)\\(0.0, 0.0)}&\makecell[c]{(949.3, 2.0)\\(4.4, 0.7)}&\makecell[c]{(954.9, 2.2)\\(267.1, 57.6)}&\makecell[c]{(947.2, 2.7)\\(0.0, 0.0)}&\makecell[c]{(948.4, 1.2)\\(3.9, 1.0)}&\makecell[c]{(954.3, 1.9)\\(268.6, 61.8)}&\makecell[c]{(879.7, 11.7)\\(0.0, 0.0)}&\makecell[c]{(918.8, 6.8)\\(0.9, 0.2)}&\makecell[c]{(953.9, 3.1)\\(62.1, 11.0)}&\makecell[c]{(937.6, 3.5)\\(0.0, 0.0)}&\makecell[c]{(947.4, 2.5)\\(7.1, 0.2)}&\makecell[c]{(956.0, 2.4)\\(543.4, 90.3)}&\makecell[c]{(938.6, 2.8)\\(0.0, 0.0)}&\makecell[c]{(947.2, 2.4)\\(7.6, 1.0)}&\makecell[c]{(951.8, 1.2)\\(661.3, 145.3)}&\makecell[c]{(944.6, 2.4)\\(0.0, 0.0)}&\makecell[c]{(951.4, 1.4)\\(5.9, 1.4)}&\makecell[c]{(953.9, 1.6)\\(570.7, 94.8)}\\\hline
s3v80c1000-8&\makecell[c]{(942.0, 2.5)\\(80.7, 18.9)}&\makecell[c]{(944.7, 1.6)\\(343.8, 40.6)}&\makecell[c]{(945.1, 2.9)\\(335.6, 87.0)}&\makecell[c]{(950.7, 3.3)\\(312.5, 66.2)}&\makecell[c]{(875.2, 10.0)\\(0.0, 0.0)}&\makecell[c]{(909.3, 6.6)\\(3.0, 0.6)}&\makecell[c]{(928.1, 4.7)\\(229.2, 67.7)}&\makecell[c]{(932.0, 2.4)\\(0.0, 0.0)}&\makecell[c]{(943.5, 0.8)\\(4.7, 0.3)}&\makecell[c]{(952.2, 2.3)\\(279.1, 73.0)}&\makecell[c]{(937.7, 1.0)\\(0.0, 0.0)}&\makecell[c]{(943.1, 0.7)\\(4.0, 1.0)}&\makecell[c]{(952.5, 2.6)\\(266.5, 57.2)}&\makecell[c]{(940.8, 1.7)\\(0.0, 0.0)}&\makecell[c]{(943.5, 0.8)\\(4.6, 0.8)}&\makecell[c]{(952.0, 2.8)\\(278.1, 76.2)}&\makecell[c]{(873.5, 10.0)\\(0.0, 0.0)}&\makecell[c]{(917.0, 3.9)\\(0.5, 0.2)}&\makecell[c]{(949.6, 4.2)\\(60.6, 10.4)}&\makecell[c]{(934.4, 3.8)\\(0.0, 0.0)}&\makecell[c]{(942.8, 1.5)\\(4.3, 1.1)}&\makecell[c]{(950.9, 1.8)\\(547.6, 94.7)}&\makecell[c]{(936.1, 3.9)\\(0.0, 0.0)}&\makecell[c]{(943.3, 1.6)\\(6.8, 1.3)}&\makecell[c]{(947.1, 0.9)\\(668.3, 156.3)}&\makecell[c]{(941.8, 2.9)\\(0.0, 0.0)}&\makecell[c]{(946.6, 1.7)\\(4.8, 1.2)}&\makecell[c]{(950.2, 0.4)\\(582.9, 111.5)}\\\hline
s3v80c1000-9&\makecell[c]{(944.1, 4.1)\\(80.8, 22.5)}&\makecell[c]{(951.4, 1.6)\\(343.7, 104.2)}&\makecell[c]{(955.1, 1.6)\\(318.8, 77.1)}&\makecell[c]{(955.0, 2.2)\\(307.5, 58.1)}&\makecell[c]{(873.4, 9.0)\\(0.0, 0.0)}&\makecell[c]{(909.3, 6.5)\\(3.2, 0.9)}&\makecell[c]{(931.7, 5.7)\\(230.4, 64.3)}&\makecell[c]{(938.2, 2.2)\\(0.0, 0.0)}&\makecell[c]{(948.3, 2.3)\\(4.0, 1.1)}&\makecell[c]{(958.4, 0.8)\\(268.5, 55.6)}&\makecell[c]{(944.9, 4.8)\\(0.0, 0.0)}&\makecell[c]{(950.1, 4.7)\\(3.7, 0.7)}&\makecell[c]{(957.4, 1.6)\\(274.8, 66.0)}&\makecell[c]{(951.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(947.2, 3.2)\\(4.6, 0.7)}&\makecell[c]{(958.1, 1.0)\\(278.5, 78.7)}&\makecell[c]{(879.5, 8.8)\\(0.0, 0.0)}&\makecell[c]{(914.5, 2.3)\\(0.8, 0.0)}&\makecell[c]{(955.7, 2.8)\\(62.5, 11.1)}&\makecell[c]{(939.7, 4.5)\\(0.0, 0.0)}&\makecell[c]{(951.1, 3.3)\\(6.3, 1.2)}&\makecell[c]{(958.5, 0.8)\\(550.9, 107.6)}&\makecell[c]{(942.2, 6.4)\\(0.0, 0.0)}&\makecell[c]{(954.6, 0.8)\\(6.8, 1.1)}&\makecell[c]{(957.0, 0.4)\\(648.6, 121.2)}&\makecell[c]{(946.8, 4.9)\\(0.0, 0.0)}&\makecell[c]{(953.2, 1.0)\\(5.5, 1.5)}&\makecell[c]{(954.3, 0.5)\\(580.8, 104.6)}\\\hline
s3v80c1000-10&\makecell[c]{(939.5, 3.7)\\(82.3, 21.1)}&\makecell[c]{(951.1, 0.8)\\(349.4, 102.0)}&\makecell[c]{(948.6, 3.0)\\(316.2, 85.5)}&\makecell[c]{(951.0, 3.2)\\(315.8, 77.8)}&\makecell[c]{(874.9, 12.8)\\(0.0, 0.0)}&\makecell[c]{(910.3, 6.8)\\(2.8, 0.9)}&\makecell[c]{(929.5, 4.4)\\(231.0, 78.4)}&\makecell[c]{(944.4, 3.0)\\(0.0, 0.0)}&\makecell[c]{(952.8, 1.2)\\(3.4, 0.8)}&\makecell[c]{(956.6, 1.6)\\(277.0, 69.6)}&\makecell[c]{(925.2, 2.2)\\(0.0, 0.0)}&\makecell[c]{(953.0, 1.3)\\(4.4, 0.7)}&\makecell[c]{(956.1, 1.1)\\(276.8, 72.3)}&\makecell[c]{(937.6, 2.5)\\(0.0, 0.0)}&\makecell[c]{(953.0, 1.6)\\(4.0, 0.8)}&\makecell[c]{(955.8, 1.0)\\(263.3, 55.5)}&\makecell[c]{(873.5, 12.7)\\(0.0, 0.0)}&\makecell[c]{(920.9, 5.3)\\(0.4, 0.0)}&\makecell[c]{(951.8, 5.8)\\(68.4, 12.7)}&\makecell[c]{(941.8, 5.2)\\(0.0, 0.0)}&\makecell[c]{(949.9, 2.8)\\(6.5, 1.0)}&\makecell[c]{(958.9, 0.3)\\(558.9, 118.1)}&\makecell[c]{(927.1, 3.4)\\(0.0, 0.0)}&\makecell[c]{(941.5, 2.9)\\(7.1, 1.3)}&\makecell[c]{(947.5, 1.0)\\(668.5, 137.6)}&\makecell[c]{(939.3, 3.6)\\(0.0, 0.0)}&\makecell[c]{(946.7, 1.0)\\(7.0, 0.7)}&\makecell[c]{(951.0, 1.1)\\(576.4, 106.9)}\\\hline

\hline
\end{tabular}


==> tables/max3sat80variable_sls.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
&WalkSat&$MCTS\_{WalkSat}$&\multicolumn{2}{c}{$NMC\_{WalkSat}$}&$NMC\_{Novelty}$&Best Solver\\
\hline
&flip=$10^{5.5}$&m=200&level 1, flip=$10^{3.5}$&level 2&level 1&-\\
\hline
statistic&\makecell[c]{(772.7, 0.2),(41.0, 5.8)}&\makecell[c]{(768.1, 1.9),(2475.1, 270.1)}&\makecell[c]{(772.4, 0.6),(34.6, 5.8)}&\makecell[c]{(0.0, 0.0),(0.0, 0.0)}&--&773.06\\\hline
s3v80c600-1&\makecell[c]{(586.0, 0.0),(35.2, 4.6)}&\makecell[c]{(581.7, 1.8),(2034.6, 65.6)}&\makecell[c]{(585.1, 0.3),(27.2, 2.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(583.3, 2.0),(98.1, 11.0)}&586\\\hline
s3v80c600-2&\makecell[c]{(584.0, 0.0),(35.3, 5.1)}&\makecell[c]{(580.3, 1.7),(1938.1, 29.5)}&\makecell[c]{(584.0, 0.0),(26.5, 2.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(583.0, 1.1),(95.9, 2.6)}&584\\\hline
s3v80c600-3&\makecell[c]{(589.0, 0.0),(39.7, 5.0)}&\makecell[c]{(582.8, 1.9),(1940.1, 46.7)}&\makecell[c]{(589.0, 0.0),(28.2, 3.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(585.8, 1.9),(91.7, 9.7)}&589\\\hline
s3v80c600-4&\makecell[c]{(587.0, 0.0),(35.8, 7.8)}&\makecell[c]{(582.8, 1.2),(1979.7, 35.2)}&\makecell[c]{(586.9, 0.3),(28.8, 3.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(584.7, 1.7),(100.9, 12.6)}&587\\\hline
s3v80c600-5&\makecell[c]{(588.0, 0.0),(35.6, 5.4)}&\makecell[c]{(584.8, 1.0),(1904.9, 51.1)}&\makecell[c]{(587.6, 0.5),(27.1, 2.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(587.4, 0.7),(81.1, 6.2)}&588\\\hline
s3v80c600-6&\makecell[c]{(586.0, 0.0),(38.1, 4.5)}&\makecell[c]{(582.7, 1.3),(1976.1, 83.1)}&\makecell[c]{(585.9, 0.3),(30.9, 2.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(583.3, 1.7),(96.6, 10.8)}&586\\\hline
s3v80c600-7&\makecell[c]{(588.0, 0.0),(36.4, 4.8)}&\makecell[c]{(583.6, 1.4),(1973.8, 58.9)}&\makecell[c]{(587.7, 0.5),(26.6, 2.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(587.3, 0.8),(80.2, 9.1)}&588\\\hline
s3v80c600-8&\makecell[c]{(585.0, 0.0),(32.4, 2.8)}&\makecell[c]{(581.1, 1.4),(1990.1, 41.5)}&\makecell[c]{(584.5, 0.5),(31.2, 3.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(583.4, 1.4),(101.1, 8.4)}&585\\\hline
s3v80c600-9&\makecell[c]{(588.0, 0.0),(34.7, 4.8)}&\makecell[c]{(583.8, 1.3),(1973.5, 64.7)}&\makecell[c]{(587.9, 0.3),(28.7, 3.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(586.7, 1.4),(84.5, 8.2)}&588\\\hline
s3v80c600-10&\makecell[c]{(585.0, 0.0),(37.9, 3.7)}&\makecell[c]{(580.2, 1.4),(2041.8, 52.3)}&\makecell[c]{(584.7, 0.5),(30.9, 4.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(583.5, 0.8),(96.4, 5.4)}&585\\\hline
s3v80c700-1&\makecell[c]{(681.0, 0.0),(40.2, 4.8)}&\makecell[c]{(678.6, 1.9),(2272.7, 56.7)}&\makecell[c]{(680.5, 0.5),(33.2, 3.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(680.0, 1.1),(121.3, 12.0)}&681\\\hline
s3v80c700-2&\makecell[c]{(680.0, 0.0),(41.4, 6.8)}&\makecell[c]{(675.4, 1.4),(2300.6, 99.6)}&\makecell[c]{(679.7, 0.6),(32.3, 3.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(677.9, 1.6),(124.6, 11.8)}&680\\\hline
s3v80c700-3&\makecell[c]{(682.0, 0.0),(40.4, 7.6)}&\makecell[c]{(677.0, 0.8),(2250.9, 78.0)}&\makecell[c]{(682.0, 0.0),(34.6, 2.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(680.3, 1.6),(123.4, 11.4)}&682\\\hline
s3v80c700-4&\makecell[c]{(685.0, 0.0),(38.0, 6.5)}&\makecell[c]{(683.5, 1.2),(2309.4, 93.9)}&\makecell[c]{(685.0, 0.0),(30.3, 3.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(683.6, 1.1),(109.9, 8.0)}&685\\\hline
s3v80c700-5&\makecell[c]{(679.0, 0.0),(40.0, 5.1)}&\makecell[c]{(673.5, 2.2),(2281.1, 105.0)}&\makecell[c]{(678.5, 0.7),(33.5, 4.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(677.1, 0.7),(131.7, 14.3)}&679\\\hline
s3v80c700-6&\makecell[c]{(682.0, 0.0),(36.7, 3.2)}&\makecell[c]{(676.8, 1.6),(2324.3, 91.8)}&\makecell[c]{(682.0, 0.0),(31.8, 4.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(681.2, 1.1),(122.9, 10.5)}&682\\\hline
s3v80c700-7&\makecell[c]{(678.8, 0.4),(39.5, 3.9)}&\makecell[c]{(674.6, 1.4),(2276.8, 93.5)}&\makecell[c]{(678.4, 0.5),(34.8, 7.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(677.2, 0.9),(133.0, 15.6)}&679\\\hline
s3v80c700-8&\makecell[c]{(681.0, 0.0),(38.5, 3.9)}&\makecell[c]{(676.5, 1.6),(2286.1, 101.9)}&\makecell[c]{(680.9, 0.3),(34.0, 6.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(679.5, 1.3),(123.4, 14.9)}&681\\\hline
s3v80c700-9&\makecell[c]{(682.0, 0.0),(39.7, 3.1)}&\makecell[c]{(676.9, 2.0),(2281.1, 78.4)}&\makecell[c]{(681.8, 0.4),(28.6, 2.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(678.7, 2.5),(123.6, 14.4)}&682\\\hline
s3v80c700-10&\makecell[c]{(681.0, 0.0),(38.9, 6.3)}&\makecell[c]{(676.4, 1.6),(2310.5, 87.2)}&\makecell[c]{(680.4, 0.9),(31.0, 6.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(679.5, 1.3),(115.8, 9.4)}&681\\\hline
s3v80c800-1&\makecell[c]{(772.0, 0.0),(39.4, 5.5)}&\makecell[c]{(769.5, 1.6),(2553.6, 302.9)}&\makecell[c]{(771.7, 0.5),(36.4, 9.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(770.6, 1.9),(151.2, 14.9)}&772\\\hline
s3v80c800-2&\makecell[c]{(767.1, 0.3),(41.5, 4.0)}&\makecell[c]{(761.4, 2.6),(2559.9, 294.5)}&\makecell[c]{(766.5, 0.8),(37.7, 9.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(766.6, 1.0),(162.0, 24.4)}&768\\\hline
s3v80c800-3&\makecell[c]{(773.0, 0.0),(41.4, 5.3)}&\makecell[c]{(768.2, 1.2),(2487.1, 219.0)}&\makecell[c]{(772.9, 0.3),(34.4, 4.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(772.2, 0.6),(160.4, 22.4)}&773\\\hline
s3v80c800-4&\makecell[c]{(774.0, 0.0),(39.8, 3.1)}&\makecell[c]{(768.1, 2.7),(2492.0, 212.7)}&\makecell[c]{(773.9, 0.3),(34.3, 4.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(771.4, 1.4),(154.7, 16.0)}&774\\\hline
s3v80c800-5&\makecell[c]{(772.5, 0.5),(42.1, 5.0)}&\makecell[c]{(766.1, 1.8),(2535.7, 279.2)}&\makecell[c]{(772.4, 0.8),(34.4, 3.9)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(770.9, 1.5),(161.5, 19.3)}&773\\\hline
s3v80c800-6&\makecell[c]{(772.0, 0.0),(38.7, 2.8)}&\makecell[c]{(767.4, 2.5),(2509.4, 257.7)}&\makecell[c]{(772.0, 0.0),(33.3, 3.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(771.3, 1.4),(160.0, 24.4)}&772\\\hline
s3v80c800-7&\makecell[c]{(772.7, 0.5),(40.7, 3.4)}&\makecell[c]{(768.6, 2.1),(2510.7, 241.5)}&\makecell[c]{(772.5, 0.5),(35.4, 5.6)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(770.7, 2.5),(163.3, 24.7)}&773\\\hline
s3v80c800-8&\makecell[c]{(775.0, 0.0),(42.1, 5.0)}&\makecell[c]{(768.9, 2.5),(2504.1, 242.5)}&\makecell[c]{(774.8, 0.4),(34.8, 5.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(773.6, 1.2),(154.5, 19.2)}&775\\\hline
s3v80c800-9&\makecell[c]{(773.8, 0.4),(41.5, 4.9)}&\makecell[c]{(769.7, 2.1),(2501.4, 242.6)}&\makecell[c]{(773.1, 0.7),(34.7, 4.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(773.0, 1.2),(156.8, 21.7)}&774\\\hline
s3v80c800-10&\makecell[c]{(772.0, 0.0),(41.0, 4.1)}&\makecell[c]{(768.4, 1.9),(2487.9, 239.3)}&\makecell[c]{(771.9, 0.7),(34.8, 5.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(771.4, 0.8),(150.1, 13.1)}&773\\\hline
s3v80c900-1&\makecell[c]{(864.4, 0.7),(44.5, 5.9)}&\makecell[c]{(858.7, 1.7),(2689.6, 406.1)}&\makecell[c]{(863.7, 0.6),(36.7, 7.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(863.6, 1.3),(170.3, 25.6)}&865\\\hline
s3v80c900-2&\makecell[c]{(862.8, 0.4),(43.3, 5.5)}&\makecell[c]{(857.8, 2.1),(2672.3, 399.8)}&\makecell[c]{(862.2, 0.6),(37.4, 7.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(861.5, 0.8),(176.8, 28.2)}&863\\\hline
s3v80c900-3&\makecell[c]{(865.0, 0.0),(44.7, 8.1)}&\makecell[c]{(861.4, 1.7),(2700.5, 436.1)}&\makecell[c]{(864.5, 0.8),(36.6, 5.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(864.2, 2.0),(177.4, 34.3)}&866\\\hline
s3v80c900-4&\makecell[c]{(863.8, 0.6),(43.5, 6.1)}&\makecell[c]{(860.2, 1.3),(2697.9, 422.3)}&\makecell[c]{(862.5, 1.6),(37.9, 7.5)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(860.9, 2.8),(177.9, 30.7)}&865\\\hline
s3v80c900-5&\makecell[c]{(867.2, 0.7),(42.6, 5.1)}&\makecell[c]{(862.3, 1.7),(2718.8, 430.0)}&\makecell[c]{(867.1, 0.7),(39.5, 11.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(867.2, 0.6),(181.7, 31.3)}&868\\\hline
s3v80c900-6&\makecell[c]{(868.2, 0.4),(43.8, 6.1)}&\makecell[c]{(863.4, 2.5),(2710.8, 425.7)}&\makecell[c]{(868.2, 0.9),(36.4, 5.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(866.9, 1.4),(175.3, 31.5)}&869\\\hline
s3v80c900-7&\makecell[c]{(865.9, 0.3),(43.5, 7.0)}&\makecell[c]{(859.0, 1.9),(2718.4, 441.6)}&\makecell[c]{(865.6, 0.5),(37.6, 7.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(864.5, 1.1),(183.7, 38.8)}&866\\\hline
s3v80c900-8&\makecell[c]{(866.9, 0.3),(43.5, 7.9)}&\makecell[c]{(863.8, 1.2),(2728.6, 374.2)}&\makecell[c]{(866.4, 0.7),(36.5, 5.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(865.6, 1.4),(177.1, 31.4)}&867\\\hline
s3v80c900-9&\makecell[c]{(864.0, 0.0),(43.4, 5.1)}&\makecell[c]{(858.1, 1.4),(2689.5, 370.9)}&\makecell[c]{(863.5, 0.7),(36.5, 6.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(862.9, 1.0),(179.1, 33.0)}&864\\\hline
s3v80c900-10&\makecell[c]{(863.3, 0.6),(46.4, 13.1)}&\makecell[c]{(858.5, 1.9),(2725.0, 436.6)}&\makecell[c]{(863.6, 0.7),(35.2, 4.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(862.8, 1.2),(182.8, 30.7)}&865\\\hline
s3v80c1000-1&\makecell[c]{(955.9, 0.3),(46.1, 9.0)}&\makecell[c]{(949.2, 3.9),(2868.7, 538.5)}&\makecell[c]{(955.5, 0.7),(40.8, 10.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(955.2, 1.0),(198.8, 36.3)}&956\\\hline
s3v80c1000-2&\makecell[c]{(956.2, 0.7),(45.9, 8.1)}&\makecell[c]{(951.1, 2.6),(2853.0, 512.2)}&\makecell[c]{(954.8, 0.7),(38.6, 7.3)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(955.6, 1.4),(197.5, 38.8)}&957\\\hline
s3v80c1000-3&\makecell[c]{(960.5, 0.5),(45.2, 10.6)}&\makecell[c]{(953.9, 3.4),(2866.3, 540.7)}&\makecell[c]{(959.8, 1.2),(41.2, 11.0)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(958.3, 2.3),(196.4, 36.8)}&961\\\hline
s3v80c1000-4&\makecell[c]{(953.5, 0.5),(45.4, 6.5)}&\makecell[c]{(948.5, 2.1),(2928.7, 572.5)}&\makecell[c]{(953.3, 0.8),(40.1, 7.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(953.3, 1.2),(208.0, 53.8)}&955\\\hline
s3v80c1000-5&\makecell[c]{(957.9, 0.3),(42.5, 5.5)}&\makecell[c]{(952.6, 3.1),(2926.3, 576.0)}&\makecell[c]{(957.8, 0.9),(41.5, 9.8)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(958.1, 1.0),(230.7, 30.1)}&959\\\hline
s3v80c1000-6&\makecell[c]{(960.0, 0.0),(45.9, 8.9)}&\makecell[c]{(956.0, 3.0),(2882.8, 520.8)}&\makecell[c]{(959.8, 0.4),(40.3, 8.4)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(957.2, 3.1),(201.2, 39.6)}&960\\\hline
s3v80c1000-7&\makecell[c]{(959.9, 0.3),(44.5, 6.0)}&\makecell[c]{(956.7, 1.0),(2908.1, 525.8)}&\makecell[c]{(960.0, 0.0),(38.4, 7.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(958.3, 2.2),(196.0, 41.2)}&960\\\hline
s3v80c1000-8&\makecell[c]{(957.8, 0.7),(45.1, 9.2)}&\makecell[c]{(951.9, 2.7),(2893.2, 553.4)}&\makecell[c]{(957.7, 1.2),(42.7, 16.1)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(0, 0),(0, 0)}&959\\\hline
s3v80c1000-9&\makecell[c]{(960.8, 0.6),(43.8, 6.2)}&\makecell[c]{(957.7, 2.3),(2889.4, 537.3)}&\makecell[c]{(960.5, 1.7),(39.2, 7.7)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(959.0, 2.0),(203.7, 46.5)}&962\\\hline
s3v80c1000-10&\makecell[c]{(960.4, 0.5),(45.4, 7.5)}&\makecell[c]{(954.6, 3.8),(2898.2, 536.5)}&\makecell[c]{(960.4, 0.5),(38.2, 6.2)}&\makecell[c]{(0, 0),(0, 0)}&\makecell[c]{(958.6, 1.3),(196.8, 37.6)}&961\\\hline





\end{tabular}


==> tables/novelty_120v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{10}{*}{1200}
&1&1039.0&1039.0&1038.4&1039.0&1039.0&1038.8&1039\\
&2&1039.5&1039.7&1038.4&1038.4&1038.5&1038.5&1041\\
&3&1039.9&1040.0&1038.7&1039.1&1039.9&1039.1&1040\\
&4&1042.4&1042.4&1042.0&1042.2&1042.1&1042.1&1043\\
&5&1055.7&1055.7&1056.1&1056.6&1056.0&1056.2&1057\\
&6&1032.7&1033.0&1030.3&1031.1&1032.0&1030.7&1033\\
&7&1038.0&1038.0&1034.2&1037.9&1037.5&1036.6&1038\\
&8&1033.0&1033.3&1033.4&1033.4&1033.1&1033.1&1035\\
&9&1052.0&1052.0&1052.0&1051.9&1052.0&1051.7&1052\\
&10&1046.0&1046.0&1046.0&1045.9&1046.0&1046.0&1046\\
&1&1119.6&1119.0&1119.6&1119.2&1119.2&1117.8&1120\\
&2&1127.5&1127.9&1126.4&1126.6&1127.3&1126.5&1128\\
&3&1126.3&1126.3&1126.4&1125.9&1126.1&1125.8&1127\\
&4&1123.6&1123.9&1123.5&1123.4&1123.9&1122.9&1124\\
&5&1131.6&1131.2&1131.5&1130.6&1131.4&1131.0&1132\\
&6&1117.4&1117.9&1118.8&1118.0&1118.3&1117.1&1120\\
&7&1130.1&1130.1&1130.5&1130.0&1130.8&1129.7&1131\\
&8&1125.7&1125.8&1126.0&1126.0&1125.8&1124.8&1126\\
&9&1113.6&1113.1&1113.2&1112.8&1113.7&1112.5&1114\\
&10&1120.0&1120.0&1119.9&1119.8&1119.8&1119.6&1120\\
&1&1202.8&1202.9&1202.4&1202.8&1203.0&1202.0&1203\\
&2&1207.8&1208.1&1208.0&1207.9&1208.1&1207.6&1209\\
&3&1210.8&1210.5&1209.2&1208.7&1210.3&1209.4&1211\\
&4&1196.4&1196.4&1196.5&1196.4&1196.4&1194.5&1200\\
&5&1201.0&1200.9&1201.0&1199.5&1200.9&1200.7&1201\\
&6&1203.3&1203.8&1203.2&1203.5&1203.6&1203.2&1204\\
&7&1192.3&1193.3&1192.5&1192.1&1191.7&1193.4&1194\\
&8&1205.1&1205.1&1205.6&1204.0&1204.2&1204.3&1206\\
&9&1201.8&1201.4&1201.2&1200.9&1201.2&1200.1&1202\\
&10&1186.8&1187.8&1186.1&1187.1&1185.0&1185.7&1189\\
&1&1289.0&1289.0&1288.0&1289.0&1288.9&1288.5&1289\\
&2&1286.0&1286.7&1286.8&1285.3&1285.4&1286.0&1287\\
&3&1292.7&1292.8&1292.7&1292.0&1291.8&1292.1&1293\\
&4&1285.8&1286.1&1284.8&1285.6&1285.2&1284.7&1288\\
&5&1264.5&1265.3&1263.1&1264.0&1265.2&1265.9&1267\\
&6&1290.8&1290.8&1290.4&1290.7&1289.5&1290.2&1291\\
&7&1283.2&1282.8&1282.9&1282.8&1282.7&1283.1&1284\\
&8&1287.7&1287.2&1287.5&1287.7&1287.6&1287.3&1288\\
&9&1277.0&1277.0&1276.8&1276.2&1275.5&1276.7&1277\\
&10&1283.8&1284.2&1284.6&1284.6&1285.6&1279.1&1287\\
&1&1289.0&1289.0&1288.0&1289.0&1288.9&1288.5&1367\\
&2&1286.0&1286.7&1286.8&1285.3&1285.4&1286.0&1361\\
&3&1292.7&1292.8&1292.7&1292.0&1291.8&1292.1&1367\\
&4&1285.8&1286.1&1284.8&1285.6&1285.2&1284.7&1381\\
&5&1264.5&1265.3&1263.1&1264.0&1265.2&1265.9&1353\\
&6&1290.8&1290.8&1290.4&1290.7&1289.5&1290.2&1365\\
&7&1283.2&1282.8&1282.9&1282.8&1282.7&1283.1&1375\\
&8&1287.7&1287.2&1287.5&1287.7&1287.6&1287.3&1363\\
&9&1277.0&1277.0&1276.8&1276.2&1275.5&1276.7&1360\\
&10&1283.8&1284.2&1284.6&1284.6&1285.6&1279.1&1367\\
\midrule
\multicolumn{2}{l}{Aggregate}&1186.9&1187.0&1186.5&1186.5&1186.6&1186.2&1203.9\\
\bottomrule
\end{tabular}

==> tables/novelty_140v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{10}{*}{1200}
&1&1053.8&1053.8&1052.6&1053.2&1052.7&1053.4&1056\\
&2&1043.3&1043.3&1043.4&1042.9&1043.0&1043.5&1045\\
&3&1044.9&1044.8&1044.0&1043.2&1044.4&1044.0&1045\\
&4&1047.9&1048.9&1047.6&1049.2&1050.4&1048.4&1052\\
&5&1056.3&1056.5&1056.1&1055.9&1055.3&1056.3&1057\\
&6&1049.9&1049.5&1049.8&1050.0&1048.3&1048.8&1052\\
&7&1049.5&1049.6&1049.9&1048.7&1050.2&1049.5&1052\\
&8&1046.6&1047.1&1046.3&1046.6&1045.3&1046.7&1048\\
&9&1048.6&1048.4&1048.4&1047.9&1048.3&1047.8&1049\\
&10&1059.5&1060.0&1059.8&1059.2&1059.5&1059.1&1060\\
\midrule
\multirow{10}{*}{1300}
&1&1137.2&1137.4&1136.4&1136.5&1136.3&1136.1&1138\\
&2&1128.1&1128.8&1127.3&1128.3&1127.6&1127.9&1129\\
&3&1131.1&1130.0&1130.3&1129.9&1130.6&1130.3&1132\\
&4&1135.3&1135.3&1134.1&1134.8&1135.4&1130.8&1136\\
&5&1129.2&1129.2&1128.8&1128.7&1129.1&1128.0&1131\\
&6&1131.0&1131.0&1130.6&1131.0&1130.7&1130.4&1132\\
&7&1139.4&1138.9&1139.8&1139.4&1139.5&1139.4&1140\\
&8&1142.4&1142.6&1142.2&1142.3&1141.8&1141.2&1143\\
&9&1137.8&1137.7&1136.9&1137.2&1136.3&1136.4&1138\\
&10&1128.7&1129.1&1128.7&1128.5&1128.1&1127.8&1130\\
\midrule
\multirow{10}{*}{1400}
&1&1215.9&1215.9&1216.6&1215.7&1215.5&1215.9&1218\\
&2&1221.8&1221.5&1219.6&1219.9&1220.1&1217.9&1222\\
&3&1206.8&1206.8&1205.7&1205.3&1205.8&1206.2&1207\\
&4&1216.0&1216.0&1215.9&1215.4&1215.3&1214.0&1216\\
&5&1212.9&1212.9&1212.2&1212.5&1212.2&1211.7&1213\\
&6&1211.4&1211.5&1211.3&1211.3&1210.7&1210.8&1212\\
&7&1211.4&1212.3&1211.5&1211.1&1209.4&1210.0&1213\\
&8&1218.8&1218.6&1217.4&1217.1&1217.3&1216.6&1219\\
&9&1214.6&1214.6&1214.0&1213.8&1213.8&1213.9&1215\\
&10&1211.8&1211.4&1211.9&1209.7&1211.0&1210.4&1212\\
\midrule
\multirow{10}{*}{1500}
&1&1294.6&1294.5&1294.1&1293.5&1293.6&1294.4&1295\\
&2&1298.7&1299.3&1299.1&1298.9&1298.9&1298.8&1301\\
&3&1286.8&1287.0&1286.8&1285.4&1286.9&1285.4&1288\\
&4&1301.4&1301.0&1302.1&1300.5&1300.8&1301.6&1303\\
&5&1293.3&1293.1&1292.2&1292.9&1292.6&1292.6&1295\\
&6&1300.1&1300.8&1300.6&1300.5&1300.6&1300.4&1302\\
&7&1297.8&1296.0&1296.3&1295.9&1295.2&1296.5&1298\\
&8&1300.8&1300.1&1298.8&1299.2&1298.2&1297.7&1301\\
&9&1300.9&1301.0&1300.2&1300.4&1300.2&1300.3&1301\\
&10&1296.7&1297.2&1296.9&1296.4&1295.7&1296.5&1298\\
\midrule
\multirow{10}{*}{1600}
&1&1378.5&1378.5&1378.4&1378.1&1378.2&1377.5&1379\\
&2&1378.3&1377.8&1377.8&1377.4&1377.9&1376.0&1379\\
&3&1370.2&1372.4&1371.3&1370.4&1371.4&1370.5&1374\\
&4&1375.9&1377.3&1378.0&1376.9&1376.8&1375.9&1380\\
&5&1370.4&1370.9&1369.8&1369.9&1369.9&1369.8&1372\\
&6&1379.2&1379.5&1379.4&1379.3&1379.9&1379.7&1380\\
&7&1382.0&1381.8&1381.1&1381.8&1381.7&1381.4&1382\\
&8&1371.1&1372.3&1371.4&1371.7&1370.9&1370.9&1373\\
&9&1371.4&1371.7&1371.7&1370.3&1370.7&1371.3&1372\\
&10&1371.6&1373.2&1372.8&1372.1&1371.8&1371.3&1374\\
\midrule
\multicolumn{2}{l}{Aggregate}&1214.0&1214.2&1213.8&1213.5&1213.5&1213.2&1215.18\\
\bottomrule
\end{tabular}

==> tables/novelty_160v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{10}{*}{1300}
&1&1128.8&1128.8&1127.4&1129.7&1128.5&1130.0&1133\\
&2&1160.6&1160.8&1160.7&1160.6&1159.9&1159.5&1161\\
&3&1140.6&1141.9&1140.6&1140.8&1140.7&1139.4&1143\\
\midrule
\multirow{10}{*}{1400}
&1&1231.5&1232.9&1232.4&1232.2&1231.8&1231.8&1234\\
&2&1233.6&1233.6&1233.7&1232.7&1233.4&1231.8&1236\\
&3&1230.7&1230.7&1232.1&1232.3&1232.3&1231.4&1233\\
\midrule
\multirow{10}{*}{1500}
&1&1315.8&1315.8&1315.2&1315.6&1314.8&1315.6&1317\\
&2&1298.8&1299.2&1298.1&1297.6&1298.4&1298.3&1300\\
&3&1313.2&1313.2&1313.8&1313.7&1314.0&1313.9&1316\\
\midrule
\multirow{10}{*}{1600}
&1&1374.7&1375.2&1374.6&1375.5&1376.5&1375.0&1378\\
&2&1377.1&1376.9&1375.6&1377.8&1377.5&1376.9&1378\\
&3&1386.1&1386.2&1385.2&1386.3&1385.6&1380.4&1387\\
\midrule
\multirow{10}{*}{1700}
&1&1473.4&1473.3&1473.2&1473.0&1472.4&1473.0&1474\\
&2&1468.7&1468.3&1468.3&1468.3&1468.8&1468.8&1470\\
&3&1448.9&1449.4&1449.0&1449.2&1448.9&1448.4&1451\\
\midrule
\multirow{10}{*}{1800}
&1&1545.0&1544.6&1544.3&1543.7&1544.1&1542.9&1548\\
&2&1542.9&1542.7&1543.2&1542.3&1542.8&1542.9&1544\\
&3&1543.4&1543.5&1543.3&1543.4&1542.4&1543.1&1545\\
\midrule
\multirow{10}{*}{1900}
&1&1638.8&1638.9&1638.5&1638.8&1638.4&1637.7&1639\\
&2&1636.2&1636.6&1636.4&1636.8&1636.2&1636.3&1638\\
&3&1633.4&1634.4&1634.4&1634.1&1634.3&1632.8&1636\\
\midrule
\multirow{10}{*}{2000}
&1&1706.4&1705.5&1704.9&1705.9&1706.0&1706.0&1707\\
&2&1727.9&1727.8&1728.0&1727.6&1726.4&1728.0&1728\\
&3&1717.0&1716.8&1715.8&1717.0&1714.5&1717.0&1718\\
\midrule
\multirow{10}{*}{2100}
&1&1805.0&1805.9&1804.4&1804.8&1804.9&1805.1&1806\\
&2&1800.2&1800.5&1799.9&1800.1&1800.3&1799.9&1801\\
&3&1793.8&1794.8&1792.8&1793.7&1792.4&1794.0&1795\\
\midrule
\multirow{10}{*}{2200}
&1&1887.8&1888.3&1888.9&1888.9&1889.2&1888.4&1890\\
&2&1866.3&1866.6&1866.0&1865.1&1864.0&1861.6&1867\\
&3&1872.8&1873.3&1873.3&1872.6&1873.2&1872.6&1874\\
\midrule
\multirow{10}{*}{2300}
&1&1945.9&1945.6&1944.3&1945.3&1945.1&1945.1&1947\\
&2&1947.9&1948.6&1947.3&1948.1&1947.9&1945.4&1951\\
&3&1955.1&1955.4&1954.9&1953.9&1954.7&1954.4&1957\\
\midrule
\multirow{10}{*}{2400}
&1&2027.3&2026.4&2025.8&2026.4&2025.9&2025.8&2030\\
&2&2034.1&2034.9&2033.6&2034.2&2033.1&2033.4&2035\\
&3&2018.6&2019.8&2016.2&2017.4&2019.1&2017.5&2020\\
\midrule
\multirow{10}{*}{2500}
&1&2114.8&2115.3&2115.4&2115.4&2114.5&2116.0&2117\\
&2&2117.8&2118.2&2115.8&2116.2&2117.2&2117.3&2120\\
&3&2117.8&2117.0&2117.8&2117.7&2117.9&2118.0&2118\\
\midrule
\multirow{10}{*}{2600}
&1&2207.4&2207.9&2207.4&2206.1&2204.7&2205.0&2208\\
&2&2200.9&2201.4&2201.8&2200.9&2200.6&2201.5&2203\\
&3&2185.4&2186.1&2185.6&2183.5&2184.8&2181.9&2187\\

\midrule
\multicolumn{2}{l}{Aggregate}&1670.8&1671.0&1670.5&1670.6&1670.4&1670.1&1672.38\\
\bottomrule
\end{tabular}

==> tables/novelty_180v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{7}{*}{1200}
&1&1062.0&1062.6&1061.6&1063.1&1062.2&1061.5&1066\\
&2&1068.5&1068.8&1067.4&1067.9&1068.8&1068.2&1070\\
&3&1067.0&1067.1&1067.7&1067.1&1067.5&1066.9&1069\\
&4&1068.8&1069.0&1069.1&1069.0&1068.8&1069.7&1072\\
\midrule
\multirow{7}{*}{1300}
&1&1144.9&1144.5&1143.0&1143.7&1143.6&1142.1&1147\\
&2&1161.7&1161.7&1161.5&1161.6&1161.7&1161.3&1162\\
&3&1148.5&1148.7&1148.2&1147.7&1148.5&1148.8&1150\\
&4&1149.2&1148.6&1149.2&1149.3&1149.4&1149.6&1151\\
\midrule
\multirow{7}{*}{1400}
&1&1232.5&1232.7&1232.5&1232.3&1232.1&1230.4&1235\\
&2&1232.8&1233.3&1232.4&1231.6&1231.3&1232.0&1235\\
&3&1244.0&1244.0&1243.7&1243.2&1243.5&1243.3&1244\\
&4&1235.9&1237.4&1237.4&1237.1&1235.5&1235.7&1240\\
\midrule
\multirow{7}{*}{1500}
&1&1313.0&1313.4&1313.5&1313.6&1313.5&1313.6&1316\\
&2&1317.4&1318.0&1317.8&1317.3&1316.6&1317.6&1320\\
&3&1319.8&1320.1&1320.1&1319.5&1319.4&1318.4&1321\\
&4&1316.9&1317.4&1316.9&1316.7&1316.3&1316.0&1319\\
\midrule
\multirow{7}{*}{1600}
&1&1396.5&1397.9&1397.7&1396.1&1395.5&1396.9&1400\\
&2&1392.5&1394.2&1392.4&1392.1&1392.9&1393.3&1396\\
&3&1382.3&1383.3&1381.9&1381.3&1381.3&1381.2&1384\\
&4&1398.1&1399.4&1398.4&1398.8&1398.7&1398.7&1400\\
\midrule
\multirow{7}{*}{1700}
&1&1474.6&1474.4&1474.5&1474.2&1472.6&1474.2&1475\\
&2&1467.7&1469.6&1468.0&1467.0&1467.1&1469.4&1471\\
&3&1489.4&1490.6&1490.3&1490.1&1490.7&1488.9&1491\\
&4&1493.8&1493.7&1493.4&1493.8&1493.6&1493.5&1494\\
\midrule
\multirow{7}{*}{1800}
&1&1557.5&1557.8&1556.6&1556.9&1557.2&1556.8&1559\\
&2&1555.1&1556.6&1554.9&1554.6&1555.3&1555.5&1558\\
&3&1566.2&1566.9&1566.2&1566.7&1566.4&1565.8&1568\\
&4&1557.4&1557.7&1558.0&1555.8&1556.5&1556.1&1559\\
\midrule
\multirow{7}{*}{1900}
&1&1652.1&1653.5&1653.4&1653.3&1653.7&1653.7&1655\\
&2&1651.4&1651.5&1651.6&1650.8&1652.1&1652.3&1654\\
&3&1647.5&1647.2&1647.5&1646.7&1648.0&1648.0&1648\\
&4&1639.0&1641.9&1640.1&1640.3&1640.0&1638.8&1643\\
\midrule
\multirow{7}{*}{2000}
&1&1714.5&1716.2&1715.3&1713.7&1713.7&1715.4&1718\\
&2&1713.1&1712.7&1713.0&1713.3&1711.8&1712.7&1715\\
&3&1728.2&1728.4&1727.8&1728.0&1727.1&1726.9&1729\\
&4&1718.8&1719.1&1719.0&1719.1&1719.1&1718.9&1720\\
\midrule
\multirow{7}{*}{2100}
&1&1803.2&1804.8&1803.8&1802.8&1803.2&1803.2&1806\\
&2&1795.5&1796.0&1795.0&1795.3&1795.3&1793.9&1799\\
&3&1804.8&1804.4&1803.8&1805.6&1805.6&1805.0&1807\\
&4&1794.5&1794.8&1792.8&1793.5&1793.5&1794.7&1797\\
\midrule
\multirow{7}{*}{2200}
&1&1866.9&1868.6&1866.5&1866.3&1866.3&1867.1&1870\\
&2&1876.9&1880.1&1878.5&1875.9&1876.5&1876.9&1882\\
&3&1892.2&1893.1&1893.5&1891.8&1892.0&1892.0&1894\\
&4&1881.1&1881.7&1882.0&1881.0&1881.0&1881.1&1883\\
\midrule
\multicolumn{2}{l}{Aggregate}&1477.1&1477.8&1477.2&1476.9&1476.9&1477.0&1479.36\\
\bottomrule
\end{tabular}

==> tables/novelty_200v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{7}{*}{1200}
&1&1080.1&1079.7&1079.8&1080.0&1080.4&1080.5&1082\\
&2&1071.7&1070.7&1071.0&1069.9&1067.7&1069.2&1073\\
&3&1073.1&1072.7&1072.8&1072.8&1071.7&1072.3&1075\\
&4&1084.2&1084.3&1084.1&1084.2&1084.8&1083.7&1085\\
&5&1080.9&1081.4&1080.2&1080.5&1080.1&1081.0&1083\\
&6&1070.7&1070.6&1069.0&1067.8&1066.8&1068.7&1073\\
&7&1086.5&1086.2&1085.9&1086.4&1086.9&1085.9&1088\\
\midrule
\multirow{7}{*}{1300}
&1&1152.9&1152.5&1152.8&1152.4&1152.1&1153.0&1156\\
&2&1152.7&1154.1&1152.5&1152.5&1153.0&1152.8&1157\\
&3&1176.7&1176.9&1176.1&1176.0&1176.1&1176.5&1179\\
&4&1158.8&1159.7&1159.4&1158.5&1158.2&1159.1&1161\\
&5&1155.5&1156.0&1154.4&1153.9&1155.2&1154.9&1158\\
&6&1162.7&1163.2&1163.3&1162.1&1161.8&1161.3&1166\\
&7&1170.3&1171.0&1170.7&1170.3&1169.8&1170.5&1172\\
\midrule
\multirow{7}{*}{1400}
&1&1241.8&1242.5&1241.5&1240.2&1241.6&1241.1&1244\\
&2&1251.3&1251.3&1251.2&1251.0&1251.1&1248.4&1253\\
&3&1247.9&1248.4&1247.0&1247.2&1247.3&1246.9&1250\\
&4&1233.5&1233.6&1231.4&1232.5&1231.5&1231.6&1236\\
&5&1243.4&1243.4&1244.0&1244.0&1243.8&1243.1&1247\\
&6&1254.5&1254.8&1254.0&1254.5&1254.6&1254.8&1255\\
&7&1256.8&1256.9&1256.1&1254.8&1255.3&1256.3&1258\\
\midrule
\multirow{7}{*}{1500}
&1&1332.5&1332.6&1331.3&1331.6&1329.8&1331.5&1335\\
&2&1333.3&1333.8&1334.0&1334.0&1334.0&1334.0&1335\\
&3&1333.9&1334.1&1334.3&1333.5&1334.6&1334.6&1335\\
&4&1318.5&1319.3&1316.7&1319.7&1320.0&1318.8&1322\\
&5&1324.8&1324.5&1323.9&1323.8&1323.5&1324.8&1326\\
&6&1318.0&1318.2&1317.1&1316.3&1317.5&1316.7&1320\\
&7&1314.6&1318.3&1311.8&1315.3&1313.3&1315.2&1321\\
\midrule
\multirow{7}{*}{1600}
&1&1399.7&1400.9&1400.5&1399.9&1401.0&1400.2&1405\\
&2&1419.5&1420.0&1420.0&1419.5&1419.6&1419.9&1422\\
&3&1411.8&1412.7&1412.3&1413.1&1413.0&1409.7&1414\\
&4&1401.5&1401.9&1401.6&1401.5&1401.0&1401.7&1405\\
&5&1400.5&1403.4&1399.2&1401.0&1400.1&1402.0&1406\\
&6&1419.9&1419.9&1420.5&1419.9&1419.9&1420.3&1421\\
&7&1403.1&1403.2&1403.3&1403.9&1403.2&1404.1&1408\\
\midrule
\multirow{7}{*}{1700}
&1&1504.6&1506.8&1506.0&1506.2&1505.6&1506.6&1507\\
&2&1490.2&1491.2&1489.5&1490.4&1490.4&1490.4&1493\\
&3&1484.6&1484.4&1483.1&1484.6&1484.5&1483.6&1487\\
&4&1486.0&1486.2&1485.3&1485.4&1485.2&1485.8&1488\\
&5&1480.2&1482.1&1480.8&1478.8&1479.4&1480.6&1483\\
&6&1490.0&1490.2&1489.4&1489.3&1488.8&1489.1&1491\\
&7&1497.0&1497.9&1497.0&1497.1&1497.1&1497.1&1499\\
\midrule
\multirow{7}{*}{1800}
&1&1593.0&1592.5&1592.9&1592.7&1592.8&1592.8&1594\\
&2&1576.5&1576.8&1575.8&1575.7&1575.7&1574.0&1577\\
&3&1569.6&1569.3&1569.2&1568.4&1568.6&1567.8&1571\\
&4&1574.9&1575.5&1574.6&1575.2&1575.6&1573.6&1579\\
&5&1574.1&1573.5&1575.2&1574.7&1573.4&1574.4&1580\\
&6&1567.8&1569.1&1569.2&1568.8&1566.9&1568.4&1572\\
&7&1569.8&1572.0&1570.1&1571.4&1571.7&1572.1&1574\\

\midrule
\multicolumn{2}{l}{Aggregate}&1326.4&1326.9&1326.2&1326.2&1326.0&1326.2&1329.0\\
\bottomrule
\end{tabular}

==> tables/novelty_250v.tex <==

\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{7}{*}{1200}
&1&989.0&988.3&987.7&986.9&987.7&986.8&995\\
&2&989.4&989.5&988.8&988.4&988.6&988.2&995\\
&3&988.8&989.4&986.9&987.8&988.6&987.6&995\\
&4&986.9&987.9&986.8&986.8&987.4&985.9&994\\
&5&987.6&989.7&987.7&986.7&987.6&987.2&994\\
&6&988.1&988.7&987.2&986.6&986.8&985.9&994\\
&7&987.6&988.2&987.2&987.3&987.1&986.7&994\\
&8&987.4&988.4&987.2&986.8&987.1&987.2&995\\
&9&988.5&988.0&987.7&987.3&987.0&986.8&994\\
&10&988.1&989.0&988.5&986.4&986.8&987.5&994\\
&11&988.6&988.5&988.8&987.1&987.3&987.0&994\\
&12&988.6&989.0&988.4&986.5&986.4&987.3&994\\
&13&988.5&988.5&987.7&988.2&987.0&986.4&995\\
&14&988.6&989.0&988.4&986.8&986.9&987.8&995\\
&15&990.0&989.4&988.3&986.4&987.3&986.1&995\\
&16&987.8&989.3&987.9&986.6&987.4&986.8&995\\
&17&988.1&988.7&987.0&985.8&986.3&986.9&994\\
&18&988.8&988.1&986.7&987.2&988.5&986.1&994\\
&19&988.2&989.3&986.9&986.7&986.7&985.9&995\\
&20&988.2&988.7&987.2&986.3&986.8&986.8&993\\
&21&988.7&989.1&988.0&987.1&986.9&986.7&996\\
&22&988.1&988.1&987.0&987.5&987.1&986.0&995\\
&23&988.4&989.9&988.4&987.3&987.9&987.1&994\\
&24&989.4&988.6&987.5&987.3&988.4&988.3&995\\
statistic&\\
\midrule
\multicolumn{2}{l}{Aggregate}&988.4&988.8&987.7&987.0&987.3&986.9&994.5\\
\bottomrule
\end{tabular}

==> tables/novelty_300v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{7}{*}{1200}
&1&1185.5&1187.8&1184.6&1184.3&1185.4&1184.1&1194\\
&2&1186.0&1187.0&1185.1&1184.6&1185.7&1185.2&1195\\
&3&1185.9&1185.5&1184.7&1183.3&1184.3&1185.0&1194\\
&4&1185.1&1185.2&1184.7&1183.7&1185.3&1184.6&1193\\
&5&1185.9&1186.2&1185.8&1184.6&1184.7&1183.9&1194\\
&6&1185.3&1185.6&1185.4&1184.8&1185.5&1185.1&1194\\
&7&1185.6&1186.0&1187.3&1184.9&1185.4&1183.6&1195\\
&8&1185.0&1186.1&1185.4&1184.7&1184.7&1184.8&1193\\
&9&1184.9&1185.0&1184.4&1184.9&1185.2&1184.8&1193\\
&10&1184.9&1184.8&1184.8&1185.5&1184.2&1184.2&1193\\
&11&1185.8&1186.2&1184.2&1185.3&1185.8&1184.1&1194\\
&12&1187.5&1185.8&1185.8&1184.0&1185.2&1184.9&1193\\
&13&1186.4&1186.5&1187.5&1185.3&1184.9&1185.4&1194\\
&14&1186.4&1187.0&1185.5&1184.2&1184.9&1185.3&1194\\
&15&1185.7&1185.4&1184.8&1185.5&1184.1&1184.3&1193\\
&16&1185.8&1185.8&1185.1&1185.5&1184.0&1184.3&1194\\
&17&1185.1&1186.4&1184.6&1184.6&1183.5&1184.8&1193\\
&18&1186.9&1186.4&1185.5&1185.5&1184.9&1184.1&1193\\
&19&1184.0&1185.4&1184.9&1184.5&1184.6&1184.6&1194\\
&20&1184.1&1184.6&1184.5&1183.9&1185.4&1184.8&1194\\
&21&1185.9&1186.2&1185.6&1184.1&1185.2&1185.0&1195\\
&22&1186.1&1185.9&1185.4&1184.3&1184.7&1184.6&1194\\
&23&1186.1&1187.1&1185.7&1186.3&1185.8&1184.6&1193\\
&24&1185.7&1185.5&1185.7&1183.9&1185.4&1185.3&1193\\
\midrule
\multicolumn{2}{l}{Aggregate}&1185.6&1186.0&1185.3&1184.7&1185.0&1184.6&1193.70\\
\bottomrule
\end{tabular}

==> tables/novelty_70v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{10}{*}{800}
&1&767.9&768.5&766.8&767.5&767.9&767.9&769\\
&2&765.5&764.9&763.8&765.5&765.7&764.7&766\\
&3&769.9&770.0&769.9&770.0&770.0&769.6&770\\
&4&771.4&771.4&769.4&770.4&770.1&769.7&772\\
&5&768.7&768.6&767.3&768.4&768.4&768.1&769\\
&6&769.9&769.9&769.6&769.8&769.8&769.8&770\\
&7&768.9&768.9&768.1&768.4&768.0&768.4&769\\
&8&765.7&765.9&765.4&765.3&765.4&765.3&766\\
&9&767.3&767.0&766.2&766.2&766.1&767.0&768\\
&10&769.7&769.8&769.6&769.5&769.7&769.6&770\\
\midrule
\multirow{10}{*}{900}
&1&860.2&860.3&859.0&860.3&859.2&860.3&861\\
&2&862.0&862.0&861.6&861.9&861.9&861.9&862\\
&3&860.2&860.7&858.6&860.8&860.8&860.1&861\\
&4&860.1&860.5&858.5&860.0&860.1&859.9&861\\
&5&859.8&859.7&858.2&859.4&859.0&859.0&860\\
&6&858.8&858.6&858.0&857.6&858.0&858.3&859\\
&7&859.2&859.8&857.3&858.6&858.4&857.4&860\\
&8&858.0&858.0&857.7&857.9&858.0&857.9&858\\
&9&864.6&864.8&864.2&864.0&864.2&864.6&865\\
&10&860.4&860.4&858.8&860.1&860.4&860.6&861\\
\midrule
\multirow{10}{*}{1000}
&1&951.7&951.2&949.6&951.8&950.9&951.1&953\\
&2&957.0&956.9&955.5&957.0&957.0&957.0&957\\
&3&952.8&952.9&952.5&952.1&952.6&953.0&955\\
&4&952.0&951.9&949.4&951.5&952.3&950.8&953\\
&5&958.0&958.0&957.2&957.1&957.7&957.7&958\\
&6&949.5&949.3&948.0&948.5&948.5&948.4&950\\
&7&949.7&950.0&947.6&949.6&948.2&948.6&951\\
&8&952.0&952.0&950.6&951.7&951.4&951.7&952\\
&9&950.3&950.3&948.4&949.6&949.9&950.1&951\\
&10&955.0&955.0&954.7&954.8&955.0&955.0&955\\
\midrule
\multirow{10}{*}{1100}
&1&1043.2&1043.8&1042.0&1043.1&1043.3&1042.9&1044\\
&2&1044.6&1044.7&1042.8&1043.8&1043.5&1044.0&1045\\
&3&1046.4&1046.2&1045.4&1045.9&1045.3&1045.9&1047\\
&4&1048.0&1047.7&1046.4&1047.5&1047.9&1047.8&1048\\
&5&1047.0&1047.0&1046.0&1046.7&1046.7&1046.9&1047\\
&6&1046.8&1046.6&1045.2&1045.8&1046.0&1045.6&1047\\
&7&1046.0&1047.0&1045.8&1045.5&1046.2&1044.1&1047\\
&8&1049.0&1049.0&1043.6&1046.9&1045.8&1046.9&1049\\
&9&1052.0&1051.5&1052.0&1052.0&1052.0&1051.5&1052\\
&10&1041.8&1041.8&1041.0&1041.5&1041.3&1041.6&1042\\
\midrule
\multirow{10}{*}{1200}
&1&1133.4&1133.5&1132.5&1133.2&1133.4&1133.1&1134\\
&2&1136.4&1136.8&1135.4&1135.7&1136.6&1135.9&1137\\
&3&1135.0&1135.0&1134.1&1134.5&1134.5&1134.7&1135\\
&4&1133.0&1133.0&1132.2&1132.5&1132.7&1132.7&1133\\
&5&1134.8&1134.9&1134.2&1134.6&1133.8&1134.3&1135\\
&6&1134.0&1134.0&1132.7&1133.1&1133.4&1134.0&1134\\
&7&1137.4&1137.4&1136.4&1137.2&1137.4&1137.2&1138\\
&8&1136.6&1136.4&1133.3&1135.4&1135.6&1135.4&1137\\
&9&1138.7&1138.2&1135.2&1138.7&1138.8&1138.5&1139\\
&10&1135.8&1136.9&1133.4&1135.7&1135.2&1136.3&1137\\

\midrule
\multicolumn{2}{l}{Aggregate}&952.7&952.8&951.4&952.3&952.3&952.3&953.18\\
\bottomrule
\end{tabular}

==> tables/novelty_80v.tex <==
\begin{tabular}{ll*{7}{r}}
\toprule
Clauses & Ins &$UCTMax$&$NMCTSMax$&\multicolumn{2}{c}{$NMCSZMax$}&\multicolumn{2}{c}{$NMCSMax$}&Optimal\\
&&&&&&&& Solution\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & &m=100&rounds=5&rounds=1&rounds=5&rounds=1& \\
       &     & &     &level 1&level 2&level 1&level 2& \\
\midrule
\multirow{10}{*}{600}
&1&585.2&585.8&585.1&585.2&585.2&585.8&586\\
&2&583.6&583.4&582.5&583.4&583.4&583.4&584\\
&3&588.2&587.8&586.2&587.4&587.4&585.7&589\\
&4&586.7&586.3&586.0&586.3&586.6&585.7&587\\
&5&588.0&587.7&587.8&587.7&587.8&587.9&588\\
&6&585.6&585.9&584.4&584.2&585.1&584.5&586\\
&7&588.0&588.0&587.4&587.5&587.8&587.6&588\\
&8&584.2&584.1&582.0&583.2&582.4&584.1&585\\
&9&588.0&588.0&588.0&588.0&587.9&587.8&588\\
&10&584.8&584.7&583.3&584.3&584.9&584.6&585\\
\midrule
\multirow{10}{*}{700}
&1&680.9&680.9&680.6&680.7&680.7&680.4&681\\
&2&679.9&679.7&678.5&678.5&679.3&679.3&680\\
&3&681.8&681.3&680.6&681.3&680.6&681.8&682\\
&4&684.9&685.0&684.4&684.4&684.5&685.0&685\\
&5&678.4&678.7&677.2&678.7&678.2&678.7&679\\
&6&681.8&681.4&679.5&680.9&680.5&680.6&682\\
&7&677.6&677.9&677.0&677.9&678.0&678.4&679\\
&8&680.7&680.8&678.2&679.6&679.7&679.8&681\\
&9&680.5&679.9&679.7&679.6&680.5&679.9&682\\
&10&680.9&681.0&679.5&680.1&680.3&680.6&681\\
\midrule
\multirow{10}{*}{800}
&1&771.7&771.3&770.5&771.3&771.3&771.0&772\\
&2&767.5&767.7&766.3&767.5&767.0&767.1&768\\
&3&772.8&772.8&771.7&771.5&771.4&771.6&773\\
&4&773.2&773.8&769.5&773.0&772.7&772.9&774\\
&5&771.9&771.6&769.8&769.0&770.1&771.6&773\\
&6&771.4&771.7&771.1&771.5&771.2&770.5&772\\
&7&772.8&773.0&772.2&772.8&772.4&772.4&773\\
&8&774.2&774.4&773.0&773.3&774.1&774.3&775\\
&9&773.8&774.0&772.6&773.9&773.3&773.6&774\\
&10&771.9&772.3&772.0&772.1&771.6&771.9&773\\
\midrule
\multirow{10}{*}{900}
&1&864.8&864.7&862.7&863.3&863.5&863.5&865\\
&2&863.0&862.8&861.0&862.7&861.9&862.5&863\\
&3&865.7&865.0&863.1&864.6&864.8&864.8&866\\
&4&862.1&862.4&861.2&862.1&862.3&862.4&865\\
&5&867.3&867.7&865.8&867.0&867.8&867.6&868\\
&6&867.9&868.5&868.5&867.9&867.9&868.7&869\\
&7&865.5&865.2&864.2&865.4&865.1&864.9&866\\
&8&867.0&866.9&866.6&866.3&866.6&866.1&867\\
&9&863.8&863.9&863.5&862.8&863.2&863.8&864\\
&10&863.8&864.2&863.2&863.9&863.1&863.9&865\\
\midrule
\multirow{10}{*}{1000}
&1&955.5&955.3&954.4&955.0&954.9&954.8&956\\
&2&956.8&957.0&954.9&955.6&955.5&956.2&957\\
&3&960.8&959.8&957.9&958.9&959.4&960.2&961\\
&4&954.2&954.3&953.7&954.3&953.4&954.3&955\\
&5&958.6&958.1&956.9&957.6&957.1&958.1&959\\
&6&960.0&959.7&957.8&959.3&959.5&957.9&960\\
&7&960.0&960.0&959.5&959.5&960.0&959.5&960\\
&8&958.6&958.0&957.8&957.2&957.9&958.3&959\\
&9&960.9&960.9&959.5&960.9&960.4&960.7&962\\
&10&960.5&959.9&959.6&959.5&960.0&960.2&961\\
\midrule
\multicolumn{2}{l}{Aggregate}&772.6&772.5&771.4&772.0&772.0&772.1&773.06\\
\bottomrule
\end{tabular}

==> tables/rollouttrial.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
&MCTS&$MCTS\_{H1}$&$MCTS\_{H2}$&$MCTS\_{H3}$&\multicolumn{3}{c}{NMC}&\multicolumn{3}{c}{$NMC\_{H1}$}&\multicolumn{3}{c}{$NMC\_{H2}$}&\multicolumn{3}{c}{$NMC\_{H3}$}\\
\hline
&m=200&m=200&m=200&m=200&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2&playout&level 1&level 2\\
\hline
statistic&\makecell[c]{(933.2, 3.7)\\(73.5, 10.3)}&\makecell[c]{(943.9, 1.4)\\(303.8, 49.6)}&\makecell[c]{(943.7, 1.9)\\(297.5, 55.9)}&\makecell[c]{(945.0, 2.0)\\(289.0, 50.8)}&\makecell[c]{(875.0, 10.3)\\(0.0, 0.0)}&\makecell[c]{(907.3, 6.2)\\(2.9, 0.7)}&\makecell[c]{(926.1, 4.5)\\(199.8, 36.0)}&\makecell[c]{(929.7, 2.8)\\(0.0, 0.0)}&\makecell[c]{(941.0, 2.1)\\(3.8, 0.7)}&\makecell[c]{(947.2, 1.6)\\(231.3, 35.3)}&\makecell[c]{(930.1, 2.7)\\(0.0, 0.0)}&\makecell[c]{(941.2, 2.0)\\(3.7, 0.7)}&\makecell[c]{(947.1, 1.7)\\(226.5, 32.9)}&\makecell[c]{(935.4, 2.5)\\(0.0, 0.0)}&\makecell[c]{(941.0, 2.1)\\(3.6, 0.7)}&\makecell[c]{(947.2, 1.7)\\(227.5, 38.9)}\\
\end{tabular}
%statistic&\makecell[c]{(736.1, 3.3)\\(73.7, 13.0)}&\makecell[c]{(745.3, 1.1)\\(282.1, 45.6)}&\makecell[c]{(745.4, 1.7)\\(261.8, 44.7)}&\makecell[c]{(746.9, 1.7)\\(251.3, 38.0)}&\makecell[c]{(682.5, 9.0)\\(0.0, 0.0)}&\makecell[c]{(711.4, 5.5)\\(2.5, 0.7)}&\makecell[c]{(728.4, 3.9)\\(196.4, 31.4)}&\makecell[c]{(732.8, 2.3)\\(0.0, 0.0)}&\makecell[c]{(743.0, 2.0)\\(3.3, 0.7)}&\makecell[c]{(748.8, 1.3)\\(233.5, 37.8)}&\makecell[c]{(734.6, 2.2)\\(0.0, 0.0)}&\makecell[c]{(743.0, 2.0)\\(3.4, 0.7)}&\makecell[c]{(748.6, 1.4)\\(231.1, 42.6)}&\makecell[c]{(738.9, 2.3)\\(0.0, 0.0)}&\makecell[c]{(742.8, 1.9)\\(3.6, 0.6)}&\makecell[c]{(748.7, 1.3)\\(229.9, 41.1)}\\\hline
